Collaborative Inference for Large Models with Task Offloading and Early Exiting

In 5G smart cities, edge computing is employed to provide nearby computing services for end devices, and the large-scale models (e.g., GPT and LLaMA) can be deployed at the network edge to boost the service quality. However, due to the constraints of memory size and computing capacity, it is difficult to run these large-scale models on a single edge node. To meet the resource constraints, a large-scale model can be partitioned into multiple sub-models and deployed across multiple edge nodes. Then tasks are offloaded to the edge nodes for collaborative inference. Additionally, we incorporate the early exit mechanism to further accelerate inference. However, the heterogeneous system and dynamic environment will significantly affect the inference efficiency. To address these challenges, we theoretically analyze the coupled relationship between task offloading strategy and confidence thresholds, and develop a distributed algorithm, termed DTO-EE, based on the coupled relationship and convex optimization. DTO-EE enables each edge node to jointly optimize its offloading strategy and the confidence threshold, so as to achieve a promising trade-off between response delay and inference accuracy. The experimental results show that DTO-EE can reduce the average response delay by 21%-41% and improve the inference accuracy by 1%-4%, compared to the baselines.

==> content/ProblemFormulation.tex <==
\subsection{System Workflow}


The system workflow is illustrated in Fig. \ref{fig:sysprocess}. We divide the system timeline into fixed-length time slots, each comprising a configuration update phase and a task offloading phase.
Unlike current algorithms that maintain a static offloading strategy over a long time slot\cite{chen2018computation}, our approach updates the task offloading strategy and confidence threshold every few seconds, enhancing adaptability to dynamic edge environments.
% Each time slot is divided into two phases: the configuration update phase and the task offloading phase.
% Shorter time slots offer better adaptability to dynamic environment. 
% Some current algorithms assume a fixed task offloading strategy over a long time slot\cite{chen2018computation}, which is unsuitable for high-speed dynamic scenarios.
% Our proposed scheme updates the configuration of task offloading strategy and confidence threshold every few seconds, sufficiently accommodating dynamic edge scenarios (such as the Internet of Vehicles).
% During the configuration update phase of each time slot, each node updates the offloading strategy and confidence threshold based on local information.
% information, including the resource utilization status(such as computing resources and bandwidth) and the the estimated remaining time.
% This local information can be obtained or measured through requests and return messages between edge nodes\cite{zekri2012review}.
% Compared with the length of the entire time slot, the length of the strategy update phase (about 50ms) is negligible. 
% We propose a distributed optimization algorithm that iteratively achieves efficient offloading strategy and confidence threshold with performance guarantees.
% %The algorithm consists of two parts, one is the task receiver algorithm, and the other is the task offloader algorithm.
% During the configuration update phase of each time slot, each node updates the offloading strategy and confidence threshold based on local communication.

The configuration update phase is responsible for determining the task offloading strategy and confidence threshold, which are used during the task offloading phase.
Specifically, during the configuration update phase, as a predecessor or successor, each edge node conducts multiple rounds of local communication with its neighboring nodes to update its task offloading strategy.
% as a task receiver or task offloader, each edge node conducts multiple rounds of local communication with its predecessor or successors to updates its task offloading strategy.
% Specifically, all ESs execute the Task Receiver Algorithm, while the ESs not in $S^{H}$ and all EDs execute the Task Offloader Algorithm.
In each round of communication, each successor node $e^{h+1}_{j}$ receives Resource-Utilization-Request (RUR) messages from its predecessors in $V^{h+1}_{j}$. 
The RUR message from the predecessor $e^{h}_{i}$ includes the required computing resources on $e^{h+1}_{j}$ for $e^{h}_{i}$, denoted as $\xi^{h}_{i,j}$.
Based on this information, $e^{h+1}_{j}$ calculates the total required computing resources $\lambda^{h+1}_{j}$, and sends Resource-Utilization-Status (RUS) messages in response. 
The RUS message includes $\lambda^{h}_{j}$, $\mu^{h}_{j}$, $r^{h}_{i,j}$, the remaining completion time $\gamma^{h}_{j}$ and gradient information $rd^{h}_{j}$ (details in Section \ref{sec:alg}).
% Subsequently, each predecessor node $e^{h}_{i}$ updates its offloading strategy based on all RUS messages from its successors in $L^{h}_{i}$, and then sends RUR messages based on new offloading strategy to its successors in $L^{h}_{i}$. 
After receiving all RUS messages from its successors in $L^{h}_{i}$, each predecessor node $e^{h}_{i}$ updates its offloading strategy accordingly, and sends RUR messages based on new offloading strategy to its successors. 



% In the t-th round of communication, each predecessor $e^{h}_{i}$ sends Resource Utilization Request (RUR) messages to its successors in $L^{h}_{i}$, the RUR messages includes the computing resource requested $\xi^{h,(t)}_{i,j}$ by $e^{h}_{i}$ to $e^{h+1}_{j}$, where $\xi^{h,(t)}_{i,j} = p^{h, (t)}_{i,j} \phi^{h}_{i} I_{h}(C) \alpha_{h+1}$, and $p^{h, (t)}_{i,j}$ represents the task offloading strategy of $e^{h}_{i}$ in round t.
% After each task receiver $e^{h}_{j}$ receives the RUR messages from all edge nodes in $V^{h}_{j}$, it calculates the total computing resource required $\lambda^{h,(t)}_{j}$ and sends Resource Utilization Status (RUS) messages in response. 
% The RUS message includes $\lambda^{h,(t)}_{j}$, $\mu^{h}_{j}$, $r^{h}_{i,j}$, the remaining completion time $\gamma^{h,(t)}_{j}$ and gradient information $rd^{h,(t)}_{j}$ (details in Section \ref{sec:alg}).
% After receiving RUS messages from all task receiver in $L^{h}_{i}$, each task offloader $e^{h}_{i}$ updates its offloading strategy according to these messages and start a new round of communication. 


This iterative process continues until the task offloading strategy converges. 
Upon convergence, the predecessor node terminates the update of the strategy and sends the END message to its successors, which will forward this message to a proxy edge node.
The END message includes the total computing resources required by the edge node and its maximum computing resources.
% Until the task offloading strategy converges, $e^{h}_{i}$ broadcasts the END message and terminate the update of task offloading strategy.
After the proxy edge node collects the END messages of all edge nodes, it selects and broadcasts a new confidence threshold to balance the task response delay and inference accuracy, and then initiates the task offloading phase.

\begin{figure}[!t]
	\centering
	\includegraphics[width=0.90\linewidth]{./fig2/system process (2).png}
	\caption{\label{fig:sysprocess} Algorithm overview.}
\end{figure}

% In the update phase of the task offloading strategy, all ESs execute the Task Receiver Algorithm, while all EDs and ESs not in $S^{K}$ execute the Task Offloader Algorithm.
% The update of the task offloading strategy requires multiple rounds of communication between the task offloader and the task receiver.
% In the t-th round, any task offloader $e^{h}_{i}$ sends Resource Utilization Request (RUR) messages to all task receiver in $L^{h}_{i}$ based on its task offloading strategy $p^{h, (t)}_{i}$, the RUR messages represents the requested computing resources in the t-th round $\xi^{h,(t)}_{i,j}$, where $\xi^{h,(t)}_{i,j} = p^{h, (t)}_{i,j} \phi^{h}_{i} I_{k}(C) \alpha_{k+1}$. 
% After receiving resource request messages from all edge nodes in $V^{h}_{j}$, the task receiver $e^{h}_{j}$ estimates the total computing resources required, and send Resource Utilization Status (RUS) messages in response. 
% After receiving RUS messages from all task receiver in $L^{h}_{i}$, the task offloader $e^{h}_{i}$ updates its offloading strategy according to these messages and start a new round of communication. 
% Until the task offloading strategy converges, $e^{h}_{i}$ broadcasts the END message to conclude the update phase of the task offloading strategy.

% After the task offload strategy update phase, the system needs to evaluate the treadoff of response delay and inference precision. 
% We elect a proxy ES in $S^{1}$ for the configuration update of the confidence threshold.
% The proxy ES gathers the resource utilization status information of all ESs, selects and broadcast the best confidence threshold configuration based on the evaluation function of response delay and inference accuracy. 
% If the confidence threshold remains unchanged, the configuration update phase ends and the task offloading phase starts. Otherwise, a new task offloading strategy update phase starts.


%As task receivers, all ESs execute the DTO-R algorithm (introduced in Section \ref{section:DTO-R}).
%$p^{(t)}_{i,\cdot}$ represents the task offloading strategy of edge node $e_{i}$ in the $t$-th round. In the $t$-th round, the ES $e_{j}$ receives the resource utilization request (RUR) message from each edge node $e_{i}\in L_{j}$.
%The RUR message includes $\xi^{(t)}_{i,j}$, $\xi^{(t)}_{i,j}=p^{(t)}_{i,j}\phi_{i}I_{i}\alpha_{j}$, which is the computing resource requested by $e_{i}$ from ES $e_{j}$.
%The ES $e_{j}$ estimates the total computing resources required $\lambda^{(t)}$ for $t$-th round by receiving all RUR messages.
%In addition, the ES $e_{j}$ in $S^{1}$ estimates the uplink transmission rate from ED $e_{i}$ to $e_{j}$.
%Then each ES $e_{j}$ broadcasts its resource utilization status (RUS) message, which contains $\lambda^{(t)}$, $\mu_{j}$, $r_{i,j}$, etc. Note that these resource information are not the actual data of the ES, but the estimated value based on the request messages received by the ES in $t$-th round.
%
%As task offloaders, all EDs and some ESs execute the DTO-O algorithm (introduced in Section \ref{section:DTO-O}).
%For each edge node $e_{i}$, its offloading strategy in the $t$-th round is expressed as $p^{(t)}_{i,\cdot} = \{p^{(t)}_{i,j} | ej \in L_{i}$.
%After receiving the RUS message from the ES in $L_{i}$, $e_{i}$ makes a new offloading strategy $p^{(t+1)}_{i,\cdot}$ based on these messages.
%Then $e_{i}$ sends a RUR message to each ES $e_{j} \in L_{i}$.
%The edge node updates its task offloading strategy through multiple iterations.
%When the edge node $e_{i}$ obtains a convergent task offloading strategy, then the task offloader algorithm terminates, and $e_{i}$ sends END message to the ESs in $L_{i}$ and starts the task offloading phase. 



% The system workflow is illustrated in Fig. \ref{fig:sysprocess}. We divide the system timeline into fixed-length time slots, each comprising a configuration update phase and a task offloading phase.
% Unlike current algorithms that maintain a static offloading strategy over a long time slot\cite{chen2018computation}, our approach updates the task offloading strategy and confidence threshold every few seconds, enhancing adaptability to dynamic edge environments.


% The configuration update phase is responsible for determining the task offloading strategy and confidence threshold, which are used during the task offloading phase.
% Specifically, during the configuration update phase, as a predecessor or successor, each edge node conducts multiple rounds of local communication with its neighboring nodes to update its task offloading strategy.
% % as a task receiver or task offloader, each edge node conducts multiple rounds of local communication with its predecessor or successors to updates its task offloading strategy.
% % Specifically, all ESs execute the Task Receiver Algorithm, while the ESs not in $S^{H}$ and all EDs execute the Task Offloader Algorithm.
% In each round of communication, each successor node $e^{h+1}_{j}$ receives Resource-Utilization-Request (RUR) messages from its predecessors in $V^{h+1}_{j}$. 
% The RUR message from the predecessor $e^{h}_{i}$ includes the required computing resources on $e^{h+1}_{j}$ for $e^{h}_{i}$, denoted as $\xi^{h}_{i,j}$.
% Based on this information, $e^{h+1}_{j}$ calculates the total required computing resources $\lambda^{h+1}_{j}$, and sends Resource-Utilization-Status (RUS) messages in response. 
% The RUS message includes $\lambda^{h}_{j}$, $\mu^{h}_{j}$, $r^{h}_{i,j}$, the remaining completion time $\gamma^{h}_{j}$ and gradient information $rd^{h}_{j}$ (details in Section \ref{sec:alg}).
% % Subsequently, each predecessor node $e^{h}_{i}$ updates its offloading strategy based on all RUS messages from its successors in $L^{h}_{i}$, and then sends RUR messages based on new offloading strategy to its successors in $L^{h}_{i}$. 
% After receiving all RUS messages from its successors in $L^{h}_{i}$, each predecessor node $e^{h}_{i}$ updates its offloading strategy accordingly, and sends RUR messages based on new offloading strategy to its successors. 


\subsection{Problem Definition}
We divide the system timeline into fixed-length time slots (\eg, 5s), each comprising a configuration update phase and a task offloading phase.
During the configuration update phase, we need to jointly optimize the task offloading strategy and the confidence threshold, based on which to achieve the trade-off between average response delay and inference accuracy during the task offloading phase. 
% The configuration update phase is responsible for determining the task offloading strategy and confidence threshold, which are used during the task offloading phase.


% By jointly optimizing the task offloading strategy and the confidence threshold, we aim to strike a balance between the average response delay and the inference accuracy of tasks in the collaborative inference framework. 


The average response delay of tasks consists of the average offloading delays of $H$ subtasks, with $T^{h}$ representing the delay of $h$-th subtask.
% Each subtask's offloading delay includes transmission and computing delays denoted as $T^{h}$ for the average offloading delay of the $h$-th subtask.
We use $T^{h}_{i}$ to represent the average offloading delay of the $h$-th subtask at edge node $e^{h}_{i}$.
\begin{equation}
	T^{h} = \sum_{e^{h}_{i}\in S \cup D}\frac{\phi^{h}_{i}}{\Phi} T^{h}_{i},h=0,1,...H-1
\end{equation}
\begin{equation}
	T^{h}_{i} = \sum_{e^{h+1}_{j}\in L^{h}_{i}} p^{h}_{i,j} (T^{cm,h}_{i,j} + T^{cp,h+1}_{j})
\end{equation}


% The average response delay of tasks is influenced by the task offloading strategy and the configuration of the confidence threshold. 
% Throughout the entire process from task arrival at an ED to obtaining the inference results, each task passes through $K$ ESs at most, corresponding to K sub-models. 
% This process can be considered as $K$ instances of task offloading process, with each instances involving data transmission delay and computation delay
% We use $T^{k}$ to represent the average delay of the $k$-th task offloading process, and we use $T^{k}_{i}$ to represent the estimate task offloading delay of edge node $e^{k}_{i}$.
% \begin{equation}
% 	U(T,Acc) = \frac{\sqrt{T^2 + a^2}}{(Acc - Acc_{min})/(Acc_{max} - Acc_{min})}
% \end{equation}

To trade off the average response delay $T$ and inference accuracy $\mathcal{A}$, we introduce a utility function $U(T,\mathcal{A})$ to evaluate system performance:
\begin{equation}
	U(T,\mathcal{A}) = \frac{\sqrt{T^2 + a^2}}{(\mathcal{A} - \mathcal{A}_{min})/(\mathcal{A}_{max} - \mathcal{A}_{min})}
\end{equation}
where $a$ is a weight coefficient used to balance delay and inference accuracy, and the denominator is the normalized representation of accuracy.
When $a=0$, this utility function indicates that we should employ a new configuration, which reduces the delay by a greater proportion than the accuracy.
Additionally, setting a larger value of $a$ motivates the pursuit of higher accuracy when the delay is small.
% $\mathcal{A}_{max}$ and $\mathcal{A}_{min}$ denote the highest and lowest achievable inference accuracies, respectively, generally corresponding to scenarios where all tasks remain and all exit at the earliest branch, respectively.
We need to minimize the utility function $U$ of the system while satisfying the resource constraints, the question can be formalized as follows:
\begin{equation}
	(P1):\min\limits_{P,C} U(\sum_{h=0}^{H-1} T^{h},\mathcal{A}(C))
    \label{funU}
\end{equation}

$$ s.t.\left\{
\begin{aligned}
	% &T^{h}_{i} \!=\!\!\!\!\!\sum_{e^{h+1}_{j}\in L^{h}_{i}}\!\!\!\! p^{h}_{i,j} (T^{cm,h}_{i,j}\!\!+  T^{cp,h+1}_{j}),\!\!\!\!\!\!\! &\forall e^{h}_{i} \in S\cup D\\
	% &E^{0}_{i} < E_{i}^{0,max},  &\forall  e^{0}_{i} \in D\\
	&\lambda^{h}_{j} < \mu^{h}_{j},  &\forall  e^{h}_{j} \in S\\
	&\sum_{e^{h+1}_{j} \in L^{h}_{i}} p^{h}_{i,j} = 1, &\forall  e^{h}_{i} \in S\cup D\\
	&0 \leq p^{h}_{i,j} \leq 1, &\forall  e^{h}_{i}, e^{h+1}_{j} \in S\cup D
\end{aligned}
\right.
$$
% The first equation models the average delay for each edge node $e^{h}_{i}$ to offload subtasks, encompassing both transmission and computing delays. 
% The second inequality represents the energy consumption limit for each ED, stipulating that the transmission energy consumption per unit time generated by ED must be less than its energy consumption threshold. 
The first set of inequalities ensures that the total computing requirement on each ES should not exceed its maximum computing capacity. 
% The first inequality sets the constraint on the computing resources of each ES, ensuring that the total required computing resources should not exceed the maximum computing resources. 
The last two conditions ensure that each task can be successfully offloaded to one and only one ES.
% on the task offloading strategy for each edge node, ensuring that every task can be successfully offloaded.




==> content/ack.tex <==
This article is supported in part by the National Key Research and Development Program of China (Grant No. 2021YFB3301501); in part by the National Science Foundation of China (NSFC) under Grants 62132019, 62102391 and 61936015; in part by the Jiangsu Province Science Foundation for Youths (Grant No. BK20210122).

==> content/algorithm.tex <==

\begin{figure}[!t]
	\centering
	\includegraphics[width=0.90\linewidth]{./fig2/system process (2).png}
	\caption{\label{fig:sysprocess} Algorithm overview.}
\end{figure}

We first present an overview of the algorithm, as shown in Fig. \ref{fig:sysprocess}.
During the configuration update phase, each edge node, as a task offloader or a task receiver, conducts multiple rounds of local communication with its neighboring nodes to update its task offloading strategy under fixed confidence thresholds.
In each communication round, offloaders send Resource-Utilization-Request (RUR) messages to their respective receivers, who then respond with Resource-Utilization-Status (RUS) messages.
Based on the RUR messages received from the receivers, each offloader updates its task offloading strategy for the next round.
% Each offloader updates its task offloading strategy according to the RUR messages received  from its receivers and then starts the next round of communication.
This iterative process continues until the task offloading strategy converges, then each offloader broadcasts END messages, which will be gathered by a proxy edge node to determine a new confidence threshold.



% In this section, we demonstrate an efficient task offloading approach for the optimization problem \textbf{(P1)}.
% By jointly optimizing the task offloading strategy and the confidence threshold, we aim to achieve the promising trade-off between response delay and inference accuracy, thereby minimizing the objective function.
% \textbf{(P1)} is classified as a Mixed Integer Nonlinear Programming (MINP) problem due to the discrete nature of the confidence threshold.
% % The optimization problem in (\ref{funU}) is a Mixed Integer Nonlinear Programming (MINP) problem.
% To effectively tackle this complexity, we decompose the complex problem into two sub-problems:
% \begin{itemize}
%     \item [1).]Task Offloading Strategy Optimization Problem: With a fixed confidence threshold, \textbf{(P1)} simplifies to a convex optimization problem focusing on task offloading strategy. 
%     the main challenge here is using local information to derive the optimal solution $P$.
%     \item [2).]Confidence Threshold Optimization Problem: Given a task offloading strategy $P$, this sub-problem becomes an integer programming problem involving the confidence threshold $C$. 
%     The difficulties in this sub-problem include quickly evaluating the impact of different threshold settings on inference accuracy, and preventing the solution from settling into local optima.
%     % However, because the confidence threshold and the task offloading strategy are coupled, optimizing the confidence threshold $C$ may cause $P$ to no longer be the optimal solution of the task offloading strategy in the original problem.
% \end{itemize}

Next, we present the specific details of the algorithm. 
We first transform the problem by exterior-point method (Sec. \ref{Problem Transformation}). Then we introduce the DTO-R (Sec. \ref{section:DTO-R}) algorithm performed by each task receiver and the DTO-O algorithm (Sec. \ref{section:DTO-O}) performed by each task offloader, followed by the DTO-EE algorithm (Sec. \ref{section:DTO-EE}) for deriving the confidence threshold. Finally, we prove the convergence for DTO algorithm in Sec. \ref{sec:analysis}.



% \subsection{Task Offloading Strategy Optimization}


% This section introduces the task offloading strategy optimization problem with a fixed confidence threshold. 
% We begin by transforming the original problem, followed by the introduction of our distributed task offloading algorithm (DTO), which comprises the task offloader algorithm (DTO-offloader) and the task receiver algorithm (DTO-receiver). 
% Finally, we prove the convergence of the algorithm.

\subsection{Problem Transformation}\label{Problem Transformation}

%layer 不太好，需要改一下 第k次卸载
%We regard the set of all EDs as $S^{0}$, which is the 0th layer in the network, and the ESs in $S^{h}$ are regarded as the kth layer. Formula (11) presents a problem of minimizing the average offloading time of multiple layers, where $T^{h}$ represents the average local offloading time from the layer k to layer k+1.
%We find that only updating the task offloading strategy of the edge nodes in layer k does not change the average delay of task offloading from layer 0 to layer k-1, because the load of ESs in and before layer k does not change.
%On the contrary, changing the task offloading strategy of edge nodes in layer k will not only affect their own local offloading time, but also change the load of ESs behind layer k.
%
%For the edge nodes of each layer, just minimizing their average local offloading time can not optimize the average response delay of the task.
%Because there may be some edge nodes, their own resources are rich but their subsequent ESs are scarce, which makes the response delay of the task still high.
%Therefore, the optimization of task offloading strategy needs to consider not only the local offloading time of the task, but also the remaining completion time after the local offloading, which represents the time after the inference is completed until the inference result is obtained.
%We use $\gamma_{i}$ to represent the remaining completion time after the task completes inference on the ES $e_{i}$. The remaining completion time of each edge ndoe can be calculated by the following formula:
%\begin{equation}
%	\gamma_{i} = \sum_{e_{j} \in L_{i}}p_{i,j}(T^{cm}_{i,j} + T^{q}_{j} + T^{cp}_{j} + I_{j} \gamma_{j})
%	\label{newgamma}
%\end{equation}
%In particular, for the ES $e_{j}$ in $S^{H}$, because its output is the final inference result, its remaining completion time $\gamma_{j}$ is 0.
%In addition, we also need to consider the robustness of the delay of each ES, which is represented by the magnitude of the delay as the load changes. 
%We use $rd_{i}$ to represent the robustness of the delay of edge node $e_{i}$ to the load:
%\begin{equation}
%	rd_{i} = \frac{\alpha_{i}}{2(\mu_{i}-\lambda_{i})^{2}} + I_{i} \sum_{e_{j} \in L_{i}}p_{i,j}^{2} rd_{j}
%	\label{newrd}
%\end{equation}
%
%
%From the formulas (\ref{newphi}) and (\ref{newgamma}), we know that the average remaining completion time of the k-th layer edge node is equivalent to the local offloading time from the k-th layer to the K-1 layer, $\ie$
%\begin{equation}
%	\sum\limits_{e_{i}\in S^{h}} \frac{\phi_{i}}{\Phi} \gamma_{i} = \sum_{h}^{H-1} T^{h}
%\end{equation}
%Since the offloading strategy of the edge node in layer k does not change the average offloading delay from layer 0 to layer k-1, for the edge node in layer k, minimizing the average response delay of the task is equivalent to minimizing the average remaining completion time of layer k.





%From formula (5), we know that in the stationary state of the system, the task arrival rate $\Phi_{i}$ of ES $s_{i}$ depends on the offloading decision of nodes in $V_{i}$. The $\Phi_{i}$ of any ES $s_{i}$ is also optimal when the offload decisions of all the edge mobile devices and all the ESs optimal. 
%The sum of the transfer delay, queuing delay and computing delay in the process of offloading task to the next ES is regarded as the local offloading delay.
%For each edge mobile device $d_{m}$ or ES $e_{i}$, just minimizing the local offload delay does not minimize the response delay of the entire system, because an offload decision that minimizes the local offloading delay does not make $\Phi_{j}$ of next ES $s_{j}$ in $L_{m}$ or $L_{i}$ optimal.
%Therefore, the optimal offloading decision needs to consider not only the transmission delay, queuing delay and calculation delay during the local offloading process, but also needs to consider how long it will take from the completion of the calculation of the ES to the completion of all the reasoning of the task.
%%%%例子
%Therefore, we also need to introduce a variable $\gamma$ and $rd$, which represents the remaining completion time and the gradient information of the ES, respectively. The remaining completion time $\gamma_{i}$ represents the time from the completion of inference calculation on the ES $s_{i}$ to the final inference result of the task. The remaining completion time of each ES can be calculated by the following formula:
%\begin{equation}
%	\gamma_{i} = \sum_{s_{j} \in L_{i}}p_{i,j}(T^{cm}_{i,j} + T^{q}_{j} + T^{cp}_{j} + I_{j} \gamma_{j})
%\end{equation}
%for any ES $s_{i}$,The remaining completion time $r_{i}$ includes the local offloading delay and the remaining completion time of the ES $s_{j}$ in $L_{i}$. In particular, for any ESs $s_{j}$ in $S^{H}$, $r_{j}=0$.
%%%%rd解释
%\begin{equation}
%	rd_{i} = \frac{\theta_{i} \alpha_{i}}{2(\mu_{i}-\lambda_{i})^{2}} + I_{i} \sum_{s_{j} \in L_{i}}p_{i,j}^{2} rd_{j}
%\end{equation}

% Each edge node first optimizes the task offloading strategy with fixed confidence thresholds.
Each time slot is configured with fixed confidence thresholds, and each edge node first optimizes the task offloading strategy under the confidence thresholds of the previous time slot. 
% in a distributed manner 
To facilitate the analysis of distributed algorithms, we transform the constraints of the problem \textbf{(P1)} into its optimization objective by the exterior-point method. 
Such that we can deal with the problem whose solution may exceed the feasible region.
Specifically, we define the penalty function $N(P)$ as follows:
% This method allows us to consider solutions that may initially fall outside the feasible domain by incorporating a penalty function for constraint violations. 
% We define the penalty function $N(P)$ as follows:
% \begin{equation}
% 	\begin{aligned}
% 	N(P) &= C \cdot [ \sum_{e^{0}_{i}\in D}(\max\{0, E^{0}_{i}-E_{i}^{0,max}\})^{2} \\
% 		 &+ \sum_{e^{h}_{j}\in S}(\max\{0,\lambda^{h}_{j}-\mu^{h}_{j} \})^{2} ]
% 	\end{aligned}
% \end{equation}
\begin{equation}
	\begin{aligned}
	N(P) = K \cdot \sum_{e^{h}_{j}\in S}(\max\{0,\lambda^{h}_{j}-\mu^{h}_{j} + \epsilon \})^{2} 
	\end{aligned}
\end{equation}
where $\epsilon$ is an arbitrarily small positive constant, and $K$ is a sufficiently large positive constant, called the penalty factor. 
By adding this penalty function to the objective function, we define a new objective function $R(P) = \sum_{h=0}^{H-1}T^{h}+N(P)$. 
With fixed confidence thresholds, the original problem is transformed into a new optimization problem:
\begin{equation}
	\textbf{(P2)}:\min\limits_{P} R(P)
\end{equation}
$$ s.t.\left\{
\begin{aligned}
	&0 \leq p^{h}_{i,j} \leq 1,      &\forall e^{h}_{i}\in S\cup D\\
	&\sum_{e^{h+1}_{j} \in L^{h}_{i}} p^{h}_{i,j} = 1, &\forall e^{h}_{i}\in S\cup D
\end{aligned}
\right.
$$
If the offloading strategy $P$ is not satisfied $\lambda^{h}_{j}<\mu^{h}_{j} - \epsilon$ for any node $e^{h}_{j}\in S$ (h\textgreater0), the value of $R(P)$ will be very large. 
Therefore, by setting a sufficiently large value for $K$, we can approximate the optimal solution for \textbf{(P1)} by solving \textbf{(P2)}.
The main challenge to obtain the optimal solution of \textbf{(P2)} is the incompleteness of information in distributed scenarios. 
% Since edge nodes lack real-time access to comprehensive information from other nodes, such as current resource usage or offloading strategy,
% It is difficult for a single node to consider the computing resource constraints when making its delay-optimal strategy. 
The offloading strategy made by a single node without the strategies of other nodes may violate the computing resource constraint.
% To address this problem, we propose DTO, a distributed algorithm that enables each node to independently derive an optimal task offloading strategy using only local information.


\subsection{Task Receiver Algorithm (DTO-R)}\label{section:DTO-R}
This section describes the task receiver algorithm DTO-R, which is executed by edge servers during the configuration update phase.
In each communication round, a receiver $e^{h}_{j}\in S$ collects RUR or END messages from its offloaders in $V^{h}_{j}$, estimates the total required computing resources $\lambda^{h}_{j}$, and responds with RUS messages.
An RUR message from the offloader $e^{h-1}_{i}$ includes the required computing resources on receiver $e^{h}_{j}$ for $e^{h-1}_{i}$, denoted as $\xi^{h-1}_{i,j}$, and the vector $\xi^{h-1}_{\cdot,j} = \{\xi^{h-1}_{i,j} | e^{h-1}_{i} \in V^{h}_{j}\}$ represents the received RURs on receiver $e^{h}_{j}$.
Additionally, if END messages are received, the receiver $e^{h}_{j}$ forwards them to the proxy edge node.
An RUS message includes $\lambda^{h}_{j}$, $\mu^{h}_{j}$, $r^{h}_{i,j}$ and the gradient information $rd^{h}_{j}$.

The gradient information $rd^{h}_{j}$ represents the rate of change of delay under the current load, which is used to guide the update direction of the task offloading strategy.
Note that the gradient information $rd^{h}_{j}$ is obtained when the node $e^{h}_{j}$ runs the Task Offloader Algorithm (DTO-O), and $rd^{H}_{j}=0$ for each node $e^{H}_{j} \in S^{H}$.
 Algorithm 1 formally describes the DTO-R algorithm.
For ease of description, we add $t$ to the upper-right corner of the variable to indicate the value of the variable at $t$-th communication round.

% An RUS message includes $\lambda^{h}_{j}$, $\mu^{h}_{j}$, $r^{h}_{i,j}$, the estimated remaining completion time $\gamma^{h}_{j}$ and gradient information $rd^{h}_{j}$.
% The vector $\xi^{h-1}_{\cdot,j} = \{\xi^{h-1}_{i,j} | e^{h-1}_{i} \in V^{h}_{j}\}$ represents the resource request information received by the $e^{h}_{j}$, and the total computing resource required by $e^{h}_{j}$ are calculated as follows:
% \begin{equation}
% 	\lambda^{h}_{j} = \sum_{e^{h-1}_{i} \in V^{h}_{j}} \xi^{h-1}_{i,j}\
%     \label{newlambda}
% \end{equation}

% To enable the system to efficiently offload multiple interdependent subtasks, the receiver $e^{h}_{j}$ estimates its remaining completion time $\gamma^{h}_{j}$ and gradient information $rd^{h}_{j}$.
% $\gamma^{h}_{j}$ represents the average remaining completion time after tasks have been inferred on receiver $e^{h}_{j}$, which is given by:
% \begin{equation}
% 	\gamma^{h}_{j} =\!\!\!\! \sum_{e^{h+1}_{k} \in L^{h}_{j}}\!\!\! p^{h}_{j,k}(T^{cm,h}_{j,k} + T^{cp,h+1}_{k} + I_{h+1} \gamma^{h+1}_{k})
% 	\label{newgamma}
% \end{equation}
% In particular, $\gamma^{H}_{j} = 0$ for each receiver $e^{H}_{j} \in S^{H}$, as its output is the final inference result.
% The gradient information $rd^{h}_{j}$ represents the rate of change of delay under the current load, which is used to guide the update direction of the task offloading strategy.
% Then, the gradient information $rd^{h}_{j}$ can be calculated as:
% \begin{equation}
% 	rd^{h}_{j} = \frac{\partial (T^{cp,h}_{j} \!\!+ I_{h}\gamma^{h}_{j})}{\partial \phi^{h}_{j}} = \frac{\alpha_{h}^2}{(\mu^{h}_{j}-\lambda^{h}_{j})^{2}} +\!\!\!\! \sum_{e^{h+1}_{k} \in L^{h}_{j}}\!\!\!\!(p^{h}_{j,k} I_{h})^{2} rd^{h+1}_{k}
% 	\label{newrd}
% \end{equation}
% Note that $\gamma^{h+1}_{k}$ and $rd^{h+1}_{k}$ are obtained from RUS messages when $e^{h}_{j}$ runs the task offloader algorithm.
% Algorithm 1 formally describes the DTO-R algorithm.
% For ease of description, we add $t$ to the upper-right corner of the variable to indicate the value of the variable at $t$-th communication round.

% The RUS messages sent by $e^{h}_{j}$ includes the estimated total computing resources required $\lambda^{h}_{j}$, remaining completion time $\gamma^{h}_{j}$, growth rate of delay to load $rd^{h}_{i}$, transfer rate $r^{h-1}_{i,j}$, and maximum computing resources $\mu^{h}_{j}$.

% RUS messages are used to update the task offloading strategy of the task offloader. 
% For ease of description, we add $t$ to the upper-right corner of the variable to indicate the value of the variable at $t$-th round.
% The vector $\xi^{h-1,t}_{\cdot,j} = \{\xi^{h-1,t}_{i,j} | e^{h-1}_{i} \in V^{h}_{j}\}$ represents the RUR information received by the ES $e^{h}_{j}$ at $t$-th round.
% The total computing resource required by $e^{h}_{j}$ in $t$-th round is $\lambda^{h,t}_{j} = \sum_{e^{h-1}_{i} \in V^{h}_{j}} \xi^{h-1,t}_{i,j}$.
% Due to model partitioning, for any $e^{h}_{i} \notin S^{H}$, the task from the end of the inference on $e^{h}$ to the completion of the entire inference process still takes some time.
% We use $\gamma^{h}_{i}$ to represent the remaining completion time after the task completes inference on the ES $e^{h}_{i}$. 
% The remaining completion time of each edge node can be calculated by the following formula:
% \begin{equation}
% 	\gamma^{h}_{i} =\!\!\!\! \sum_{e^{h+1}_{j} \in L^{h}_{i}}\!\!\! p^{h}_{i,j}(T^{cm,h}_{i,j} + T^{cp,k+1}_{j} + I_{h+1} \gamma^{h+1}_{j})
% 	\label{newgamma}
% \end{equation}
% In particular, for ES $e^{H}_{i}$ in $S^{H}$, because its output is the final inference result, its remaining completion time $\gamma^{H}_{i} = 0$.
% In addition, we also need to consider the growth rate of delay as the load changes $rd^{h}_{i}$ of ES $e^{h}_{i}$, which is represented by The delay change caused by changing one unit of load.
% \begin{equation}
% 	rd^{h}_{i} = \frac{\alpha_{h}}{(\mu^{h}_{i}-\lambda^{h}_{i})^{2}} + \sum_{e^{h+1}_{j} \in L^{h}_{i}}(p^{h}_{i,j} I_{h})^{2} rd^{h+1}_{j}
% 	\label{newrd}
% \end{equation}
% The ES $s^{h}_{i} \notin S^{H}$ will execute both the task offloader algorithm and task receiver algorithm during the task offloading update phase, the $\gamma^{h}_{i}$ and $rd^{h}_{i}$ will be updated continuously in the algorithm (introduced in Section 3.3).
% If the ES $e^{h}_{j}$ receives the END message from $e^{h-1}_{i}$ in $t$-th round, it means that $e^{h-1}_{i}$ has obtained its final offloading strategy and starts the task offloading phase, $e^{h}_{j}$ sets $\xi^{h-1,(t')}_{i,j}=\xi^{h-1,t}_{i,j}, \forall t'>t$.
% Algorithm 1 formally describes DTO-Receiver.
\begin{algorithm}[!t]
	\caption{Task Receiver Algorithm (DTO-R) for $e^{h}_{j}$} \label{TRA} 
	\begin{algorithmic}%[1]
%		\REQUIRE $e^{h}_{j}$,$V^{h}_{j}$ 
%		\ENSURE $y = x^n$ 
		\State $t = 0$ 
		\While{$true$} 
		\State Receive RUR/END from $V^{h}_{j}$ to get $\xi_{\cdot,j}^{h-1,t}$
        \State Forward END to the proxy edge node
        \State Get $rd^{h,t}_{j}$\! from Task Offloader Algorithm
        % \State Get \!$\gamma^{h+1,t}_{k}$ \!\!and $rd^{h+1,t}_{k}$\!\! from Task Offloader Algorithm
        \State Calculate $\lambda_{j}^{h,t}$ by Eq. (\ref{newlambda})
        % \State Calculate $\gamma^{h,t}_{j}$ by Eq. (\ref{newgamma})
        % \State Calculate $rd^{h,t}_{j}$ by Eq. (\ref{newrd})
%		\IF{$s_{j} \in S^{1}$}
%		\State measure the received power of the edge mobile devices in $V_{j}$
%		\ENDIF
		% \State $\lambda_{j}^{h,t} = \sum_{e^{h-1}_{i} \in V^{h}_{j}} \xi_{\cdot,j}^{h-1,t}$
  %       \State $\gamma^{h,t}_{j} =\!\! \sum_{e^{h+1}_{k} \in L^{h}_{j}}\! p^{h}_{j,k}(T^{cm,h}_{j,k} + T^{cp,h+1}_{k} + I_{h+1} \gamma^{h+1}_{k}) $
 	% 	%\State $\phi_{j} = \lambda_{j}^{t} / \aleph_{j}$
		% \State $\gamma^{h,t}_{j}$, $rd^{h,t}_{j}$ $\gets$ synchronizes from Task Offloader Algorithm
		% \If{$e^{h}_{j} \in S^{1}$}
		% \For{each $e^{0}_{i}$ in $V^{1}_{j}$}
		% \State Measure the transmission power of $e^{0}_{i}$
		% \State $r_{i,j}^{0} = B log_{2}(1+\frac{\eta_{i}g_{i,j}}{\sigma^2+\sum_{e^{0}_{i'}\in V^{1}_{j}\backslash \{ e^{0}_{i}\} }\eta_{i'}g_{i',j}})	$
		% \EndFor
		% \EndIf
        \State Broadcast RUS including $\lambda_{j}^{h,t}, rd_{j}^{h,t}, \mu^{h}_{j}, r^{h}_{i,j}$ to $V^{h}_{j}$
		% \State Broadcast RUS including $\lambda_{j}^{h,t},\gamma_{j}^{h,t},rd_{j}^{h,t}, \mu^{h}_{j}$ to $V^{h}_{j}$
		\State $t=t+1$ 
		\EndWhile 
	\end{algorithmic} 
\end{algorithm}

\subsection{Task Offloader Algorithm (DTO-O)}\label{section:DTO-O}
This section describes the task offloader algorithm DTO-O, which is executed by all edge nodes not in $S^{H}$ during the configuration update phase.
% We first introduce the initialization and termination conditions of the algorithm.
At the beginning of the algorithm, each offloader $e^{h}_{i} \in D\cup S/S^{H}$ initializes its task offloading strategy, $\ie$,  $p^{h,(0)}_{i,j} = 1/|L^{h}_{i}|, \forall e^{h+1}_{j}\in L^{h}_{i}$. %\in D\cup S/S^{H}
Then it sends the initialized RUR messages containing $\xi^{h,(0)}_{i,j} = p^{h,(0)}_{i,j}\phi^{h}_{i}I_{h}\alpha_{h+1}$ to each receiver $e^{h+1}_{j} \in L^{h}_{i}$.

In the subsequent $t$-th round, $e^{h}_{i}$ receives the RUS message from each receiver $e^{h+1}_{j} \in L^{h}_{i}$, which includes $\lambda_{j}^{h+1,t}$,$\gamma_{j}^{h+1,t}$, $rd_{j}^{h+1,t}$ and $\mu^{h+1}_{j}$.
% of each edge node $e^{h+1}_{j}$.
Based on this information, $e^{h}_{i}$ calculates its remaining completion time $\gamma^{h,t}_{i}$, and detects the following conditions:
\begin{subequations}
	%\left\{
	\begin{align}
		&\lambda^{h+1,t}_{j} < \mu^{h+1}_{j} - \epsilon, \forall e^{h+1}_{j} \in L^{h}_{i}\label{Za}\\
		&\gamma_{i}^{h,t} \leq (1+\Psi)\gamma_{i}^{h,t-1}\label{Zb}
	\end{align}
	%\right.
    \label{endcondition}
\end{subequations}
The condition (\ref{Za}) indicates that if the total required computing resources on each receiver $e^{h+1}_{j} \in L^{h}_{i}$ exceeds its limit, $e^{h}_{i}$ will continue a new round of communication. 
The condition (\ref{Zb}) indicates that the remaining completion time difference between two successive iterations is small. 
If $e^{h}_{i}$ satisfies these conditions, it will terminate the update of task offloading strategy, and send END messages including the $\xi^{h,t+1}_{i,j}$, $\lambda^{h,t+1}_{i}$ and $\mu^{h}_{i}$ to the receivers in $L^{h}_{i}$.
% The END message includes the $\xi^{h,t+1}_{i,j}$, $\lambda^{h,t+1}_{i}$ and $\mu^{h}_{i}$.
Otherwise, it will get a new offloading strategy and send RUR messages to the receivers in $L^{h}_{i}$.

\begin{algorithm}[!t] 
	\caption{Task Offloader Algorithm (DTO-O) for $e^{h}_{i}$} 
	\label{DTO-O} 
	\begin{algorithmic}%[1]
		%\REQUIRE $n \geq 0 \vee x \neq 0$ 
		%\ENSURE $y = x^n$ 
%		\STATE Initialize $r_{i}^{(0)} = 0$
%		\STATE Initialize $rd_{i}^{(0)} = 0$
		\For{each $e^{h+1}_{j} \in L^{h}_{i}$}
		\State Initialize $p_{i,j}^{h,(0)} = 1/|L^{h}_{i}|$
		%%改
		\State Send RUR messages including $\xi_{i,j}^{h,(0)}$ to $e^{h+1}_{j}$
		\EndFor
		\State $t = 0$ 
		\While{$true$} 
		\State Receive RUS from $L^{h}_{i}$ to get $\lambda_{j}^{h+1,t}$, $\gamma_{j}^{h+1,t}$, $rd_{j}^{h+1,t}$, $\mu^{h+1}_{j}$ of each  $e^{h+1}_{j}$
		\State Calculate $\gamma^{h,t}_{j}$ by Eq. (\ref{newgamma})
		\If{t\textgreater0 and Conditions (\ref{endcondition}) are satisfied}
		\For{each $e^{h+1}_{j} \in L^{h}_{i}$} 
        \State $p^{h,t+1}_{i,j} = p_{i,j}^{h,t}$
 		\State Send END including $\xi^{h,t+1}_{i}$, $\lambda^{h,t+1}_{i}$, $\mu^{h,t+1}_{i}$ to $e^{h+1}_{j}$
		\EndFor
        \State Continue
		% \State Return $p^{h}_{i}, \gamma^{h,t}_{i}, rd^{h,t}_{i}$
		\EndIf
        \State Calculate $\Delta_{i,j}^{h,t}$ for each $e^{h+1}_{j} \in L^{h}_{i}$ by Eq. (\ref{Delta})
		\State Get new offloading strategy $p^{h,t+1}_{i,\cdot}$ by Eq. (\ref{newp})
		\For{each $e^{h+1}_{j} \in L^{h}_{i}$}
		\State $\xi_{i,j}^{h,t+1} = p_{i,j}^{h,t+1} \phi_{i} \alpha_{h+1}$
		\State Send RUR including $\xi_{i,j}^{h,t+1}$ to $e^{h+1}_{j}$
		\EndFor
		\State $t=t+1$ 
		\EndWhile
	\end{algorithmic} 
\end{algorithm}
The main idea of updating the offloading strategy is to increase the offloading probability of the most idle and promising receiver, which can offer the lowest offloading delay and remaining completion time.
We define $\Delta_{i,j}^{h,t}$ as the repulsive factor of $e^{h}_{i}$ to $e^{h+1}_{j}$ in $t$-th round.
\begin{equation}
	\begin{aligned}
        \Delta_{i,j}^{h,t} \!\!= & T^{cm,h,t}_{i,j} \!\!\!+\! T^{cp,h+1,t}_{j} \!\!\!+\! I_{h+1} \gamma^{h+1,t}_{j} \!\!\!+\! \phi^{h}_{i}  p^{h,t}_{i,j} I_{h} rd^{h+1,t}_{j} \\
		+ &2K \cdot \max\{0,\phi^{h}_{i} I_{h} \alpha_{h+1}(\lambda^{h+1,t}_{j}-\mu^{h+1}_{j}+\epsilon)\} %\tag*{}
		\label{Delta}
	\end{aligned}
\end{equation}
The offloaders tend to assign higher offloading probabilities to the receiver with lower deterrence factors (the reason is explained in Section \ref{sec:analysis}). 
Note that as long as $\lambda^{h+1,t}_{j} > \mu^{h+1}_{j}-\epsilon$, which means that the receiver $e^{h+1}_{j}$ is overloaded, $\Delta_{i,j}^{h,t}$ will be very large and $e^{h}_{i}$ will reduce the offloading probability of $e^{h+1,}_{j}$.
We define $e^{h+1}_{j^{*}}$ as the receiver in $L^{h}_{i}$ that minimizes the value of $\Delta_{i,j}^{h,t}$, and the new offloading strategy $p_{i,\cdot}^{h,t+1}$ for $e^{h}_{i}$ is given by:
\begin{equation}
	\left\{
	\begin{aligned}
		& p_{i,j}^{h,t+1} = (1-\tau) p_{i,j}^{h,t},     e^{h+1}_{j} \in L^{h}_{i}, j \neq j^{*}\\
		& p_{i,j^{*}}^{h,t+1} = p_{i,j^{*}}^{h,t} + \tau \sum\nolimits_{j\neq j^{*}}p_{i,j}^{h,t},    e^{h+1}_{j} \in L^{h}_{i}
	\end{aligned}
    \label{newp}
	\right.
\end{equation}
Where $\tau \in(0,1]$ is the step size, which determines the convergence speed.
Algorithm 2 formally describes DTO-O.





\begin{comment}
	

\subsection{Process of system}

In each time slot, the edge mobile device runs the resource request algorithm. The ES $s_{i}$ is a resource requester for $L_{i}$ and a task receiver for $V_{i}$, so it runs both the resource request algorithm and the task receiving algorithm.

We first introduce the initialization and termination conditions of the algorithm. At the beginning of the algorithm, the edge mobile device $d_{m}$ randomly selects an ES in $L_{m}$ as the target for task offloading, and the ES $s_{i}$ average its offloading probabilities, for each ES $s_{j} \in L_{i}$, $p_{i,j} = 1 / |L_{i}|$. 

We define a positive threshold $\Psi$, which determines the accuracy required when the algorithm terminates. Each ES $s_{i}$ detects the following two conditions:
\begin{equation}
	\left\{
	\begin{aligned}
		&\lambda_{j} < \mu_{j},  \forall s_{j} \in L_{i}\\
		&R_{i}^{t} \leq (1+\Psi)R_{i}^{t-1}\\
	\end{aligned}
	\right.
\end{equation}
Condition 1 means that as long as required computing resources on any ES $s_{j} \in L_{i}$ exceeds its limit, the iterative algorithm will continue to execute. The condition 2 indicates that the algorithm convergence can be judged when the performance difference between two successive iterations is very small. If the above two conditions are met, the iteration will terminate, otherwise it will start the next round of iteration to obtain a new round of offloading strategy.

$p^{t}$ and $a^{t}$ represent the offload decision of the ESs and edge mobile devices in the round t iteration, respectively. In round t iteration of the resource request algorithm, the edge mobile device $d_{m}$ or ES $s_{i}$ sends the resource request message (RRM) to the offload target ESs in $L_{m}$ and $L_{i}$ respectively. RRM includes the required resources $\xi^{t}$, for edge mobile devices $d_{m}$, RRM also includes $\eta_{m}$, $h_{m,j}$, and $\xi_{m,j}^{t}=a_{m,j}^{t}\phi_{m}\theta_{j}\alpha_{j}$, for ESs $s_{i}$, $\xi_{i,j}^{t} = p_{i,j}^{t}\Phi_{i}\theta_{j}\alpha_{j}$.

In the round t iteration of the task receiving algorithm, the ES receives the all the RRMs to obtain the total computing resources required, transmission rate, and estimate its remaining completion time. 
Then each ES $s_{j}$ broadcasts its resource status message (RSM) to the edge mobile devices or ESs in $V_{j}$. The RSM includes the total compute resources required $\lambda_{i}$, transmission rate $r^{d2s}_{m,j}$ or $r^{s2s}_{i,j}$, remaining completion time $r_{j}$, and gradient information $rd_{j}$. Note that the compute resources, remaining completion time and gradient information here are not the actual data of the ES, it is a numerical estimate based on the request message sent by the device at round t. After all RUSs is received by the edge mobile device or ES, the new offloading decisions are made based on this information.
In this way, edge mobile devices and ESs adjust their offload decisions through multiple iterations. When all nodes have reached a convergent unload decision, the algorithm terminates, nodes will send END message to the ESs.


\begin{algorithm} 
	\caption{Resource Request Algorithm for $s_{i}$} 
	\label{RRA} 
	\begin{algorithmic}
		%\REQUIRE $n \geq 0 \vee x \neq 0$ 
		%\ENSURE $y = x^n$ 
		\STATE Initialize $r_{i}^{(0)} = 0$
		\STATE Initialize $rd_{i}^{(0)} = 0$
		\FOR{each $s_{j} \in L_{i}$}
		\STATE Initialize $p_{i,j}^{(0)} = 1/|L_{i}|$
		%%改
		\STATE send RRM including $\xi_{i}^{(0)}$ to $s_{j}$
		\ENDFOR
		\STATE $t = 0$ 
		\WHILE{$true$} 
		\STATE receive $\lambda_{j}^{t},r_{j}^{t},rd_{j}^{t}$ from $L_{i}$
		\STATE $R_{i}^{t} \gets $
		\IF{t>0 and Condition (16) is true}
		\FOR{each $s_{j} \in L_{i}$}
		\STATE send END to $s_{j}$
		\STATE $p_{i,j} = p_{i,j}^{t}$
		\ENDFOR
		\STATE return $p_{i,\cdot}$
		\ENDIF
		\STATE $p_{i,\cdot}^{t+1} \gets$
		\STATE $r_{i}^{t+1} \gets$
		\STATE $rd_{i}^{t+1} \gets$
		\FOR{each $s_{j} \in L_{i}$}
		\STATE $\xi_{i,j}^{t+1} = p_{i,j}^{t+1}$
		\STATE send RRM including $\xi_{i,j}^{t+1}$
		\ENDFOR
		\STATE $t=t+1$ 
		\ENDWHILE
	\end{algorithmic} 
\end{algorithm}

The main idea of the offload strategy update algorithm is to simply increase the offload probability of the most idle ES, and then greedily reduce the offload probability of other ESs, thereby reducing the average response time. 
Therefore, we define $\Delta_{i,j}^{t}$ as the preference factor of ES $s_{i}$ to ES $s_{j}$ in round $t$.
\begin{equation}
	\begin{split}
		\Delta_{i,j}^{t}= 
		&\frac{\theta_{j} \beta_{j}}{r^{s2s}_{i,j}} + \frac{\lambda_{j}}{2\mu_{j}(\mu_{j}-\lambda_{j})} + \frac{\theta_{j} \alpha_{j}}{\mu_{j}} + I_{j} \gamma_{j} + p_{i,j} \Phi_{i} rd_{j}\\
		& +2C max\{0,\theta_{i}\alpha_{i}(\lambda_{j}-\mu_{j} + \epsilon)\}
	\end{split}
\end{equation}
The smaller the value of $\Delta_{i,j}^{t}$, the more biased ES $s_{i}$ is to assign a greater offload probability to $s_{j}$ in the next iteration.
Note that as long as $\lambda_{j} > \mu_{j}$, which means that the ES $s_{j}$ is overloaded, the value of $\Delta_{i,j}^{t}$ will be large, so $s_{i}$ will reduce the probability of offloading to $s_{j}$ in the next iteration.
We define $s_{j*}$ as the ES in $L{i}$ that minimizes the value of $\Delta_{i,j}^{t}$, then the new offloading strategy $p_{i,\cdot}^{t+1}$ is obtained by the following formula:
\begin{equation}
	\left\{
	\begin{aligned}
		& p_{i,j}^{t+1} = (1-\tau) p_{i,j}^{t},    &\forall s_{j} \in L_{i}, j \neq j^{*}\\
		& p_{i,j^{*}}^{t+1} = p_{i,j^{*}}^{t} + \tau \sum^{}_{j\neq j^{*}}p_{i,j}^{t},    &s_{j} \in S
	\end{aligned}
	\right.
\end{equation}
Where $\tau \in(0,1]$ is the step length, it can ensure that the formula can converge through iteration, and can also determine the convergence speed. The update algorithm is shown as follows:

\begin{algorithm} 
	\caption{Offloading Strategy Update Algorithm for $s_{i}$} 
	\label{OFUA} 
	\begin{algorithmic}
		%\REQUIRE $n \geq 0 \vee x \neq 0$ 
		%\ENSURE $y = x^n$ 
		\STATE Select the ES $s_{j*}$, satisfy $\Delta_{i,j*}^{t} = min{\Delta_{i,j}^{t}}_{s_{j}\in L_{i}}$
		\STATE Get the new offloading strategy $p_{i,\cdot}^{t+1}$ by formula (18).
		\STATE Get the new $gamma_{i}^{t+1}$ by formula (13).
		\STATE Get the new $rd_{i}^{t+1}$ by formula (14).
		
	\end{algorithmic} 
\end{algorithm}



\subsection{early exit}
The offloading strategy mentioned above is based on the average case of the early exit mechanism, as shown in formula 7, where the average number of tasks entered per batch of ES $s_{i}$ is $\theta_{i}$. In fact, for each ES with an early exit point, it has multiple early exit cases, and the number of early exit tasks per batch is not fixed. After passing the early exit point, if the number of tasks remaining is small, it requires less transmission delay and computation delay.

Therefore, we can design multiple offloading strategies for each ES with early exit point, corresponding to different early exit situations, and we can choose different offloading strategies for task offloading based on the actual situation of early exit. In the case of the most fine-grained offloading strategy, we divide the original single offloading strategy of each ES into $\theta_{0}$ offloading strategies, corresponding to the number of output tasks for each early exit situation. Similarly, $\gamma$ and $rd$ are also divided into $\theta_{0}$ species.
$p_{i} = \{p^{1}_{i},p^{2}_{i},...,p^{\theta_{0}}_{i}\}$, $\gamma_{i} = \{\gamma^{1}_{i},\gamma^{2}_{i},...,\gamma^{\theta_{0}}_{i}\}$, $rd_{i} = \{rd^{1}_{i},rd^{2}_{i},...,rd^{\theta_{0}}_{i}\}$

\begin{algorithm} 
	\caption{Fine-grand Offloading Strategy Update Algorithm for $s_{i}$} 
	\label{FOFUA} 
	\begin{algorithmic}
		%\REQUIRE $n \geq 0 \vee x \neq 0$ 
		%\ENSURE $y = x^n$ 
		\FOR{each $\theta$ in 1 to $\theta_{0}$}
			\STATE Select the ES $s_{j*}$, satisfy $\Delta_{i,j*}^{\thetat} = min{\Delta_{i,j}^{\thetat}}_{s_{j}\in L_{i}}$
			\STATE Get the new offloading strategy $p_{i,\cdot}^{\thetat+1}$ by formula (18).
			\STATE Get the new $\gamma_{i}^{\thetat+1}$ by formula (13).
			\STATE Get the new $rd_{i}^{\thetat+1}$ by formula (14).
		\ENDFOR
	\end{algorithmic} 
\end{algorithm}

\end{comment}

\subsection{Confidence Threshold Optimization}
To balance the response delay and inference accuracy, we adjust the confidence threshold after task offloading strategies of all edge nodes converge.
We select a proxy edge node $\hat{e}^{H}_{i} \in S^{H}$ to gather END messages from all edge nodes.
$\hat{e^{H}_{i}}$ evaluates the response delays and inference accuracy of various settings of confidence thresholds, and then selects an appropriate confidence threshold $C$ to broadcast to all edge nodes.
However, evaluating the inference accuracy across various settings of confidence thresholds can be very time-consuming. 
In addition, we must avoid inappropriate confidence thresholds that may result in the system being in a local optimum.
To address these challenges, we use a reuse-based evaluation method and a simulated annealing algorithm.

\subsubsection{Reuse-based Evaluation}
Given the extensive range of confidence threshold combinations, it is impractical to evaluate each combination individually.
Instead, we adopt a reuse-based method that can predetermine the outcomes for all confidence thresholds by a single evaluation. 
Specially, since the confidence threshold does not change the inference outputs of each branch, we use a verification dataset to evaluate the model without enabling the samples to exit early, and we capture the softmax outputs of all samples at each branch.
These outputs can be reused to screen out the samples that exit early with different settings of confidence thresholds.
In this way, we only need to evaluate the model once to obtain an accuracy-ratio table, which records the accuracy and exit ratio for each setting of confidence thresholds.



\subsubsection{Configuration Update}\label{section:DTO-EE}

\begin{algorithm}[!t] 
	\caption{DTO-EE} \label{cup} 
	\begin{algorithmic}
%		\REQUIRE $e^{h}_{j}$,$V^{h}_{j}$ 
%		\ENSURE $y = x^n$ 
		\State $\hat{e}^{H}_{i}$ receives END messages of all edge nodes
        \State Calculate the candidate confidence threshold $C$ that minimizes the utility function $U$
        \If{$random()>x$}
        \State Mutate the candidate confidence threshold $C$
        \EndIf
        \State $\hat{e}^{H}_{i}$ broadcasts $C$ to all edge nodes
        \State Record best confidence threshold $C^{*}$;
	\end{algorithmic} 
\end{algorithm}
After receiving all END messages, the proxy edge node $\hat{e}^{H}_{i}$ assesses the maximum and total required computing resources of each node.
$\hat{e}^{H}_{i}$ can select different confidence thresholds to scale the total required computing resources of each node, and the degree of scaling is related to the exit ratio.
Therefore, based on the accuracy-ratio table and the current task offloading strategy $P$, $\hat{e}^{H}_{i}$ calculates the candidate confidence threshold $C$ that minimizes the utility function $U$.
To escape potential local optima, we use simulated annealing to explore more efficient confidence thresholds.
Especially, $\hat{e}^{H}_{i}$ select the candidate confidence threshold $C=\{c_{h}|E_{h}=1\}$ with a certain probability, Otherwise mutate the candidate confidence threshold $C$, and randomly selects the confidence threshold of each branch in the range of $[c_{h}-\Delta c, c_{h}+\Delta c]$.
Algorithm 3 formally describes the configuration update phase.



\subsection{Convergence Analysis}\label{sec:analysis}
% In this section, we prove that the DTO algorithm enables the task offloading strategy to converge to the global optimum.
This section validates that the DTO algorithm ensures convergence of the task offloading strategy to an optimum.
We define $P^{t} = \{p^{h,t}_{i}|e^{h}_{i}\in S\cup D \}$ as the task offloading strategies of all edge nodes in the $t$-th round.
% The update process $\Gamma$ modifies $P^{t}$ each round, aiming for convergence when $P^{*} = \Gamma(P^{*})$, 
We use $\Gamma$ to represent the update process of the task offloading strategy each round.
% Define $p^{t,h} = {p^{t}_{i,j}|e_{i}\in S^{h},e_{j}\in S^{h+1}}$ as the task offload strategy for edge nodes in $S^{h}$ ($S^{0}$ represents the set of all EDs) at the $t$-th round. 
% After the edge nodes send RUR messages according to strategy $p^{t}$ and receive RUS messages from ESs, the edge nodes execute DTO-OU algorithm to get the $t+1$-th round offloading strategy $p^{t+1,h}$. 
% The transformation of strategy can be expressed as:
$$P^{t+1} = \Gamma(P^{t})$$
if $P^{*} = \Gamma(P^{*})$, $P^{*}$ is the fixed point of the update process. 
In $t$-th round, the objective function $R(P)$ can be regarded as a continuous function of $p^{h,t}_{i,j}$.

\begin{lemma}
	if $P^{t} \neq P^{*}$, the transformation $\Gamma$ gives a gradient descent direction of $R(P^{t})$ at point $P^{t}$, $\ie$,
	$$\langle\nabla R(P^{t}), \Gamma(P^{t}) - P^{t}\rangle \textless 0$$
	where $\nabla$ is the gradient operator, and $\langle a, b \rangle$ represents the inner product of vectors a and b.
\end{lemma}
\begin{proof}
	The partial derivative of $R(P^{t})$ with respect to $p_{i,j}^{h,t}$ is 
	\begin{equation}
		\begin{aligned}
			\hspace{-1mm}
			\!\!\frac{\partial R(P^{t})}{\partial p_{i,j}^{h,t}} = &\frac{\phi_{i}}{\Phi}[(T^{cm,h}_{i,j} \!\!+\! T^{cp,h+1}_{j} \!\!+\! I_{h+1}\gamma^{h+1}_{j}) \\
            &+ p_{i,j}^{h,t}\frac{\partial  (T^{cp,h+1}_{j} + \gamma^{h+1}_{j})}{\partial p_{i,j}^{h,t}} + \frac{\partial (N(P))}{\partial p_{i,j}^{h,t}}]\\
			% &= \frac{\phi_{i}}{\Phi}[(T^{cm}_{i,j} + T^{q}_{j} + T^{cp}_{j} + I_{j}r_{j}) + p_{i,j}^{t}\phi_{i}rd_{j}^{t}+\frac{\partial (N(p))}{\partial p_{i,j}^{t}}]\\
			=& \frac{\phi_{i}}{\Phi}\Delta_{i,j}^{h,t} \nonumber 
		\end{aligned}
	\end{equation}
	where $\Delta_{i,j}^{t}$ is defined in formula (\ref{Delta}), therefore,
	\begin{equation}
		\begin{aligned}
			&\langle\nabla R(P^{t}), \Gamma(P^{t}) - P^{t}\rangle \\
			&= \frac{1}{\Phi}\sum_{e^{h}_{i}\in S\cup D} \phi_{i} \sum_{e^{h+1}_{j}\in L^{h}_{i}}\Delta_{i,j}^{h,t}(p_{i,j}^{h,t+1}-p_{i,j}^{h,t}) \nonumber
		\end{aligned}
	\end{equation}
	
	
For edge node $e^{h}_{i}$, $e^{h+1}_{j^*}$ is the ES that minimizes $\Delta^{h}_{i,j}$, so for any $e^{h+1}_{j}\in L^{h}_{i}$, $\Delta_{i,j^*}^{h,t} \leq \Delta_{i,j}^{h,t}$
	\begin{equation}
		\begin{aligned}
			&\sum_{e^{h+1}_{j} \in L^{h}_{i}} \!\!\! \Delta_{i,j}^{h,t}p_{i,j}^{h,t+1} \!\!= 
			\Delta^{h,t}_{i,j^*}p_{i,j*}^{h,t+1}\!\! +\!\!\!\! \sum_{\substack{e^{h+1}_{j} \in L^{h}_{i}\\
            j\neq j^{*}}} \!\! \Delta_{i,j}^{h,t}p_{i,j}^{h,t+1}\\
			&=\Delta^{h,t}_{i,j^*}(p_{i,j*}^{h,t} \!\! + \tau \!\! \!\sum_{\substack{e^{h+1}_{j} \in L^{h}_{i}\\j\neq j^{*}}} \!\!p_{i,j}^{h,t} \!\!+\!\! \sum_{\substack{e^{h+1}_{j} \in L^{h}_{i}\\j\neq j^{*}}} \!\! \Delta_{i,j}^{h,t}(1-\tau)p_{i,j}^{h,t}\\
			&=\!\!\!\!\sum_{e^{h+1}_{j} \in L^{h}_{i}} \!\!\! \Delta_{i,j}^{h,t}p_{i,j}^{h,t} \!\!+\! \tau (\Delta_{i,j^*}^{h,t} \!\!\sum_{\substack{e^{h+1}_{j} \in L^{h}_{i}\\j\neq j^{*}}} \!\!\!\!\! p_{i,j}^{h,t} - \!\!\!\! \sum_{\substack{e^{h+1}_{j} \in L^{h}_{i}\\j\neq j^{*}}} \!\!\!\! \Delta_{i,j}^{h,t}p_{i,j}^{h,t})\\
			&\leq \sum_{e^{h+1}_{j} \in L^{h}_{i}}\Delta_{i,j}^{h,t}p_{i,j}^{h,t}	\nonumber 
		\end{aligned}	
	\end{equation}
$R(P^{t})$ is strictly convex, and since $P^{t} \neq P^{*}$, there is at least one node $e^{h+1}_{j}$ satisfying $\Delta^{h,t}_{i,j} \textgreater \Delta^{h,t}_{i,j*}$. therefore, $\sum_{e^{h+1}_{j} \in L^{h}_{i}}\Delta_{i,j}^{h,t}p_{i,j}^{h,t+1} \textless \sum_{e^{h+1}_{j} \in L^{h}_{i}}\Delta_{i,j}^{h,t}p_{i,j}^{h,t}$, and $\langle\nabla R(P), \Gamma(P^{t}) - P^{t}\rangle \textless 0$
\end{proof}









==> content/bio.tex <==

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.2in,clip,keepaspectratio]{bio/yangxu.png}}]
{Yang Xu}
(Member, IEEE) is currently an associate researcher in the School of Computer Science and Technology at University of Science and Technology of China. He got his Ph.D. degree in computer science and technology from University of Science and Technology of China in 2019. He got his B.S. degree in Wuhan University of Technology in 2014. His research interests include Ubiquitous Computing, Deep Learning and Mobile Edge Computing.
\end{IEEEbiography}
% \vspace{-0.25cm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/yunmingliao.jpg}}]
{Yunming Liao}
received B.S. degree in 2020 from  the University of Science and Technology of China.   He is currently pursuing his M.S. degree in the School of Computer Science and Technology, University of Science and Technology of China. His research interests include mobile edge computing and federated learning. 
\end{IEEEbiography}
% \vspace{-0.25cm}
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.2in,clip,keepaspectratio]{bio/honglixu.png}}]
{Hongli Xu}
(Member, IEEE) received the B.S. degree in computer science from the University of Science and Technology of China, China, in 2002, and the Ph. D degree in computer software and theory from the University of Science and Technology of China, China, in 2007. He is a professor with the School of Computer Science and Technology, University of Science and Technology of China, China. He was awarded the Outstanding Youth Science Foundation of NSFC, in 2018. He has won the best paper award or the best paper candidate in several famous conferences. He has published more than 100 papers in famous journals and conferences, including the IEEE/ACM Transactions on Networking, IEEE Transactions on Mobile Computing, IEEE Transactions on Parallel and Distributed Systems, Infocom and ICNP, etc. He has also held more than 30 patents. His main research interest is software defined networks, edge computing and Internet of Thing.
\end{IEEEbiography}
% \vspace{-0.25cm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/zhenguoma.jpg}}]
{Zhenguo Ma}
received the B.S. degree in software engineering from the Shandong University, China, in 2018. He is currently pursuing his Ph.D. degree in the School of Computer Science and Technology, University of Science and Technology of China. His research interests include edge computing and federated learning.
\end{IEEEbiography}
% \vspace{-0.25cm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.2in,clip,keepaspectratio]{bio/lunwang.png}}]
{Lun Wang}
received the B.S. degree in 2019 from the University of Electronic Science and Technology of China. He is currently pursuing his Ph.D. degree in the School of Computer Science and Technology, University of Science and Technology of China. His research interests include mobile edge computing and federated learning.
\end{IEEEbiography}
% \vspace{-0.25cm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/jianchunliu.jpg}}]
{Jianchun Liu} 
(Student Member, IEEE) received B.S. degree in 2017 from the North China Electric Power University. He is currently a Ph.D. candidate in the School of Data Science, University of Science and Technology of China (USTC). His main research interests are software defined networks, network function virtualization, edge computing and federated learning.
\end{IEEEbiography}

==> content/convergence.tex <==
In this section, we prove that the proposed algorithm will converge to a global optimal. 
Define $p^{(t)}_{i}$ as the task offload strategy for edge server $s_{i}$ at the round $t$ iteration. 
After the edge server $s_{i}$ send RRM messages according to strategy $p^{(t)}_{i}$ and receive RSM messages from edge servers in $L_{i}$, the edge server executes DTO-OU algorithm to get the $t+1$ round offloading strategy $p^{(t+1)}_{i}$. 
The transformation of strategy $p_{i}$ can be expressed as:
$$p^{(t+1)}_{i} = \Gamma(p^{(t)}_{i})$$
if $p^*_{i} = \Gamma(p^*_{i})$ for any edge server $s_{i}$, $p^*_{i}$ is the convergence point. 
In round $t$ iteration, the objective function $R_{i}(p_{i}^{(t)})$ of the edge server $s_{i}$ can be regarded as an N-dimensional function of $p$.

\begin{lemma}
	if $p_{i}^{(t)} \neq p_{i}^{*}$, the transformation $\Gamma$ gives a gradient descent direction of $R_{i}(p_{i}^{(t)})$ at $p_{i}^{(t)}$, i.e
	$$\langle\nabla R_{i}^{(t)}, \Gamma(p^{(t)_{i}}) - p^{(t)_{i}}\rangle < 0$$
	where $\nabla$ is the gradient operator, and $\langle a, b \rangle$ represents the inner product of vectors a and b.
\end{lemma}
\begin{proof}
	The partial derivative of $R_{i}(p_{i}^{(t)})$ with respect to $p_{i}^{(t)}$ is 
	\begin{equation}
		\begin{aligned}
			\hspace{-1mm}
			&\frac{\partial R_{i}(p_{i}^{(t)})}{\partial p_{i,j}^{(t)}} \\
			&= \frac{\phi_{i}}{\Phi}[(T^{cm}_{i,j} + T^{q}_{j} + T^{cp}_{j} + I_{j}r_{j}) + p_{i,j}^{(t)}\frac{\partial  (T^{q}_{j} + r_{j})}{\partial p_{i,j}^{(t)}} + \frac{\partial (N(p))}{\partial p_{i,j}^{(t)}}]\\
			&= \frac{\phi_{i}}{\Phi}[(T^{cm}_{i,j} + T^{q}_{j} + T^{cp}_{j} + I_{j}r_{j}) + p_{i,j}^{(t)}\Phi_{i}rd_{j}^{(t)}+\frac{\partial (N(p))}{\partial p_{i,j}^{(t)}}]\\
			&= \frac{\phi_{i}}{\Phi}\Delta_{i,j}^{(t)} \nonumber 
		\end{aligned}
	\end{equation}
	where $\Delta_{i,j}^{(t)}$ is defined in formula (\ref{Delta}), therefore,
	\begin{equation}
		\begin{aligned}
			&\langle\nabla R_{i}^{(t)}, \Gamma(p^{(t)}_{i}) - p^{(t)}_{i}\rangle \\
			&= \frac{1}{\Phi}\sum_{e_{i}\in S^{k}} \phi_{i} \sum_{e_{j}\in L_{i}}\Delta_{i,j}^{(t)}(p_{i,j}^{(t+1)}-p_{i,j}^{(t)}) \nonumber
		\end{aligned}
	\end{equation}
	
	
	For edge server $e_{i}$, $e_{j*}$ is the edge server that minimizes $\Delta_{i,j}$, so for any $e_{j}\in L_{i}$, $\Delta_{i,j*}^{(t)} \leq \Delta_{i,j}^{(t)}$
	\begin{equation}
		\begin{aligned}
		&\sum_{e_{j} \in L_{i}}\Delta_{i,j}^{(t)}p_{i,j}^{(t+1)} = 
		\Delta_{i,j*}p_{i,j*}^{(t+1)} + \sum_{\substack{e_{j} \in L_{i}\\j\neq j^{*}}}\Delta_{i,j}^{(t)}p_{i,j}^{(t+1)}\\
		&=\Delta_{i,j*}(p_{i,j*}^{(t)} + \tau \sum_{\substack{e_{j} \in L_{i}\\j\neq j^{*}}} p_{i,j}^{(t)} + \sum_{\substack{e_{j} \in L_{i}\\j\neq j^{*}}}\Delta_{i,j}^{(t)}(1-\tau)p_{i,j}^{(t)}\\
		&=\sum_{e_{j} \in L_{i}}\Delta_{i,j}^{(t)}p_{i,j}^{(t)} + \tau (\Delta_{i,j*}^{(t)}\sum_{\substack{e_{j} \in L_{i}\\j\neq j^{*}}}p_{i,j}^{(t)} - \sum_{\substack{e_{j} \in L_{i}\\j\neq j^{*}}}\Delta_{i,j}^{(t)}p_{i,j}^{(t)})\\
		&\leq \sum_{e_{j} \in L_{i}}\Delta_{i,j}^{(t)}p_{i,j}^{(t)}	\nonumber 
		\end{aligned}	
	\end{equation}
\end{proof}





==> content/evaluation.tex <==
This section first conducts some intuitive tests to exhibit system heterogeneity and dynamics (Section \ref{subsec_system_test}).
% This section first describes the datasets and models for experiments (Section \ref{dataset}).
Then the datasets and models are described for experiments (Section \ref{dataset}), and we introduce baselines and metrics for performance comparison (Section \ref{baselines}).
Simulation settings and results are given in (Section \ref{simulation}). 
Finally, we
evaluate FedLamp through a small-scale test-bed experiment and give the results (Section \ref{testbed1}).


\subsection{Testing of System Heterogeneity and Dynamics}\label{subsec_system_test}
First of all, we conduct some intuitive tests to exhibit the heterogeneous capacities of the commercial edge devices, \eg, NVIDIA Jetson TX2\footnote{More details about NVIDIA Jetson TX2 are available at \url{https://developer.nvidia.com/embedded/jetson-tx2-developer-kit}.}
and NVIDIA Jetson Xavier NX\footnote{More details about NVIDIA Jetson Xavier NX are available at \url{https://developer.nvidia.com/embedded/jetson-xavier-nx-devkit}.}.
Both Jetson TX2 and Jetson Xavier NX can be configured to work under different performance modes, specifying the number of working CPUs and the frequency of CPU/GPU,
so that they have different computing capacities.
Moreover, Jetson Xavier NX accelerates the NVIDIA software stack with more than 10$\times$ the performance of Jetson TX2.
The detailed technical specifications of the Jetson TX2 and Jetson Xavier NX are listed in Table \ref{table:jetson}.
It is worth noting that the proposed algorithm and theoretical analysis in this paper are not limited to mentioned devices, like TX2 or NX.
They can also be applied to various edge devices with different computing and communicating capabilities, \eg, \bluenote{mobile phones}, laptops and so on.
% They can also be applied to various edge devices with different CPU or GPU frequencies, \eg, mobile phone, Raspberry Pi, laptops and so on.

\begin{table}[t]
    \caption{Device Technical Specifications.}
    \label{table:jetson}
    \centering
      \begin{tabular}{l|c|c}
        \hline
        % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
         & \textbf{AI Performance} & \textbf{GPU Type}  \\ \hline
        Jetson TX2 & 1.33 TFLOPS & 256-core Pascal \\ \hline
        Jetson NX  & 21 TOPS & 384-core Volta\\ \hline \hline
        %Jetson AGX & 22 TOPS & 512-core Volta  \\  \hline \hline
        & \textbf{CPU Type} & \textbf{ROM} \\  \hline
       Jetson TX2 & Denver 2 and ARM 4 & 8 GB LPDDR4\\ \hline
       Jetson NX & 6-core Carmel ARM 8 & 8 GB LPDDR4x\\ \hline \hline 
       %Jetson AGX  & 8-core Carmel ARM 8 & 32 GB LPDDR4x \\  \hline
       & \textbf{CPU Frequency} & \textbf{GPU Frequency} \\  \hline
       Jetson TX2 & 2.0GHz & 1.12GHz\\ \hline
       Jetson NX & 1.9GHz & 1100MHz\\ \hline
      \end{tabular}
  \end{table}

\begin{figure}
	\centering
	\subfigure[Computing heterogeneity]
	{
		\includegraphics[width=0.46\linewidth]{fig/train_time}
		\label{fig-tx2-heterogeneity-a}
	}\quad
	\subfigure[Communication heterogeneity]
	{
		\includegraphics[width=0.46\linewidth]{fig/send_time}
		\label{fig-tx2-heterogeneity-b}
	}
	\caption{Illustrations of computing and communication heterogeneity of devices.}
	\label{fig-tx2-heterogeneity}
\end{figure}

For computing test, we adopt two NX devices (device \#1 with low-performance mode and device \#3 with high-performance mode)
and two TX2 devices (device \#2 with high-performance mode and device \#4 with low-performance mode) as the heterogeneous workers.
Both the TX2 and NX devices are implemented to perform matrix multiplication over two 1500$\times$1500 sized tensors for 30 times,
and the computing time of each device is illustrated in Fig. \ref{fig-tx2-heterogeneity-a}.
Device \#4 takes the highest average computing time of 11.2s among all the devices, while device \#3 needs the lowest average computing time (\ie, 1.6s).
The average computing time of device \#2 and device \#3 is 3.2s and 6.3s, respectively.
The computing time of the low-performance device is almost \bluenote{seven} times as long as that of the high-performance one, which obviously illustrates the computing heterogeneity.
%Generally, the TX2 devices and NX devices powered with different modes have heterogeneous capacity, which is common for EC scenario.

Except for the computing heterogeneity among workers, the bandwidth of each worker may also be different (\ie, communication heterogeneity).
In EC, workers are usually connected to the edge server through wireless links, and the signal strength of the wireless link may vary with the transmission distance \cite{tse2005fundamentals}.
We put two NX devices and two TX2 devices in two different rooms\bluenote{, which are about 50 meters} far from each other \bluenote{for the communication test.}
Concretely, device \#1 and device \#2 are close to the wireless router, while device \#3 and device \#4 are far away from the wireless router.
Four devices synchronously send a 1500$\times$1500 sized tensor to the server, which is also connected to the wireless router, and we record their communication bandwidth.
By Fig. \ref{fig-tx2-heterogeneity-b}, the bandwidth of device \#1 and device \#2 is almost 6 times as much as that of device \#3 and device \#4, which reveals the communication heterogeneity.

\subsection{Datasets and Models}\label{dataset}
\textbf{Datasets:}
We conduct extensive experiments on three real-world datasets: (i) Fashion-MNIST\footnote{\url{https://github.com/TalwalkarLab/leaf}} (FMNIST for short),
(ii) CIFAR-10\footnote{\url{https://www.cs.toronto.edu/~kriz/cifar.html}}, and (iii) CIFAR-100\footnote{\url{https://www.cs.toronto.edu/~kriz/cifar.html}}.
Specifically, FMNIST \cite{xiao2017fashion} contains a training set with 60,000 samples and a test set with 10,000 samples. Each sample in FMNIST is a 28 $\times$ 28 grayscale fashion products
from 10 categories. CIFAR-10 contains 60,000 32 $\times$ 32 color images labeled in 10 classes with 50,000 samples for training and 10,000 samples for test.
%CIFAR-10 is composed of 60,000 32 × 32 colour images (50,000 for training and 10,000 for testing) in 10 categories.
CIFAR-100 has the same total number of image samples as CIFAR-10 but consists of 100 classes, which is more challenging to train models for classification.
Except for the experiments for evaluating model performance on non-IID data, all datasets are distributed uniformly across workers by default.

\textbf{Models:} Three models with different types and structures are implemented on the above three real-world datasets for performance evaluation:
(i) CNN on FMNIST, (ii) AlexNet on CIFAR-10, (iii) ResNet9 on CIFAR-100.
The plain CNN model \cite{mcmahan2017communication} specialized for the FMNIST dataset has two 5 $\times$ 5 convolutional layers,
a fully-connected layer with 512 units, and a softmax output layer with 10 units. The CNN model is about 5M in size. 
An 8-layer AlexNet \cite{krizhevsky2012imagenet} which is composed of three 3 $\times$ 3 convolutional
layers, one 7 $\times$ 7 convolutional layer, one 11 $\times$ 11 convolutional layer, two fully-connected hidden layers,
and one fully-connected output layer is adopted for CIFAR-10. The size of AlexNet is about 15M, which is larger than the size of plain CNN model.
For the CIFAR-100 dataset which is more challenging to train,
a famous model ResNet9 \cite{rothchild2020fetchsgd} with size of 25M is adopted.

\subsection{Baselines and Metrics}\label{baselines}
%We train three models with our proposed method FedLamp, optimizing both the local updating frequency and model compression ratio.
%For comparison, we introduce other four strategies as baselines to train three models.
\textbf{Baselines:} We choose four classical and efficient algorithms as baselines for performance comparison, which are summarized as follows
\vspace{-0.2cm}
\begin{itemize}
	\item \textbf{FedAvg} \cite{mcmahan2017communication} is a famous algorithm in federated learning with fixed (non dynamic) and identical (non diverse) local updating frequency for workers without model compression.
	\item \textbf{ADP} \cite{wang2019adaptive} adaptively determines the identical local updating frequency for all workers at each communication round \bluenote{on the basis of} both the constrained resource and context dynamics so as to realize communication-efficient FL and speed up the training process.
	\item \textbf{Qsparse} \cite{basu2020qsparse} combines aggressive sparsification with quantization as model compression operator to reduce communication resource consumption without controlling the local updating frequency and model compression ratio.
	\item \textbf{FFL} \cite{nori2021fast} is a state-of-the-art algorithm, and it jointly and dynamically determines identical local updating frequency and model compression ratio for all workers at each communication round without considering the system heterogeneity.
	%which are identical among workers without considering the heterogeneities of workers.
\end{itemize}
The strategies of adjusting local updating frequency and model compression ratio in FedLamp and the baselines are summarized in Table \ref{table:baseline}.
% The first one, called 
% The second one is ADP \cite{wang2019adaptive}, where the number of local updates before one global update on each edge node are adaptively determined by the coordinator
% and can be found via linear search to minimize the loss function under given resource constraints.

% The third one is Qsparse \cite{basu2020qsparse}, which 
% The last one, called FFL \cite{nori2021fast}, 

% We adopt the following metrics to evaluate the efficiency of our proposed algorithm. for performance evaluation:
\textbf{Metrics:} The following metrics are adopted to evaluate the performance of our FedLamp and the baselines.
\vspace{-0.2cm}
\begin{itemize}
	\item \textbf{Test accuracy} is measured by the proportion between the amount of the right data predicted by the model and that of all data. Specifically, during the training process, at each communication round, we evaluate the test accuracy \bluenote{of the global model trained} with different algorithms on the test sets.
	\item \textbf{Training loss} is the quantification difference of probability distributions between model outputs and the corresponding labels.
	\item \textbf{Completion time} is defined as the total training time until the global model achieves a target accuracy. In addition, we also record the average waiting time to reflect the training efficiency of different algorithms.
	\item \textbf{Network traffic} is calculated by summing the network traffic for model transmission between workers and the PS when achieving a target accuracy.
\end{itemize}
% (i) Test accuracy is measured by the proportion between the amount of the right data predicted by the model and that of all data.
% Specifically, during the training process, at each epoch, we evaluate the test accuracy of global model trained with different strategies on the test sets.
% (ii) Training loss is the quantification difference of probability distributions between model outputs and the corresponding labels.
% (iii) Completion Time is defined as the total training time until the global model achieves a target accuracy. Besides, we record the 
% average waiting time to evaluate the training efficiency of different algorithms.
% (iv) Network Traffic is calculated by summing the network traffic for communication among all the edge nodes when achieving a target accuracy.

\begin{table}[!t]
	\caption{Different strategies of baselines and FedLamp.}
	\label{table:baseline}
	\centering
	\begin{threeparttable}
		\begin{tabular}{c|c|c|c|c}
			\hline
			% after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
			\multirow{3}*{algorithms} & \multicolumn{4}{c}{strategies}  \\ 
			\cline{2-5}
			& \multicolumn{2}{c|}{LUF\tnote{*}} & \multicolumn{2}{c}{MCR\tnote{*}}  \\
			\cline{2-5}
			& dynamic & diverse & dynamic & diverse \\ \hline
			FedAvg & $\times$  & $\times$ & -  & -\\ \hline
			ADP  & $\checkmark$ & $\times$& -  & -\\ \hline
			Qsparse & $\times$  & $\times$& $\times$  & $\times$\\ \hline
			FFL  & $\checkmark$ & $\times$& $\checkmark$ & $\times$\\ \hline
			FedLamp  & $\checkmark$ & $\checkmark$& $\checkmark$ & $\checkmark$\\ \hline
		\end{tabular}
		\begin{tablenotes}
			\footnotesize
			\item[*] LUF denotes local updating frequency.
			\item[*] MCR denotes model compression ratio.
		\end{tablenotes}
	\end{threeparttable}
\end{table}

\begin{figure*}[!t]
	\centering
	%		\vspace{5pt}
	\subfigure[FMNIST]
	{
		\includegraphics[width=0.29\linewidth,height=4cm]{fig/FashionMNIST_time_acc}
		\label{fig:time_acc_a}
	}\quad
	\subfigure[CIFAR-10]
	{
		\includegraphics[width=0.29\linewidth,height=4cm]{fig/Cifar10_time_acc}
		\label{fig:time_acc_b}
	}\quad
	\subfigure[CIFAR-100]
	{
		\includegraphics[width=0.29\linewidth,height=4cm]{fig/Cifar100_time_acc}
		\label{fig:time_acc_c}
	}
	%	\setlength{\abovecaptionskip}{-3pt}
	\caption{Test accuracy of five algorithms on the three datasets in simulation.}
	%	\vspace{-15pt}
	\label{fig:time_acc}
\end{figure*}

\begin{figure*}[!t]
	\centering
	%		\vspace{5pt}
	\subfigure[FMNIST]
	{
		\includegraphics[width=0.29\linewidth,height=4.1cm]{fig/FashionMNIST_time_loss}
	}\quad
	\subfigure[CIFAR-10]
	{
		\includegraphics[width=0.29\linewidth,height=4.1cm]{fig/Cifar10_time_loss}
	}\quad
	\subfigure[CIFAR-100]
	{
		\includegraphics[width=0.29\linewidth,height=4cm]{fig/Cifar100_time_loss}
	}
	%	\setlength{\abovecaptionskip}{-3pt}
	\caption{Training loss of five algorithms on the three datasets in simulation.}
	%	\vspace{-15pt}
	\label{fig:time_loss}
\end{figure*}

\subsection{Simulation Experiments}\label{simulation}
\subsubsection{Simulation Setup}
We evaluate the performance of FedLamp through extensive simulation experiments, which are conducted on an
AMAX deep learning workstation equipped with an Intel(R) Core(TM) i9-10900X CPU, 4 NVIDIA GeForce RTX 2080Ti GPUs and 128 GB RAM.
On the workstation, we simulate a resource-constrained EC system with 10 workers and 1 PS (each is implemented as a process in the system) for federated learning.
The implementation for model training on each worker is based on the PyTorch framework \cite{paszke2019pytorch},
and we use the socket library of Python to build up the communication between workers and the PS.

%To simulate the heterogeneous communication capacities of workers,
We consider the common situation where each worker communicates with the PS through either LANs or WANs.
To reflect the heterogeneity and dynamics of networks in our simulations, we let the inbound bandwidth of each worker fluctuate between 10Mb/s and 20Mb/s.
Considering the outbound bandwidth in typical WANs is usually smaller than the inbound bandwidth \cite{mcmahan2017communication}, we configure it to fluctuate between 0.5Mb/s and 5Mb/s.
In addition, for simulating the computing heterogeneity, we assume the computing time of one local iteration on a certain simulated worker is subject to the Gaussian distribution. 
Different simulated workers are randomly assigned with a specific Gaussian function whose mean and variance are derived from the time records of performing one local update on a commercial device (\eg, laptop, Jetson TX, Xavier NX).

% we randomly assign each worker with a different capacity factor
% that denotes the time for performing local updating and is
% set as the average value of measurements from our extensive test on some commercial devices (\eg, laptop, Jetson TX2, Xavier NX).}
In simulation experiments, the number of communication rounds are specified as 400, 500 and 500 for FMNIST, CIFAR-10 and CIFAR-100, respectively, which will guarantee the convergence of the models.
For CNN on FMNIST and AlexNet on CIFAR-10, the learning rates are separately initialized as 0.05 and 0.1, and the corresponding decay rates
are specified as 0.99 and 0.993. 
Besides, for ResNet9 on CIFAR-100, the momentum-SGD optimizer is adopted in our experiments to optimize the models, and the momentum is set as 0.9
while the weight decay is 0.001 \cite{rothchild2020fetchsgd}. Then the learning rate and the learning rate decay is initialized as 0.1 and 0.99, respectively. The batch size is set as 32 for all three models.

% For computation, according to our extensive test on some commercial devices (\eg, laptop, Jetson TX2, Xavier NX), 
% the measured computation time (when performing
% 30 times of local updating with batch size of 32) for CNN on FMNIST varies between 0.5s and 2.5s, for AlexNet on CIFAR-10 varies between 3.2s and 8.5s
% and for ResNet9 on CIFAR-100 varies between 9.3s and 20.5s.
% Meanwhile, the time for efficient implementation of model compression is about 0.1s,
% which can be ignored compared with the time for local updating and model transmission.
% Therefore, on the basis of the measurement, we dynamically and randomly assign the running time within the ranges for
% different workers while conducting local updating on different learning tasks.
% In this section, we conduct extensive simulation to evaluate the performance of the proposed algorithm.
% The simulation experiments are performed on an AMAX deep learning workstation (CPU: Intel 671 (R) E5-2620v4, GPU: NVIDIA TITAN RTX),
% where we build an FL experimental environment and implement the proposed algorithm with PyTorch [34].
% Specifically, we create 11 virtual machines in the experimental environment, where they communicate with socket.
% One of the virtual machines is specified as the parameter server (PS) and the remaining 10 virtual machines act as the edge devices.
% %In the experimental environment, we create 10 virtual machines to act as the edge devices and a virtual machine to act as the PS,
% %where they communicate with socket.
% %To simulate the heterogeneous communication resource of edge devices, we randomly assign each device with a different factor that denotes
% %the bandwidth of edge devices and is set as the average value of measurements from one of the commercial devices (e.g., smartphones, laptops, Raspberry Pi computers).
% To simulate the heterogeneous computation and communication capacities of edge devices, we randomly assign each device with different capacity factors
% that denote the time for processing one local iteration and transmiting an original model, respectively, which are set as the average value of measurements
% from one of the commercial devices (\textit{e.g.}, laptops, smartphones, Raspberry Pi computers).
%Besides, the batch size and learning rate are set as 32 and 1e-3 for FMNIST, 32 and 0.01 for CIFAR-10 as well as 32 and 0.01 for CIFAR-100 in simulation.

\begin{table}[!t]
	\centering
	\caption{Training performance of CNN on FashionMNIST.}
	\resizebox{1\linewidth}{!}{
		\begin{tabular}{c|c|ccccccccc}
			\hline
			\multicolumn{2}{c|}{Metrics}& \textit{FedLamp} & FFL & Qsparse & ADP & FedAvg\\ \hline
			\ & Accuracy    &     91.51\%       & 91.38\% &	91.32\% &	91.31\%	& 91.03\%\\
			\cline{1-7}
			\multirow{2}{*}{Accuracy = 91\%} & Time (s)    & 900    & 1778 &  2571	& 3805	& 6167\\
 			\cline{2-7}
            &Traffic (MB)  & 527   & 1436 & 718 & 3231 & 4491\\
            \hline
	\end{tabular}
    }
    \label{tb:metrics on CNN}
\end{table}

\begin{table}[!t]
	\centering
	\caption{Training performance of AlexNet on CIFAR-10.}
	\resizebox{1\linewidth}{!}{
		\begin{tabular}{c|c|ccccccccc}
			\hline
			\multicolumn{2}{c|}{Metrics}& \textit{FedLamp} & FFL & Qsparse & ADP & FedAvg\\ \hline
			\ & Accuracy    &     77.54\%       & 77.46\% &	77.15\% &	77.42\%	& 76.83\%\\
			\cline{1-7}
			\multirow{2}{*}{Accuracy = 76\%} & Time (s)    & 2089   & 4918 & 5878	& 7570	&10733\\
 			\cline{2-7}
			&Traffic (MB)  & 1352   & 3368 & 1684 & 10104 & 11227\\
            \hline
	\end{tabular}
    }
    \label{tb:metrics on AlexNet}
\end{table}

\begin{table}[!t]
	\centering
	\caption{Training performance of ResNet9 on CIFAR-100.}
	\resizebox{1\linewidth}{!}{
		\begin{tabular}{c|c|ccccccccc}
			\hline
			\multicolumn{2}{c|}{Metrics}& \textit{FedLamp} & FFL & Qsparse & ADP & FedAvg\\ \hline
			\ & Accuracy    &     55.93\%       & 55.72\% &	54.99\% &	54.9\%	& 54.31\%\\
			\cline{1-7}
			\multirow{2}{*}{Accuracy = 54\%} & Time (s)    & 4057  & 7903 &  9716	& 13678	& 17075\\
 			\cline{2-7}
			&Traffic (MB)  & 2654   & 7455 & 3727 &	16773 &	18637\\
            \hline
	\end{tabular}
    }
    \label{tb:metrics on ResNet9}
\end{table}

% \begin{figure*}[!t]
% 	\centering
% 	%		\vspace{5pt}
% 	\subfigure[FMNIST]
% 	{
% 		\includegraphics[width=0.29\linewidth,height=2.2cm]{fig/FashionMNIST_time_acc}
% 	}
% 	\subfigure[CIFAR-10]
% 	{
% 		\includegraphics[width=0.29\linewidth,height=2.2cm]{fig/Cifar10_time_acc}
% 	}
% 	\subfigure[CIFAR-100]
% 	{
% 		\includegraphics[width=0.29\linewidth,height=2.2cm]{fig/Cifar100_time_acc}
% 	}
% 	%	\setlength{\abovecaptionskip}{-3pt}
% 	\caption{Test accuracy of five strategies of three datasets in simulation.}
% 	%	\vspace{-15pt}
% 	\label{fig:time_acc}
% \end{figure*}

% \begin{figure*}[!t]
% 	\centering
% 	%		\vspace{5pt}
% 	\subfigure[FMNIST]
% 	{
% 		\includegraphics[width=0.29\linewidth,height=2.2cm]{fig/FashionMNIST_time_loss}
% 	}
% 	\subfigure[CIFAR-10]
% 	{
% 		\includegraphics[width=0.29\linewidth,height=2.2cm]{fig/Cifar10_time_loss}
% 	}
% 	\subfigure[CIFAR-100]
% 	{
% 		\includegraphics[width=0.29\linewidth,height=2.15cm]{fig/Cifar100_time_loss}
% 	}
% 	%	\setlength{\abovecaptionskip}{-3pt}
% 	\caption{Train loss of five strategies of three datasets in simulation.}
% 	%	\vspace{-15pt}
% 	\label{fig:time_loss}
% \end{figure*}

% \begin{figure*}[!t]
% 	\centering
% 	%		\vspace{5pt}
% 	\subfigure[FMNIST]
% 	{
% 		\includegraphics[width=0.29\linewidth,height=2.2cm]{fig/FashionMINIST_avg_waiting_time}
% 	}
% 	\subfigure[CIFAR-10]
% 	{
% 		\includegraphics[width=0.29\linewidth,height=2.2cm]{fig/Cifar10_avg_waiting_time}
% 	}
% 	\subfigure[CIFAR-100]
% 	{
% 		\includegraphics[width=0.29\linewidth,height=2.2cm]{fig/Cifar100_avg_waiting_time}
% 	}
% 	%	\setlength{\abovecaptionskip}{-3pt}
% 	\caption{Epoch-wise average waiting time of all devices of five strategies of three datasets in simulation.}
% 	%	\vspace{-15pt}
% 	\label{fig:waiting_time}
% \end{figure*}

% \begin{figure*}[!t]
% 	\centering
% 	%		\vspace{5pt}
% 	\subfigure[FMNIST]
% 	{
% 		\includegraphics[width=0.29\linewidth,height=2.2cm]{fig/FashionMNIST_bandwidth}
% 	}
% 	\subfigure[CIFAR-10]
% 	{
% 		\includegraphics[width=0.29\linewidth,height=2.2cm]{fig/Cifar10_bandwidth}
% 	}
% 	\subfigure[CIFAR-100]
% 	{
% 		\includegraphics[width=0.29\linewidth,height=2.2cm]{fig/Cifar100_bandwidth}
% 	}
% 	%	\setlength{\abovecaptionskip}{-3pt}
% 	\caption{Traffic consumption of five strategies when achieving the same test accuracy of three models in simulation.}
% 	%	\vspace{-15pt}
% 	\label{fig:bandwidth}
% \end{figure*}

% \begin{table}[t]
% 	\centering
% 	\caption{Performance metrics for CNN on FashionMNIST.}
% 	\resizebox{1\linewidth}{!}{
% 		\begin{tabular}{c|c|ccccccccc}
% 			\hline
% 			\multicolumn{2}{c|}{Metrics}& \textit{FedLamp} & FFL & Qsparse & ADP & FedAvg\\ \hline
% 			\ & Accuracy    &     91.51\%       & 91.38\% &	91.32\% &	91.31\%	& 91.03\%\\
% 			\cline{1-7}
% 			\multirow{2}{*}{Accuracy = 91\%} & Time (s)    & 900    & 1778 &  2571	& 3805	& 6167\\
%  			\cline{2-7}
%             &Traffic (MB)  & 527   & 1436 & 718 & 3231 & 4491\\
%             \hline
% 	\end{tabular}
%     }
%     \label{tb:metrics on CNN}
% \end{table}

% \begin{table}[!t]
% 	\centering
% 	\caption{Performance metrics for AlexNet on CIFAR-10.}
% 	\resizebox{1\linewidth}{!}{
% 		\begin{tabular}{c|c|ccccccccc}
% 			\hline
% 			\multicolumn{2}{c|}{Metrics}& \textit{FedLamp} & FFL & Qsparse & ADP & FedAvg\\ \hline
% 			\ & Accuracy    &     77.54\%       & 77.46\% &	77.15\% &	77.42\%	& 76.83\%\\
% 			\cline{1-7}
% 			\multirow{2}{*}{Accuracy = 76\%} & Time (s)    & 2089   & 4918 & 5878	& 7570	&10733\\
%  			\cline{2-7}
% 			&Traffic (MB)  & 1352   & 3368 & 1684 & 10104 & 11227\\
%             \hline
% 	\end{tabular}
%     }
%     \label{tb:metrics on AlexNet}
% \end{table}

% \begin{table}[!t]
% 	\centering
% 	\caption{Performance metrics for ResNet9 on CIFAR-100.}
% 	\resizebox{1\linewidth}{!}{
% 		\begin{tabular}{c|c|ccccccccc}
% 			\hline
% 			\multicolumn{2}{c|}{Metrics}& \textit{FedLamp} & FFL & Qsparse & ADP & FedAvg\\ \hline
% 			\ & Accuracy    &     55.93\%       & 55.72\% &	54.99\% &	54.9\%	& 54.31\%\\
% 			\cline{1-7}
% 			\multirow{2}{*}{Accuracy = 54\%} & Time (s)    & 4057  & 7903 &  9716	& 13678	& 17075\\
%  			\cline{2-7}
% 			&Traffic (MB)  & 2654   & 7455 & 3727 &	16773 &	18637\\
%             \hline
% 	\end{tabular}
%     }
%     \label{tb:metrics on ResNet9}
% \end{table}

% \begin{figure*}[!t]
% 	\centering
% 	%  \vspace{5pt}
% 	\begin{minipage}{0.62\linewidth}
% 	\subfigure[Accuracy]
% 	{
% 		\includegraphics[width=0.45\linewidth,height=2.2cm]{fig/Cifar10_non_iid_time_acc}
% 		\label{fig:non-iid_time_acc}
% 	}
% 	\subfigure[Loss]
% 	{
% 		\includegraphics[width=0.45\linewidth,height=2.2cm]{fig/Cifar10_non_iid_time_loss}
% 		\label{fig:non-iid_time_loss}
% 	}
% 	\caption{Training process of five algorithms on non-IID CIFAR-10 (p=0.8) dataset}
% 	% \vspace{-15pt}
% 	\label{fig:non-iid_Cifar101}
% 	\end{minipage}
% 	\begin{minipage}{0.32\linewidth}
% 	\subfigure[non-IID]
% 	{
% 		\includegraphics[width=0.9\linewidth,height=2.2cm]{fig/non-iid_level}
% 		\label{fig:non-iid_level}
% 	}
% 	% \setlength{\abovecaptionskip}{-3pt}
% 	\caption{Performance for deliver non-IID levels}
% 	% \vspace{-15pt}
% 	\label{fig:non-iid_Cifar102}
% 	\end{minipage}
% \end{figure*}

% \begin{figure}[!t]
% 	\centering
% 	%		\vspace{5pt}
% 	\subfigure[Accuracy]
% 	{
% 		\includegraphics[width=0.29\linewidth,height=2.2cm]{fig/Cifar10_non_iid_time_acc}
% 		\label{fig:non-iid_time_acc}
% 	}
% 	\subfigure[Loss]
% 	{
% 		\includegraphics[width=0.29\linewidth,height=2.2cm]{fig/Cifar10_non_iid_time_loss}
% 		\label{fig:non-iid_time_loss}
% 	}
% 	\subfigure[CIFAR-10]
% 	{
% 		\includegraphics[width=0.29\linewidth,height=2.2cm]{fig/non-iid_level}
% 		\label{fig:non-iid_level}
% 	}
% 	%	\setlength{\abovecaptionskip}{-3pt}
% 	\caption{Training process of non-IID CIFAR-10}
% 	%	\vspace{-15pt}
% 	\label{fig:non-iid_Cifar10}
% \end{figure}

\begin{figure*}[t]
	\centering
	%		\vspace{5pt}
	\subfigure[FMNIST]
	{
		\includegraphics[width=0.29\linewidth,height=4cm]{fig/FashionMINIST_avg_waiting_time}
	}\quad
	\subfigure[CIFAR-10]
	{
		\includegraphics[width=0.29\linewidth,height=4cm]{fig/Cifar10_avg_waiting_time}
		\label{fig:C10waiting_time}
	}\quad
	\subfigure[CIFAR-100]
	{
		\includegraphics[width=0.29\linewidth,height=4cm]{fig/Cifar100_avg_waiting_time}
	}
	%	\setlength{\abovecaptionskip}{-3pt}
	\caption{Average waiting time of five algorithms on the three datasets in simulation.}
	%	\vspace{-15pt}
	\label{fig:waiting_time}
\end{figure*}

\begin{figure*}[t]
	\centering
	%		\vspace{5pt}
	\subfigure[FMNIST]
	{
		\includegraphics[width=0.29\linewidth,height=4.4cm]{fig/FashionMNIST_bandwidth}
	}\quad
	\subfigure[CIFAR-10]
	{
		\includegraphics[width=0.29\linewidth,height=4.4cm]{fig/Cifar10_bandwidth}
		\label{fig:C10bandwidth}
	}\quad
	\subfigure[CIFAR-100]
	{
		\includegraphics[width=0.29\linewidth,height=4.4cm]{fig/Cifar100_bandwidth}
	}
	%	\setlength{\abovecaptionskip}{-3pt}
	\caption{Network traffic consumption of five algorithms when achieving the target accuracy on the three datasets in simulation.}
	%	\vspace{-15pt}
	\label{fig:bandwidth}
\end{figure*}

\begin{figure*}[t]
	\centering
	%  \vspace{5pt}
	\begin{minipage}{0.62\linewidth}
	\subfigure[Test accuracy]
	{
		\includegraphics[width=0.45\linewidth,height=4.1cm]{fig/Cifar10_non_iid_time_acc}
		\label{fig:non-iid_time_acc}
	}\quad
	\subfigure[Training loss]
	{
		\includegraphics[width=0.45\linewidth,height=4.2cm]{fig/Cifar10_non_iid_time_loss}
		\label{fig:non-iid_time_loss}
	}
	\caption{Training process of five algorithms on the non-IID (p=0.8)\\ CIFAR-10 dataset.}
	% \vspace{-15pt}
	\label{fig:non-iid_Cifar101}
	\end{minipage}\quad
	\centering
	\begin{minipage}{0.35\linewidth}
	%\subfigure[Impact on non-IID levels]
	%{
	\includegraphics[width=0.8\linewidth,height=4.1cm]{fig/non-iid_level}
	\vspace{5mm}
	%}
	% \setlength{\abovecaptionskip}{-3pt}
	\caption{Training performance for different non-IID levels.}
	\label{fig:non-iid_level}
	% \vspace{-15pt}
	\end{minipage}
\end{figure*}

\subsubsection{Simulation Results}
We implement one group of experiments of these algorithms for the three models and datasets.
The training processes of FedLamp and the baselines are presented in Fig. \ref{fig:time_acc}
and Fig. \ref{fig:time_loss}.
The results demonstrate that all the algorithms can achieve similar accuracy but FedLamp achieves the fastest convergence rate for all the three datasets,
which indicates the effectiveness of adaptively determining diverse and appropriate local updating frequencies
and model compression ratios for heterogeneous workers.
For example, by Table. \ref{tb:metrics on AlexNet} and Fig. \ref{fig:time_acc_b}, FedLamp takes 2089s to achieve 76\% accuracy for AlexNet on CIFAR-10,
while FedAvg, ADP, Qsparse, FFL takes 10733s, 7570s, 5878s, 4918s, respectively.
Besides, by Table. \ref{tb:metrics on CNN} and Fig. \ref{fig:time_acc_a}, we observe that FedLamp can speed up training by about 6.8$\times$, 4.2$\times$, 2.8$\times$ and 1.9 $\times$, compared to FedAvg, ADP, Qsparse and FFL, respectively.
Moreover, by Table. \ref{tb:metrics on ResNet9} and Fig. \ref{fig:time_acc_c} for ResNet9 on CIFAR-100,
FedLamp can reduce the completion time of training by about 48\%, 58\%, 70\% and 76\%, compared to FedAvg, ADP, Qsparse and FFL, respectively.
It is worth noting that in Tables \ref{tb:metrics on CNN}, \ref{tb:metrics on AlexNet} and \ref{tb:metrics on ResNet9}, the accuracy is set as the target that all the algorithms can achieve.

To further illustrate the efficiency of FedLamp, the average waiting time of all algorithms for three datasets are listed in Fig. \ref{fig:waiting_time},
where the horizontal axis denotes the number of training communication rounds.
By Fig. \ref{fig:waiting_time}, we can find that FedLamp takes much less waiting time than FedAvg and ADP.
For instance, by Fig. \ref{fig:C10waiting_time}, the average waiting time of FedLamp is 1.5s while FedAvg and ADP incur 13s and 11.5s average waiting time, respectively.
This is because both FedAvg and ADP assign identical local updating frequencies for workers without considering the impacts of computing heterogeneity and synchronization barrier, resulting in non-negligible waiting time.
Moreover, the variance of waiting time in FedAvg is quite large while the waiting time in FedLamp is relatively stable, since FedAvg cannot deal with the challenge of context dynamics in FL.
Besides, ADP, which adaptively determines the local updating frequency at each communication round \bluenote{on the basis of} both the constrained resource and dynamic context, can reduce the variance of waiting time to some extent.
That explains why FedLamp can achieve much faster converge rate than FedAvg and ADP in Figs. \ref{fig:time_acc} and \ref{fig:time_loss} while ADP takes less completion time than FedAvg.
The results in Fig. \ref{fig:waiting_time} demonstrate that FedLamp can well overcome the challenges of system heterogeneity and context dynamics.

To demonstrate the communication efficiency of FedLamp, we show network traffic consumption of different algorithms when they achieve different target accuracy in Fig. \ref{fig:bandwidth}.
We can find that the network traffic consumption of all algorithms for all datasets increases with the increasing accuracy.
However, FedLamp can always consume the minimum network traffic.
In addition, the algorithms with model compression can save much more network traffic than the algorithms without model compression.
For example, by Table. \ref{tb:metrics on ResNet9} for ResNet9 on CIFAR-100, FedLamp, FFL and Qsparse consume 2654MB, 7455MB and 3727MB while
ADP and FedAvg consume 16773MB and 18637MB, respectively, 
when they achieve the target accuracy.
Moreover, model compression can reduce the communication time, which explains why Qsparse and FFL incur less average waiting time and completion time than ADP and FedAvg.
However, both FFL and Qsparse assign identical local updating frequency and model compression ratio for different workers,
without overcoming the system heterogeneity (including communication heterogeneity and computing heterogeneity), so that they take more waiting time and training time than FedLamp.
With dynamic local updating frequencies and model compression ratios for workers, FFL can achieve faster convergence rate than Qsparse, but it cannot assign low model compression ratio, resulting in more network traffic compared to Qsparse.
FedLamp, which is faster than FFL, can still achieve lower model compression ratio than Qsparse.
Concretely, by Tables. \ref{tb:metrics on AlexNet} and \ref{tb:metrics on CNN},
FedLamp can save network traffic consumption by about 59\%, 19\%, 86\%, 87\% for AlexNet on CIFAR-10, and by about
909MB, 191MB, 2704MB, 3964MB for CNN on FMNIST, compared to the baselines (FFL, Qsparse, ADP, FedAvg), respectively.

In a word, since FedLamp is designed to adaptively determine diverse and appropriate local updating frequencies and model compression ratios for heterogeneous workers, it can overcome the challenges of system heterogeneity, context dynamics in resource-constrained EC systems, and can take few waiting time and network traffic consumption to achieve fast convergence rate.

\subsubsection{Impacts of non-IID levels}
% non-IID is a common data distribution in FL, where distribution of local data is not independent and identically distributed.
Considering that the workers in FL collect data from their
physical locations directly, the data on different workers in FL are not independent and identically distributed (\ie, non-IID).
Thus, we further evaluate FedLamp and the baselines on non-IID data.
Concretely, we create non-IID data of the CIFAR-10 dataset with different partition schemes for the workers.
Each worker has p (p = 0.1, 0.2, 0.4, 0.6 and 0.8) of a unique class in 10 classes
and the remaining samples of each class are partitioned to other workers uniformly. Note
that p = 0.1 is a special case, where the distribution of training dataset is IID. We denote the
non-IID levels of CIFAR-10 as 0.1, 0.2, 0.4, 0.6 and 0.8.
Note that the test datasets are partitioned uniformly among workers for a fair comparison.
For the non-IID CIFAR-10 dataset, the training process of FedLamp and the baselines are presented in Fig. \ref{fig:non-iid_time_acc}
and Fig. \ref{fig:non-iid_time_loss} in terms of training time.
The experiment results demonstrate that even in the non-IID settings, FedLamp can still achieve the fastest convergence with higher test accuracy compared to the baselines.
Besides, we show the impacts of non-IID levels on test accuracy of different algorithms in Fig. \ref{fig:non-iid_level}, where the horizontal axis is non-IID levels and the vertical axis is test accuracy.
The result indicates that all algorithms suffer from a loss of accuracy with the increasing of non-IID level on CIFAR-10, while FedLamp is more robust than other baselines.
In the future, we will pay more attention to the challenge of non-IID data and attempt to overcome it with more advanced techniques for FedLamp.

\subsection{Test-bed Experiments}\label{testbed1}
\subsubsection{Test-bed Setup}
To better evaluate the performance of different algorithms on practical hardware platform,
we further conduct some test-bed experiments.
The test-bed experiments are performed on an AMAX deep learning workstation (CPU: Intel(R) E5-2620v4, GPU: NVIDIA GeForce RTX TITAN),
5 NVIDIA Jetson TX2 developer kits and 5 NVIDIA Jetson Xavier NX developer kits,
where the AMAX workstation acts as the server while Jetson TX2 and Jetson Xavier NX serve as workers.
The detailed technical specifications of the Jetson TX2 and Jetson Xavier NX are listed in Table \ref{table:jetson}.
The experimental network is established via a router,
where the server is directly connected to the router by Ethernet while Jetson TX2 and Jetson Xavier NX are accessed via wireless link.
Besides, the Jetson TX2 and Jetson Xavier NX devices are powered with different modes to represent the computing heterogeneity and dynamics,
and the different distances between the devices and the router as well as the random
channel noise can result in the communication heterogeneity and dynamics.
Our software implementation is based on the PyTorch deep learning framework \cite{paszke2019pytorch}, which enables the model training on the workers.
Furthermore, communication among workers is established based on socket, which provides a set of sending and receiving functions contributing to much more efficient parallel communication.
In addition, we can directly record the average waiting time, completion time and network traffic consumption in the test-bed experiments.

\begin{figure}[t]
	\centering
	%		\vspace{5pt}
	\subfigure[Accuracy]
	{
		\includegraphics[width=0.46\linewidth,height=3.5cm]{fig/testbed_Cifar10_time_acc}
		\label{fig:testbed_time_acc}
	}
	\subfigure[Loss]
	{
		\includegraphics[width=0.46\linewidth,height=3.52cm]{fig/testbed_Cifar10_time_loss}
		\label{fig:testbed_time_loss}
	}
	\caption{Training processes of the algorithms on CIFAR-10 in test-bed experiments.}
	%	\vspace{-15pt}
	\label{fig:testbed_Cifar10_1}
\end{figure}
\begin{figure}[t]
	\centering
	%		\vspace{5pt}
	\subfigure[Average waiting time]
	{
		\includegraphics[width=0.46\linewidth,height=3.28cm]{fig/testbed_Cifar10_avg_waiting_time}
		\label{fig:testbed_waiting_time}
	}
	\subfigure[Traffic vs. Accuracy]
	{
		\includegraphics[width=0.46\linewidth,height=3.5cm]{fig/testbed_Cifar10_bandwidth}
		\label{fig:testbed_bandwidth}
	}
	\caption{Average waiting time and network traffic consumption of the algorithms on CIFAR-10 in test-bed experiments.}
	%	\vspace{-15pt}
	\label{fig:testbed_Cifar10_2}
\end{figure}
\begin{table}[t]
	\centering
	\caption{Training performance of test-bed experiments.}
	\resizebox{1\linewidth}{!}{
		\begin{tabular}{c|c|ccccccccc}
			\hline
			\multicolumn{2}{c|}{Metrics}& \textit{FedLamp} & FFL & Qsparse & ADP & FedAvg\\ \hline
			\ & Accuracy    &     77.06\%       & 76.06\% &	76.52\% &	76.17\%	& 76.86\%\\
			\cline{1-7}
			\multirow{2}{*}{Accuracy = 76\%} & Time (s)    & 2109   & 4697 & 6748	& 10508	& 13450\\
 			\cline{2-7}
			&Traffic (MB)  & 1453   & 3488 & 1886 & 9134 & 10257\\
            \hline
	\end{tabular}
    }
    \label{tb:testbed metrics on AlexNet}
\end{table}
\subsubsection{Test-bed Result}
We implement the training of AlexNet on CIFAR-10 in the test-bed environment.
First of all, the training process of FedLamp and the baselines are shown in Fig. \ref{fig:testbed_Cifar10_1} and Fig. \ref{fig:testbed_Cifar10_2}.
Furthermore, we show the average waiting time and network traffic consumption of different algorithms
in Fig. \ref{fig:testbed_waiting_time} and Fig. \ref{fig:testbed_bandwidth}.
The results which are similar with the simulation results indicate that FedLamp can achieve similar accuracy with the baselines, but incurs shortest average waiting time and least network traffic, so that FedLamp achieves the fastest convergence rate.
Concretely, the training performance of FedLamp and the baselines is listed in Table \ref{tb:testbed metrics on AlexNet}.
We set the target accuracy as 76\%
as it is the accuracy that all algorithms can achieve.
FedLamp takes 2109s and consumes 1453MB network traffic to achieve the target accuracy, which are the best performance compared with the baselines.
ADP with dynamic local updating frequency takes less waiting time and converges faster than FedAvg, so that ADP saves more
network traffic consumption than FedAvg.
For instance, FedAvg needs 13450s and 10257MB network traffic while ADP needs 10508s and 9134MB network traffic when they achieve the target accuracy.
Qsparse and FFL with model compression save a lot of network traffic and reduce the communication time. 
Thus, their average waiting time is less than that of ADP and FedAvg.
Qsparse takes 6748s and consumes 1886MB network traffic while FFL only needs 4697s but consumes more network traffic (3488MB). 
This is because FFL with dynamic local updating frequency can further speed up training compared to Qsparse but cannot achieve lower model compression ratio than Qsparse.
In a word, compared to the baselines (FFL, Qsparse, ADP, FedAvg), FedLamp can reduce the traffic consumption by 58\%, 22\%, 84\%, 85\% and the completion time by 55\%, 68\%, 79\%, 84\%, respectively.
The test-bed results further prove the effectiveness and efficiency of our FedLamp.



==> content/intro-backup-0722.tex <==
%%%NAS
%With the rapid development of artificial intelligence (AI) and the Internet of Things (IoT), AI applications continue to infiltrate every aspect of our daily lives. 
%Deep neural network (DNN), as one of its core technologies, has made remarkable breakthroughs in various fields\cite{AI}. 
%In particular, the emergence of large models, such as ChatGPT\cite{chatgpt}, LLaMA\cite{llama}, etc., has brought excellent performance for natural language processing, image recognition, speech processing and other tasks\cite{nlp,imageRecognition,speech,programmingbugs}. 
%Due to the need for high efficiency and real-time performance, the tasks generated by many AI-based applications are often computationally intensive and delay-sensitive, such as smart homes and intelligent transportation\cite{aibased}. 
%However, most mobile edge devices, due to resource constraints such as limited computing power, storage capacity and energy supply\cite{first,MEC}, struggle to satisfy the Quality-of-Service (QoS) of these intelligent applications.
%
%Offloading tasks to the cloud is a common strategy when mobile edge devices have limited resources. 
%Cloud servers typically have more computing power and storage capacity, and are able to perform compute-intensive tasks more efficiently, which helps to improve the inference speed of the models\cite{cloud1,cloud2}. 
%However, edge mobile devices mainly rely on wireless network connections to offload tasks to the cloud. 
%The long-distance transmission can lead to large communication delays and data transmission energy consumption\cite{clouddelay,cloudenergy}, which is not affordable for real-time applications and battery-powered edge mobile devices.
%In addition, storing and processing data in the cloud can involve security and privacy concerns\cite{security}. Once a user's sensitive data leaves the local environment, it may be exposed to potential risks such as data breaches or unauthorized access.

% \rednote{The construction of 5G smart cities relies on high-speed communication between a massive number of Internet of Things (IoT) devices. 
% Currently, video surveillance, road traffic flow analysis and abnormal accident detection are widely used in Intelligent Transportation Systems (ITS). 
% Cameras within the system transmit video data to the computing platforms where deep learning (DL) models are deployed. 
% In particular, with the rapid development of DL, large-scale models exhibit better performance in these applications due to their extensive parameters and calculations. 
% However, these applications often have stringent real-time requirements. 
% In the traditional cloud computing paradigm, data must be transmitted to distant cloud centers for processing, making it challenging to guarantee low response times, especially when a large volumes of data must traverse congested network.}%这部分简化下，另外背景也需要一些参考文献进行支撑。

% With the development of 5G smart cities, smart street lights, as a basic infrastructure, amounted to 23 million units worldwide by the end of 2022 and are expected to reach 63.8 million by 2027 \cite{report2023}. 
% Besides the lighting function, these street lights can serve as a general platform for many other intelligent services. 
% For example, surveillance cameras can be deployed to analyze traffic patterns, monitor public safety, or detect abnormal accidents\cite{yong2023implementation,mahoor2020state}.
% Supported by 5G edge servers, data from various monitoring devices can be analyzed and processed efficiently near the data source, significantly improving the real-time performance of task response. 
% Additionally, deploying deep learning (DL) models at the network edge enables more intelligent data analysis.
% To boost the performance of these services, it is necessary and practical to augment the parameters of DL models\cite{nakkiran2021deep}.
% Models such as GPT\cite{chatgpt} and LLaMA\cite{llama}, both have more than a billion parameters and can provide more accurate and comprehensive insights for time-series data\cite{gruver2024large}.
% However, since the memory and computational constraints, a single edge server often struggle with storage and processing demands of these large-scale models.

With the development of 5G smart cities, smart street lights, as a kind of critical infrastructure, have been earning much global attention. 
The global installed base of the street lights have reached 23 million by 2022, and are expected to reach 63.8 million by 2027 \cite{report2023}.
Besides the lighting function, these street lights can serve as a general platform for many other public services. 
For example, surveillance cameras can be deployed to analyze traffic patterns, monitor public safety, or detect abnormal accidents \cite{yong2023implementation,mahoor2020state}.
Besides, with the help of 5G edge servers, data from various end devices can be processed and analyzed near the data source, significantly improving the response performance of real-time services\cite{shi2016edge}. 
% Besides, deep learning (DL) models can be deployed at the network edge to enable more intelligent data analysis.
To further boost the performance of these services, deep learning (DL) models, especially the large-scale models (\eg, GPT\cite{chatgpt} and LLaMA\cite{llama}),  can be deployed at the network edge to enable more intelligent data analysis\cite{gruver2024large}.
% the large-scale models (\eg, GPT\cite{chatgpt} and LLaMA\cite{llama}) with more than a billion parameters are expected to be employed\cite{gruver2024large}.
% However, due to the memory and computational constraints of the edge nodes (\eg, end devices or edge servers), it is difficult even infeasible to run these large-scale models on each edge node.
However, due to the memory and computational constraints of the edge nodes (\eg, surveillance cameras or edge servers), it is difficult even infeasible to run these large-scale models on each edge node.

% These smart street lights are equipped with surveillance cameras to serve as a general platform for many other intelligent service, such as traffic patterns analysis, public safety monitoring, and abnormal accidents detection, with the help of 5G edge servers.
% Specifically, the data collected by various smart street lights would be transmitted to the near edge servers for analysis and processing by the deep learning models.
% To provide more accurate and comprehensive insights for time-series data, it is necessary and practical to deploy larger and more efficient models (\eg, GPT\cite{chatgpt} with 13 billion parameters and LLaMA\cite{llama} with 7 billion parameters ).
% However, due to the memory and computational constraints of the edge server, it is difficult even infeasible to deploy these large-scale models on the single edge server.


% To meet the resource constraints on edge servers, model partitioning has been proposed to cooperate the computing resources of multiple edge servers\cite{mirhoseini2017device,gao2023Task,fan2023joint,exit1}.
% Model partitioning involves dividing a large-scale model into several sub-models and distributing them across multiple edge servers.
% By processing only a sub-model that is much smaller than the original model, each edge server experiences a significantly reduced memory and computational burden\cite{yu2021gillis,li2024distributed,tang2020joint}.
% While model partitioning significantly optimizes resource utilization, efficiently offloading tasks in multi-server systems remains a critical challenge. 
% Specifically, model partitioning decomposes the original task into multiple interdependent sub-problems(\eg, some subtasks must wait for the results of other subtasks before execution), which makes the task offloading strategy more complex. 
% By implementing an optimal task offloading strategy, each subtask can be dynamically allocated to the most suitable edge server, which can further improve the execution efficiency of the system\cite{2partition2}.


To meet the resource constraints on edge servers, existing works mainly focus on model compression \cite{ganesh2021compressing,choudhary2020comprehensive} and model partitioning \cite{mirhoseini2017device,gao2023Task,fan2023joint,exit1}. 
Although model compression can significantly reduce computational and storage requirements through techniques such as quantization and pruning, it often results in a certain or even unbearable accuracy loss. 
Additionally, many model compression techniques rely on specific software or hardware support (\eg, low-precision calculations with TensorRT and GPU\cite{li2021unleashing}), or require much extra time for additional adjustments (\eg, architecture search for pruning\cite{dong2019network}).
Compared with model compression, model partitioning can coordinate multiple nodes to train or infer large-scale models without compromising accuracy.
% Compared with model compression, model partitioning can coordinate the computing resources of multiple nodes to train or infer large-scale models without compromising accuracy.
In edge scenarios, a large-scale model can be divided into several sub-models, each of which is distributed to an edge node. 
Accordingly, a complete inference task is divided into several subtasks, which are processed by the nodes holding the corresponding sub-models with reduced memory and computing burden.
% and distributed across multiple edge nodes, with each edge node solely processing the subtask derived from its sub-model, so as to reduce the memory and computing burden of each edge node. 
Considering the dependency relationship of the sub-models, a predecessor node (\ie, a node holds a sub-model whose output is the input of another sub-model) will transmit the intermediate features (\ie, the output of an intermediate sub-model) to a successor node, until the inference through all sub-models is completed.
% After completing the processing of the subtask, each edge node transmits the intermediate feature (\ie, the output of sub-model) to the edge node where the next sub-model is deployed, until the inference through all sub-models is completed.
Some works\cite{2partition1,fan2023joint,exit1,partition1} propose to divide the model into two parts and separately distribute to the edge nodes for collaborative inference.
% end devices and edge servers, then tasks can be partially processed on end devices before being offloaded to edge servers, which reduces the computing load and energy consumption.%
However, this coarse-grained model partitioning has limited ability to reduce model size, which may still lead to overload on the nodes.
To further reduce the computing load, some works propose to coordinate multiple edge nodes with a fine-grained model partitioning\cite{yu2021gillis,li2024distributed,tang2020joint}.
For instance, Tang \textit{et al}.\cite{tang2020joint} divide a large-scale model into multiple (\textgreater2) sub-models and propose a multi-task learning approach to assign each sub-model to an appropriate edge node.
% For instance, Yu \textit{et al}.\cite{yu2021gillis} propose Gillis, which divides a large-scale model across multiple edge nodes for parallel execution, and they employs a dynamic programming based model partitioning strategy to minimize inference latency.

Although fine-grained model partitioning can offload the subtasks to better adapt the capabilities of different edge nodes, the many-to-many dependency between edge nodes (\ie, a node may receive the intermediate features from multiple precursor nodes and can transmit its features to multiple successors) leads to more complex task offloading strategies.
Therefore, it is technically challenging to offload each subtask to an appropriate edge node to prevent nodes from being overloaded and enhance resource utilization.
In addition, the optimization of task offloading strategy also suffers from two other critical challenges in practical applications.
\textbf{1)Heterogeneous System.} Edge nodes typically possess limited and heterogeneous resources\cite{li2022pyramidfl,lim2020federated}. 
For instance, computing and bandwidth capacities may vary by more than tenfold among different edge nodes\cite{chen2022decentralized,lai2021oort}. 
Given the same computing load across different edge nodes, the system heterogeneity can lead to long response delay on weak nodes and waste of resources on strong nodes, significantly impacting the response efficiency.
\textbf{2)Dynamic Environment.} The task arrival rate changes over time and space\cite{ai2023smart}. 
For example, the cameras deployed at the city center or during peak hours will generate more tasks than other places and time periods. 
Additionally, the internal conditions of edge nodes, such as temperature and voltage fluctuations, can affect their computing capabilities\cite{patsias2023task}. 
The dynamic environment leads to imbalanced loads for the edge nodes, and the task offloading strategy needs to be adjusted to adapt to the dynamic environment.
% \textbf{3)Limited Connection.} In the absence of a central server for centralized decision-making, since not all edge nodes have direct communication connections with each other, the nodes cannot obtain the real-time status information of all nodes within the entire network. 
% This limitation can lead to suboptimal task offloading strategy, as edge nodes can only make decisions based on incomplete or outdated information.


Some recent works \cite{tiwary2018response,2partition2} have made the effort to address these challenges.
% So far, some solutions\cite{tiwary2018response,2partition2} to optimize task offloading strategy have been studied for these challenges.
For instance, Tiwary \textit{et al}. propose a non-cooperative game based task offloading (NGTO) method\cite{tiwary2018response} to minimize the task response delay by assigning appropriate computing loads to heterogeneous edge nodes.
However, NGTO requires each node to gather task offloading strategies of others, and update the task offloading strategy in a round-robin manner, which leads to long decision time.
Besides, Mohammed \textit{et al}.\cite{2partition2} propose DINA-O, a approach that offloads multiple interdependent subtasks by matching appropriate edge nodes to balance load and improve resource utilization.
% Besides, Mohammed \textit{et al}.\cite{2partition2} propose DINA-O, a matching game approach that offloads multiple interdependent subtasks by matching appropriate edge nodes to balance load and improve resource utilization.
% to offload multiple interdependent subtasks. 
% Although DINA-O can balance load and improve resource utilization by matching end devices with suitable edge servers, 
But it assumes that edge nodes have fixed computing resources and requires each node can obtain the status information (\eg, available computing resources) of all nodes in time, which cannot adapt to the dynamic network environment.


To realize efficient inference for large-scale models at the network edge, we propose a collaborative inference framework.
% based on model partitioning and early-exiting mechanism. 
% that schedules and balances the computing load of edge nodes with distributed task offloading strategy.
% we introduce an edge collaborative inference framework that enables parallel and pipelined task inference for multiple end devices. 
As illustrated in Fig. \ref{fig:edgecol}, assuming a large-scale model is divided into multiple sub-models, each of which is deployed across multiple edge servers.
% , and the servers collaborate with each other to complete the inference tasks.
The inference tasks are continuously produced by end devices and are offloaded to edge servers for processing.
Considering the dependency of sub-models, the edge servers are arranged to collaboratively work in a pipeline manner, and the input data or intermediate features are processed by the edge servers in sequence.
Before obtaining the inference results, each server will offload subsequent subtasks to the selected successor servers based on its current offloading strategy.
Moreover, the early-exiting mechanism is employed to further accelerate inference by outputing the predicted results before propagating through the final sub-models if the predicted probabilities exceed a confidence threshold.
% Upon the arrival of each task at an end device, it is offloaded to a nearby edge server according to the device's task offloading strategy. 
% After completing the task inference, the edge server similarly selects a successor node and offloads the intermediate features to it for further inference.
% Additionally, we incorporate the early-exiting mechanism into our framework, where the tasks can exit early from some sub-models if their predicted probabilities exceed the confidence threshold.
% , otherwise they are offloaded to the next sub-model for further inference.

% To minimize the response delay of tasks, we develop a distributed task offloading algorithm, termed DTO, where each node is enabled to optimize its task offloading strategy through local communication.
In order to schedule and balance the computing load on edge nodes (\ie, end devices and edge servers), we develop a distributed task offloading algorithm, termed DTO, where each node only needs to share status information with adjacent nodes and dynamically allocates appropriate computing loads for heterogeneous successor nodes.
% Specifically, each node only needs to share status information with adjacent nodes and dynamically allocates different computing loads for heterogeneous successor nodes tailored to their capabilities.
% Specifically, each node only needs to share status information with adjacent nodes and dynamically allocates appropriate computing loads for heterogeneous successor nodes.
Owing to the distributed settings and low computational complexity, DTO can rapidly achieve convergent offloading strategies with few communication rounds, enhancing adaptability to the dynamic environment.
% To minimize the response delay of tasks and avoid node overload, we develop a distributed task offloading algorithm, termed DTO, where each node is enabled to optimize its task offloading strategy through local communication.
% Specifically, each node only needs to share status information with adjacent nodes and dynamically allocates different computing loads for heterogeneous successor nodes tailored to their capabilities.
% Owing to the distributed settings and low computational complexity, DTO can rapidly achieve convergent offloading strategies with few communication rounds, enhancing adaptability to the dynamic environment.
% Moreover, we dynamically adjust the confidence threshold based on the computing loads of edge nodes.
As for the early-exiting decision, a lower confidence threshold will allow more tasks to exit at the earlier edge nodes\cite{laskaridis2021adaptive}, which contributes to shorter inference delay and less computing load on the subsequent edge nodes, but potentially results in more accuracy loss, and vice versa.
% Furthermore, the task offloading strategy also influences how computing loads are distributed across different edge nodes, which in turn affects subsequent decisions regarding both the offloading strategy and the confidence threshold.
% Meanwhile, the task offloading strategy also affects the distribution of computing load on different edge nodes, and the computing load in turn influences the decisions of task offloading strategy and confidence threshold. 
Therefore, we need to consider the interaction between the task offloading strategy and the confidence threshold, and jointly optimize them to achieve the ideal trade-off between task response delay and inference accuracy.
% and the servers collaborate with each other to complete the inference tasks. 
% To accelerate the collaborative inference, it is important and necessary to schedule and balance the computing load of participating edge nodes.
% Given the absence of a central server to produce centralized decisions, we develop a distributed task offloading algorithm, termed DTO, where each node is enabled to optimize its task offloading strategy without the status information of all nodes.
% Specifically, each node only needs to share status information with adjacent nodes and dynamically allocates different computing loads for heterogeneous successor nodes tailored to their capabilities.
% Owing to the distributed settings and low computational complexity, DTO can rapidly achieve convergent offloading strategies with few communication rounds, enhancing adaptability to the dynamic environment.
% Given the limited connections and the absence of a central server to perform centralized decisions, we develop a distributed task offloading algorithm, termed DTO, where each node is enabled to optimize its task offloading strategy through local communication with adjacent nodes.
% Specifically, DTO uses local communication to share resource information and dynamically allocates different computing loads for heterogeneous edge nodes tailored to their capabilities.
% Additionally, DTO can rapidly achieve convergent offloading strategies with fewer communication rounds, enhancing adaptability to the dynamic environment.
% Considering the dependencies between subtasks, it is quite challenging to optimize the overall inference efficiency through local information.
% In this collaborative inference framework without a central server for centralized decision-making, we propose a distributed algorithm, termed DTO, which optimizes the task offloading strategy of each edge node to balance the load and minimize task response delay.
% Specifically, DTO dynamically allocates different computing loads for heterogeneous edge nodes tailored to their capabilities.
% Additionally, DTO only relies on local communication between adjacent edge nodes to share resource utilization information, and rapidly achieves convergent offloading strategies with fewer communication rounds, enhancing adaptability to the dynamic environment.
% Considering the dependencies between subtasks, DTO estimates the total remaining processing delay of subsequent subtasks through queuing theory to optimize the task offloading strategy. 
% % By estimating the comprehensive remaining processing delay of subsequent subtasks through queuing theory, DTO can effectively offload interdependent subtasks.
% % DTO estimates task delays through queuing theory and relies only on local communication.
% % By sharing resource utilization information and estimating the comprehensive remaining processing delay of subsequent subtasks, DTO employs gradient descent to quickly update task offloading strategies. 
% % DTO models task delays through queuing theory, and enables edge nodes to share resource utilization information and estimate the comprehensive remaining processing time of subsequent subtasks through local communication. 
% % Additionally, DTO employs gradient descent to quickly update task offloading strategies based on resource utilization information and remaining time information from heterogeneous edge nodes, thus efficiently manage the offloading of interdependent subtasks in heterogeneous system and dynamic environment.
% To further reduce latency and save computing resources, we incorporate the early-exiting mechanism into our framework, which helps to output the inference results of some simple tasks in advance without propagating through all the sub-models.
% % , which allows some simple tasks exit early from certain sub-models if their predicted probability exceeds the confidence threshold.
% Generally, a lower confidence threshold will allow more tasks to exit at the earlier edge nodes\cite{laskaridis2021adaptive}, which contributes to shorter inference delay and less computing load on the subsequent edge nodes, but potentially results in more accuracy loss, and vice versa.
% Furthermore, the task offloading strategy influences how computing loads are distributed across different edge nodes, which in turn affects subsequent decisions regarding both the offloading strategy and the confidence threshold.
% % Meanwhile, the task offloading strategy also affects the distribution of computing load on different edge nodes, and the computing load in turn influences the decisions of task offloading strategy and confidence threshold. 
% Therefore, we need to consider the interaction between the task offloading strategy and the confidence threshold, and jointly optimize them to achieve the ideal trade-off between task response delay and inference accuracy.
%与此同时，任务卸载策略也会影响计算负载在不同边缘节点上的分布，因此我们需要考虑到任务卸载策略和置信度阈值的相互作用，通过联合优化任务卸载策略和置信度阈值去实现任务响应时延和推理精度的权衡
% Moreover, since the fine-grained model partitioning results in multiple intermediate feature transmissions and increased transmission time, we employ the early exit mechanism to further reduce latency.%%%%
% Through the early exit mechanism, some simple tasks can exit early in some sub-models if their predicted probability exceeds the confidence threshold.
% % by early exit mechanism, early exit branches are added to some sub-models to allow simple tasks to exit early.
% % Whether a task exits early depends on whether its predicted probability at the branch exceeds the predefined confidence threshold.
% Generally, a lower confidence threshold allows more tasks to exit early on the former nodes\cite{laskaridis2021adaptive}, which contributes to reduce the delay and the computational load at the later nodes, but potentially compromising accuracy, and vice versa.
% Therefore, we dynamically adjust the confidence threshold of each early exit branch to balance the response delay and inference accuracy of tasks.
% Furthermore, it is crucial to consider the interaction between the task offloading strategy and the confidence threshold.
% Specifically, task offloading strategies determine workload distribution across edge servers, which influences the overall computational load of system. 
% Meanwhile, the confidence threshold for early exit mechanisms must be adjusted dynamically to balance inference accuracy and response delay according to current load and resource availability.
% By jointly optimizing the task offloading strategy and the confidence threshold, we aim to achieve an efficient edge cooperative inference framework. 
Our main contributions are as follows:
\begin{itemize}
\item 
To enable the deployment of large-scale models at the edge, we propose a collaborative inference framework, which coordinates multiple edge nodes and employs early-exiting mechanism to provide low-latency task inference.
% Based on \rednote{model partitioning} and early-exiting mechanism, this framework coordinates multiple edge nodes to provide low-latency task inference.
\item 
We propose a distributed task offloading algorithm DTO, which estimates the processing delay of tasks through queuing theory. 
By jointly optimizing the task offloading strategies of edge nodes and the confidence thresholds of multiple exit branches, DTO can achieve the promising trade-off between response delay and inference accuracy.
\item 
We investigate the effects of various system settings on the performance of DTO. 
Compared with other baselines, simulation results show that DTO can reduce the average response delay by 21\%-41\% and improve the inference accuracy by 1\%-4\%.
% Simulation results show that DTO outperforms other baselines in a wide range of parameter settings.
\end{itemize}
% The rest of this paper is organized as follows. 
% Section \ref{sec:prelim} gives the system modeling and problem definition. We introduce DTO in Section \ref{sec:alg}, evaluate its performance through simulation experiments in Section \ref{sec:results}, Section \ref{sec:related} introduces related works, and Section \ref{sec:conclusion} concludes this paper.


% Some works propose to use edge devices or cloud to alleviate the computing load of edge servers by model partitioning\cite{2partition1,fan2023joint,exit1,partition1}.
% For instance, Gao \textit{et al}.\cite{2partition1} divide the model between devices and edge servers, and they jointly optimize model partitioning and task scheduling to minimize computational latency and energy consumption of each device.
% However, these works only consider dividing the model into two parts, and this coarse-grained model partitioning still does not work well for resource-constrained edge devices.
% To further reduce the computing load, some works propose to coordinate multiple edge servers with fine-grained model partitioning\cite{yu2021gillis,li2024distributed,tang2020joint}.
% For instance, Yu \textit{et al}.\cite{yu2021gillis} propose Gillis, which divides a large-scale model into multiple computing nodes for parallel execution, and they employs a dynamic programming based model partitioning strategy to minimize inference latency.
% However, without being considered by these works, fine-grained model partitioning decomposes a task into multiple interdependent subtasks (\eg, some subtasks must wait for the results of other subtasks before starting execution), leading to more complex task offloading strategies.

% A excellent task offloading strategy can balance computing load and improve resource utilization.
% Apart from the dependencies between subtasks, the optimization of task offloading strategy still suffers from three other critical challenges in practical applications.
% \textbf{1)System Heterogeneity.} Edge servers typically possess limited and heterogeneous resources\cite{li2022pyramidfl,lim2020federated}. For instance, computing and bandwidth capacities may vary by more than tenfold among different edge servers\cite{chen2022decentralized,lai2021oort}. Resource-constrained edge servers can lead to severe network congestion and computational overload, significantly impacting the task response latency.
% \textbf{2)Dynamic Environment.} the distribution of tasks changes over time and space\cite{ai2023smart}. For example, the cameras in the city center and during peak hours will generate more tasks than other places and times. Additionally, the internal conditions of edge servers, such as temperature and voltage fluctuations, can affect their computing capabilities\cite{patsias2023task}. The dynamic environment leads to imbalanced loads on edge servers, affecting the efficiency of system.
% \textbf{3)Unavailable Global Information.} Due to the dynamic environment and limited communication range, it is difficult to collect global real-time information of the entire network.
% Unavailable global information often results in suboptimal task offloading strategy, where tasks may be offloaded to inappropriate edge nodes.


% So far, many solutions\cite{tiwary2018response,2partition2} to optimize task offloading strategy have been studied for these challenges.
% For instance, Tiwary \textit{et al}.\cite{tiwary2018response} propose non-cooperative game based task offloading (NGTO) for multiple users to multiple edge servers. Although NGTO accounts for the heterogeneous capabilities of edge servers, users need to update the task offloading strategy in a round-robin way, leading  to a long decision time.
% Moreover, Mohammed \textit{et al}.\cite{2partition2} divide a large CNN task into multiple subtasks, and propose DINA-O, an matching game approach to offload subtasks. Although DINA-O can achieve load balancing and improve resource utilization, it assumes that computing nodes have stable computing resources, and users need to obtain and update network and node status information in real time, which can not adapt to the dynamical edge environment.




% % With the construction of 5G smart cities, smart street lights are becoming increasingly popular. 
% % The global installed base of smart street lights amounted to 23 million units at the end of 2022, and the number is expected to reach 63.8 million by 2027\cite{report2023}.
% % Cameras can be deployed on smart street lights to provide video data for real-time applications, such as video surveillance, traffic flow analysis, abnormal accident detection\cite{yong2023implementation,mahoor2020state}.
% % To improve the real-time performance of task processing, data can be analyzed and processed in 5G edge computing servers, which are located close to the data source\cite{EC1,delay}.
% % Additionally, to boost the performance of these applications or services, it is necessary and practical to augment the parameters of DL models\cite{nakkiran2021deep}.
% % % Additionally, large-scale models can be used to perform intelligent analysis of time-series data like video streams\cite{bharadiya2023artificial}, thereby enhancing the detection and recognition of special events, such as traffic accidents and illegal parking.
% % However, deploying large-scale models on a single edge server remains challenging due to their extensive parameters and computational requirements. 
% % Models like GPT\cite{chatgpt} and LLaMA\cite{llama}, each with over a billion parameters, significantly exceed the capacity of most edge servers.


% % To meet the resource constraints on edge servers, existing works mainly focus on model compression \cite{ganesh2021compressing,choudhary2020comprehensive} and model partitioning \cite{mirhoseini2017device,gao2023Task,fan2023joint,exit1}. 
% % Although model compression can significantly reduce computational and storage requirements by the techniques like quantization and pruning, it often results in a certain or even unbearable accuracy loss. 
% % Besides, many model compression techniques rely on specific software or hardware support (\eg, low-precision calculations with TensorRT and GPU\cite{li2021unleashing}) or require much extra time for additional adjustments (\eg, architecture search for pruning\cite{dong2019network}).
% % % require additional adjustments for inference (such as pruning structure optimization).
% % Compared with model compression, model partitioning can coordinate the computing resources of multiple devices to train or infer large-scale models without compromising accuracy.
% % Model partitioning involves dividing a model into several sub-models and distributing them across multiple devices, and it was originally proposed to train large-scale model on GPUs.
% % % This technique can effectively utilize resources, reduce the computational burden on individual devices, and enhance the overall system efficiency.
% % % Some works focus on how to partition models. 
% % Wang et al.\cite{wang2019supporting} proposed Tofu, which trains large-scale models across multiple GPU devices to reduce per-GPU memory usage, and they use a recursive search to find the best model partitioning plan that minimizes communication overhead.
% % Similarly, Jia et al.\cite{jia2019beyond} proposed FlexFlow for training large-scale model on GPU clusters, and they use guided randomized search to find a efficient parallel strategies that enhance training throughput.  
% % % By model partitioning, we can coordinate the computing resources of multiple devices to train or infer large-scale models without losing accuracy.
% % % b等人提出FlexFlow，它使用引导随机搜索来找到一个efficientt parallelization strategies，在GPU集群中加速训练。
% % %通过模型分割，我们可以可以协同多个设备的计算资源去训练或推理大模型而不损失精度。
% % % In order to properly partition the models, Mirhoseini $\eta$ [11] employ reinforcement learning to optimize models segmentation allocation strategies.
% % % \rednote{Existing research on model partitioning includes methods like using reinforcement learning to optimize device placement strategies and find optimal model segmentation and device allocation strategies \cite{mirhoseini2017device}.} %句子太长 
% % % Moreover, Jia $\eta$ \cite{jia2018exploring} investigate the parallelization strategy of convolutional neural networks by automated search technology. 
% % %在GUP或云中心上训练大模型
% % % However, these model partitioning methods are often complex, especially for large-scale models with numerous layers. 
% % % Additionally, dynamic changes in the available computing power and memory at different edge nodes further complicate the model partitioning strategy.

% % In edge scenarios, end devices offload computing-intensive tasks to edge servers, which may cause overload of the edge servers. 
% % Some works use model partitioning to reduce the memory usage and computing load of a single edge server.
% % For instence, Gao et al.\cite{2partition1} divide the model between devices and edge servers, and they jointly optimize model partitioning and task scheduling to minimize computational latency and energy consumption of each device.
% % Morever, Fan et al.\cite{fan2023joint} present a three-layer architecture consisting of user, edge server and cloud, and jointly optimize model partitioning strategy and resources allocation to minimize the processing delay of all tasks.
% % Howerer, these works only consider dividing the model into two or three parts, and this coarse-grained model partitioning still does not work well for resource-constrained edge devices.
% % Some works further reduce the computing load with more fine-grained model partitioning.
% % Yu et al.\cite{yu2021gillis} propose Gillis, which divides a large-scale model into multiple computing nodes for parallel execution, and they employs a dynamic programming based model partitioning strategy to minimize inference latency.
% % Beside, Li et al.\cite{li2024distributed} investigate distributed deep neural network(DNN) inference with collaborations between edge servers and edge devices, and they propose an asynchronous advantage actor-critic approach to find a model partitioning strategy that reduces DNN inference delay.
% % These works use fine-grained model partitioning to enable the system to process tasks in parallel or pipeline, which improves the utilization of computing resources and avoids the overload of a single edge server.
% % However, without being considered by these works, fine-grained model partitioning decomposes a task into multiple interdependent subtasks (\eg, some subtasks must wait for the results of other subtasks before starting execution), leading to more complex task offloading strategies.
% % Additionally, optimizing the task offloading strategy still suffers from three other critical challenges in practical applications.
% % \textbf{1)System Heterogeneity.} Edge servers typically possess limited and heterogeneous resources\cite{li2022pyramidfl,lim2020federated}. For instance, computing and bandwidth capacities may vary by more than tenfold among different edge servers\cite{chen2022decentralized,lai2021oort}. Resource-constrained edge servers can lead to severe network congestion and computational overload, significantly impacting the task response latency.
% % \textbf{2)Dynamic Environment.} the distribution of tasks changes over time and space\cite{ai2023smart}. For example, the cameras in the city center and during peak hours will generate more tasks than other places and times. Additionally, the internal conditions of edge servers, such as temperature and voltage fluctuations, can affect their computing capabilities\cite{patsias2023task}. The dynamic environment leads to imbalanced loads on edge servers, affecting the efficiency of system.
% % \textbf{3)Unavailable Global Information.} Due to the dynamic environment and limited communication range, it is difficult to collect global real-time information of the entire network, outdated global information can lead to bad decisions. 
% % To address these challenges, some works focus on optimizing task offloading strategy.
% % For instance, Tiwary et al.\cite{tiwary2018response} propose non-cooperative game based task offloading (NGTO) for multiple users to multiple edge servers. Although NGTO accounts for the heterogeneous capabilities of edge servers, users need to update the task offloading strategy in a round-robin way, leading  to a long decision time.
% % Moreover, Mohammed et al.\cite{2partition2} divide a large CNN task into multiple subtasks, and propose DINA-O, an matching game approach to offload subtasks. Although DINA-O can achieve load balancing and improve resource utilization, it assumes that computing nodes have stable computing resources, and users need to obtain and update network and node status information in real time, which can not adapt to the dynamical edge environment.





% To avoid the load bottleneck of edge servers, we propose an edge collaborative inference framework that provides parallel and pipelined task inference for multiple users, as illustrated in Figure \ref{fig:edgecol}.
% This framework divides a large-scale model into multiple sub-models based on model partitioning, and deploys each sub-model to multiple edge servers.
% Additionally, to balance the load and reduce the response delay of tasks, we propose a distributed algorithm DTO to optimize the task offloading strategies of edge devices and edge servers.
% DTO is better adapted to heterogeneous systems and dynamic environments by allocating appropriate computational loads to heterogeneous edge servers and relying only on fast local communication.
% Furthermore, since fine-grained model partitioning results in multiple intermediate feature transmissions and increased transmission time,  we employ the early exit mechanism to further reduce latency at the cost of some accuracy loss.
% by early exit mechanism, early exit branches are added to some sub-models to allow simple tasks to exit early.
% Whether a task exits early depends on whether its predicted probability in the branch exceeds the confidence threshold.
% Generally, a higher confidence threshold results in higher overall accuracy but decreases the number of tasks that exit early, leading to a longer average response delay\cite{laskaridis2021adaptive}. 
% Therefore, we dynamically adjust the confidence threshold of each early exit branch to balance the response delay and inference accuracy of tasks.
% In short, our main contributions are as follows:
% \begin{itemize}
% 	\item [1)]
% 	To enable the deployment of large-scale models at the edge, we propose an edge collaborative edge architecture. Based on model partitioning and early exit mechanism, this architecture coordinates the resources of multiple edge nodes to provide low-latency computing services.
% 	\item [2)]
% 	We propose a distributed algorithm DTO, which jointly optimize the task offloading strategy of edge nodes and the confidence threshold of multiple exit branches by local information, achieving the optimal balance between response delay and inference accuracy.
% 	\item [3)]
% 	We investigate the effects of various system settings on the performance of the distributed algorithms. Simulation results show that DTO  outperforms other baselines in a wide range of parameter settings.
% \end{itemize}
% The rest of this paper is organized as follows. 
% Section \ref{sec:prelim} gives the system model and problem definition. We introduce our distributed algorithm in Section \ref{sec:alg}, evaluate its performance through simulation experiments in Section \ref{sec:results}, Section \ref{sec:related} introduces the relevant work, and Section \ref{sec:conclusion} concludes this paper.



% Many other works focus on optimizing task offloading in edge networks through model partitioning. 
% For instance, the research \cite{kang2017neurosurgeon} proposes to automatically divides the model into user and server segments at the neural network layer granularity to minimize response latency.
% % For instance, \rednote{one study automatically divides the model into user and server segments at the neural network layer granularity to minimize response latency\cite{kang2017neurosurgeon}. } %参考我们的论文，一般我们不会用one study, another approach来引出相关工作。
% Besides, the authors in \cite{gao2023Task} consider the scenario involving multiple mobile devices and a single edge serve, and optimize the task partitioning and offloading strategies to minimize costs per mobile device.
% % \rednote{Another approach} considers the scenario involving multiple mobile devices and a single edge server, where the model is split into two parts deployed on mobile devices and edge server, respectively, \rednote{optimizing task partitioning and offloading to minimize costs per mobile device\cite{gao2023Task}. }%少用这种从句
% Furthermore, the researchers \cite{fan2023joint} present a three-layer architecture consisting of user, edge server and cloud, and jointly optimize model partitioning strategies and the allocation of computing and communication resources to minimize the processing delay of all tasks. 
% Additionally, the authors in \cite{exit1} propose an adaptive edge inference framework based on model partitioning and multi-exit deep neural networks (DNNs), they balances the number of completed tasks and average inference accuracy by optimizing exit points and partition points for each task\cite{exit1}.
% % Additionally, an adaptive edge inference framework based on model partitioning and multi-exit deep neural networks (DNNs) has been proposed. This framework, consisting of an edge node and several mobile devices, balances the number of completed tasks and average inference accuracy by optimizing exit points and partition points for each task\cite{exit1}.
% However, these works primarily focus on obtaining the optimal model partitioning strategy, overlooking the parallel needs of multiple users for large-scale models and failing to optimize task offloading strategies for multiple edge servers. 
% % \cite{tran2017collaborative,xiao2017qoe,xiao2018distributed}
% % In addition, they typically consider only two-layer or three-layer model partitioning architectures, \rednote{without addressing the potential of using model partitioning to combine the computing resources of multiple edge nodes.}%没看懂你想表达什么意思

% Therefore, we focus on optimizing parallel inference for multiple task flows. 
% Specifically, based on model partitioning, a large model is divided into sequential sub-models, with each task being inferred and offloaded in sequence from one sub-model to the next. 
% Since each sub-model is deployed across multiple edge servers, we optimize the task offloading strategies for each edge node to minimize task response delay.
% Additionally, similar to previous works\cite{exit1,eDeepSave}, we consider using the early exit mechanism, we add early exit branches for some sub-models to allow simple tasks to exit early. 
% This mechanism can further reduce task response delay at the cost of some precision loss.
% Since the early exit decision and inference precision depend on the confidence thresholds of the exit branches, we optimize the confidence threshold of each early exit branch to balance the inference precision and response delay of tasks.
% In summary, based on model partitioning and early exit mechanism, we propose an edge cooperative inference architecture, as illustrated in Figure \ref{fig:edgecol}. To achieve the optimal trade-off between response delay and inference precision for multiple task flows, we jointly optimize the task offloading strategy of each edge node and the confidence threshold of each branches.

% % Therefore, we focus on optimizing parallel inference for multiple task flows. 
% % Specifically, based on model partitioning and \rednote{the early exit mechanism}, %这里早退机制可以后面再引出，这里我觉得你应该重点说明，我们是通过任务卸载与调度来缓解各边缘节点的计算压力，缩小任务处理的响应时间。
% % we propose an edge cooperative inference architecture, as illustrated in Figure \ref{fig:edgecol}. 
% % In this architecture, a large-scale model with multiple early exit branches is divided into several sub-models, each deployed to different edge servers. 
% % Multiple task flows are inferred in parallel within this architecture. After a task is processed on a sub-model, it is offloaded to the edge server hosting the next sub-model, continuing this process until the task completes inference on all sub-models or exits early at a model branch.
% % For this edge cooperative inference architecture, to achieve the optimal trade-off between inference response delay and inference precision for multiple task flows, we jointly optimize the task offloading strategy for each edge node and the confidence threshold for multiple branches of the model. 


% We can reduce the resource requirements for deploying large-scale models and collaboratively utilize the resources of multiple edge servers through model partitioning. 
% Additionally, by implementing the early exit mechanism, we can further reduce the response delay at the cost of a partial loss in inference accuracy. 
% Through the joint optimization of task offloading strategy and the confidence thresholds, we can balance the load across multiple edge servers, and achieve an optimal trade-off between response delay and inference accuracy.
% Although the edge collaborative inference framework offers significant advantages, it faces three critical challenges in practical applications:
% \textbf{1)System Heterogeneity.} Edge servers typically possess limited and heterogeneous resources\cite{li2022pyramidfl,lim2020federated}. For instance, computing and bandwidth capacities may vary by more than tenfold among different edge servers\cite{chen2022decentralized,lai2021oort}. Resource-constrained edge servers can lead to severe network congestion and computational overload, significantly impacting the task response latency.
% \textbf{2)Dynamic Environment.} the distribution of tasks changes over time and space\cite{ai2023smart}. For example, the cameras in the city center and during peak hours will have more task data than other places and times. In addition, the internal conditions of edge servers, such as temperature and voltage fluctuations, can affect their computing capabilities\cite{patsias2023task}. The dynamic environment leads to imbalanced loads on edge servers, affecting the efficiency of system.
% \textbf{3)Unavailable Global Information.} Due to the dynamic environment and limited communication range, it is difficult to collect global real-time information of the entire network, outdated global information can lead to bad decisions. 

% To expand the ability of addressing the above challenges for efficient edge cooperative inference framework, we propose a distributed algorithm DTO. The design of DTO is based on two fundamental observations. 
% 1) Based on model partitioning, each sub-model is deployed across multiple edge servers with varying capabilities. 
% Inspired by the previous work\cite{car,ma2021adaptive}, assigning appropriate workload to different edge servers helps accommodate their varying capabilities. 
% We optimize the task offloading strategy for each node, for instance, tasks can be primarily offloaded to the edge servers with rich computing resources and bandwidth resources to prevent the resource-constrained edge server from becoming the bottleneck of response speed.
% 2)The early exit mechanism allows simple tasks to exit early, reducing the resource competition among the remaining tasks, so as to reduce the average response delay. 
% Whether a task exits early depend on whether its prediction probability at exit branch exceeds the confidence threshold. 
% Generally, a higher confidence threshold results in higher overall accuracy but decreases the number of tasks exit early, leading to a longer average response delay\cite{laskaridis2021adaptive}. 
% Therefore, We dynamically adjust the confidence threshold to adapt to the system load.
% When the system load is high, we decrease the confidence threshold to reduce overall system congestion and task response delay at the cost of slight accuracy loss. 
% conversely, when the system load is light, we increase the confidence threshold to improve the inference accuracy.


% Motivated by the above insights, DTO explores to build an efficient edge cooperative inference framework by jointly optimizing task offloading strategy and confidence threshold. 
% The difficulty of algorithm design lies in the interaction between task offloading strategy and confidence threshold.
% Specifically, task offloading strategies determine how workloads are distributed across edge servers, which in turn affects the system's overall computational load and network congestion.  
% Meanwhile, the confidence threshold for early exit mechanisms must be dynamically adjusted based on the current load and resource availability to balance inference accuracy and response delay.
% % On the one hand, to balance the precision and delay, it is desired to select an appropriate confidence threshold to balance the precision and delay. 
% % However, Due to the change of system load, the task offloading strategy must be readjusted to minimize the average response delay.
% % On the other hand, to fully utilize the resources of heterogeneous nodes, the task offloading strategy needs to assign different computing and bandwidth loads to various nodes, This requires dynamically selecting an appropriate confidence threshold to balance delay and accuracy.
% Only by jointly optimizing task offloading strategy and confidence threshold can DTO realize an efficient edge cooperative inference framework. 
% In a nutshell, our main contributions are as follows:
% \begin{itemize}
% 	\item [1)]
% 	To enable the deployment of large-scale models at the edge, we propose an edge collaborative edge architecture. Based on model partitioning and early exit mechanism, this architecture coordinates the resources of multiple edge nodes to provide low-latency computing services.
% 	\item [2)]
% 	We propose a distributed algorithm DTO, which jointly optimize the task offloading strategy of edge nodes and the confidence threshold of multiple exit branches by local information, achieving the optimal balance between response delay and inference accuracy.
% 	\item [3)]
% 	We investigate the effects of various system settings on the performance of the distributed algorithms. Simulation results show that our distributed algorithm outperforms other baselines in a wide range of parameter settings.
% \end{itemize}
% The rest of this paper is organized as follows. 
% Section \ref{sec:prelim} gives the system model and problem definition. We introduce our distributed algorithm in Section \ref{sec:alg}, evaluate its performance through simulation experiments in Section \ref{sec:results}, Section \ref{sec:related} introduces the relevant work, and summarize this paper in section \ref{sec:conclusion}.


\begin{figure}[!t]
\centering
\includegraphics[width=0.95\linewidth]{./fig2/framework (3).png}
\caption{\label{fig:edgecol}Illustration of collaborative inference of a large model with multiple edge nodes.}
\end{figure}


\begin{comment}


%ED
With the rapid development of AI and the IoT, the IoT devices are becoming increasingly intelligent.
%more and more intelligent. 
AI-based applications appear in various scenarios, such as smart homes, voice assistants, traffic management systems and so on\cite{AI,nlp,imageRecognition,speech,programmingbugs}. 
However, the computational intensity of these AI-based applications often surpasses the capabilities of battery-powered mobile devices (EDs) with constrained resources\cite{first,MEC}.  
%Since the tasks of these AI applications have a high degree of computational complexity, which is unaffordable for battery-powered EDs with limited resources. 
The traditional approach is to offload tasks to the cloud center and use its powerful computational and storage capacities for task inference, which can significantly reduce the computing load and energy consumption of EDs\cite{cloud1,cloud2}. 
%The traditional approach is to offload the task to the cloud center and use the powerful computing and storage resources of the cloud center for task inference, which can significantly reduce the computing burden and energy consumption of EDs. 
Despite its advantages, cloud offloading also presents several challenges.
%However, task offloading to the cloud still has some limitations. 
On the one hand, the lengthy communication path between EDs and cloud center can cause considerable delays, especially when large amounts of data need to pass through the congested networks, which is unacceptable for latency-critical applications\cite{clouddelay,cloudenergy}.
%On the one hand, there is a long distance communication link between the ED and the cloud center, especially when a large amount of data needs to pass through the already congested link, this approach will produce serious communication delays, it is unacceptable for many latency-sensitive tasks. 
On the other hand, transmitting raw data over wide area networks (WAN) to cloud centers raises concerns regarding privacy breaches and data loss\cite{security}.
%On the other hand, the raw data is transmitted to the cloud center through the wide area network (WAN), which may lead to privacy leakage and data loss.

%卸载到边缘
%好处
%Therefore, as an extension of cloud computing, mobile edge computing (MEC) is seen as a promising paradigm that disperses computing resources from the remote cloud to the edge closer to the user\cite{EC1}, such as deploying edge servers near the base stations (BS), and allowing them to inference tasks and manage in a collaborative manner. 
%The edge mobile device offloads the task to the edge servers, which can save the energy consumption of the edge mobile device\cite{energy} and reduce the processing delay of the task\cite{delay}.
%Offloading tasks to edge servers can leverage various resources in the edge environment. However, although the total amount of computing resources and storage resources at the edge is rich, the available resources for a single edge server are still very few compared with the cloud, and its stability is poor\cite{limited}. Therefore, the case of a single edge server in MEC has many limitations.

In order To satisfy the low-latency demands of computing tasks and ensure data privacy, MEC has become a promising paradigm, which decentralizes computing services from remote cloud centers to edge networks\cite{EC1,delay,energy}.
In the MEC network, edge servers are deployed at some nodes that are close to users and have computing capabilities, such as base stations (BS), wireless access points (AP), home gateways, tablets, \etc
EDs can connect these edge servers through the network and offload the computing tasks to nearby edge nodes for inference. 
There is huge potential for MEC, according to IDC data, by 2025, the number of smart devices will grow to 80 billion\cite{reinsel2017data}.
%(是云网络的x倍)
However, due to the challenges of system heterogeneity, dynamic environment and privacy security\cite{khan2019edge}, it is difficult to manage and co-schedule the resources of the edge network uniformly, therefore, the resources of edge network are difficult to be used efficiently.
In addition, more AI-based applications tend to use large-scale models with intensive computation.
With the development of ML, large-scale models have made breakthroughs in many fields, while its parameter scale and the computing resources required have also increasing\cite{aibased}. 
Such as ChatGPT\cite{chatgpt} and LLaMa\cite{llama}, both of them have more than a billion parameters, which are far beyond the capacity of most edge servers in the edge network.
Therefore, we need to consider combining the resources of multiple servers to deploy large-scale models at the edge, which can improve resource utilization of the edge network and provide low-latency AI services.
%
%Therefore, as an extension of cloud computing, mobile edge computing (MEC) becomes a promising paradigm.
%MEC disperses computing resources from the remote cloud center to the edge of the network. 
%In MEC network, the edge servers is deployed on edge nodes with some computing resources, such as base station (BS), wireless access points (APs), home gateway, tablet, etc. 
%EDs can connect these edge nodes through the network and offload the computing tasks to nearby edge nodes for inference.
%In this way, it can not only meet the delay requirements of some computing tasks, but also reduce the energy consumption of ED.
%According to IDC data, by 2025, the number of smart devices will grow to 80 billion, and there is huge potential for edge computing. 
%However, due to challenges such as system heterogeneity, high dynamics and privacy security in edge computing networks, it is difficult to cooperate among edge nodes, the total amount of edge computing power is rich but the resource utilization is low.
%Especially with the development of machine learning(ML), while AI-based large models have made breakthroughs in various fields, its parameter scale and the computing resources required are also increasing.
%Such as ChatGPT and LLama, both of them have more than 1 billion parameters, so it is difficult to deploy such a large model in a single-server MEC network, the computing resources and storage capacity of a single edge node are very limited compared with the cloud center.
%Therefore, we need to utilize multiple edge servers of the MEC network to fuse their resources and manage them collaboratively.


%由于模型大，模型分区
%提前退出
%The best performance of deep learning models in various fields mainly depends on the sufficient computing resources and memory size. 
%%to run large models with a large number of parameters. 
%ChatGPT and LLaMA, for example, each have more than one billion parameters\cite{chatgpt,llama}. Therefore, it is still difficult to directly deploy large models on edge servers with relatively limited resources. 
%In order to make full use of edge network computing resources, model partitioning is a common and effective method. 
%Model partitioning is a technique that splits a deep learning model into different parts(sub-models), each of which can be computed on different computing devices\cite{partition1,partition2,partition3}.
%These computing devices only need to perform calculations in the sub-model and transmit the output of the sub-model which is the intermediate inference result of the entire model. Multiple computing devices cooperate to get the final inference result.
%This process helps to improve the operational efficiency of the model, reduce the complexity of the computational tasks, and support the deployment of the large model in a distributed environment.
%
%Early exit mechanism means that in the inference process of multi-exit model, according to some conditions, an output branch can end the inference in the middle of the model in advance, without waiting for all computation of the entire model to complete\cite{exit1,exit2}. 
%By obtaining part of the output results in advance, it can achieve faster inference speed and save computing resources, which is of great significance in the edge network with high real-time requirements and relatively scarce computing resources.

%Nowadays, many smart home devices are applied to collaborative inference, such as home computing host (NAS), computing router, etc.
%By sharing the computing resources and storage capacity of multiple devices, users can realize the intelligent and personalized upgrade of some IoT device (such as camera, SmartWatch).
%%By sharing the computing resources and storage resources of multiple devices, we can realize the intelligent upgrade of ordinary cameras and personalized services of intelligent language products.
%In addition, the local storage and calculation of user data can ensure the privacy of users.
%%
In order to provide task offloading services to AI-based applications at the edge, model partitioning is proposed to reduce the computing load of edge servers.
%In order to provide better task offloading services to AI-based applications in multi-node MEC networks, we need to consider two problems.
%The first problem is that the resources required by the large model are too large, how to use the limited resources of the edge servers to carry out the task inference of the large model?
%The second problem is which edge server the device should choose to offload the tasks to in multi-node MEC network.
%%%%模型分区
%To solve the first problem, model partitioning is a useful method to solve resource constraints. 
%The completion of AI-based tasks requires inference on the DNN models, which is mainly composed of different types of layers. 
%%layer解释
Model partitioning is to divide the complete model into several consecutive parts (or sub-models) by selecting appropriate segmentation points, and then deploy each part on different edge servers\cite{partition1,partition2,partition3}.
%model partitioning is to divide the complete model into several parts (or sub-models) by selecting appropriate segmentation points, and then deploy each part on different computing nodes.
After each edge server completes the inference of the sub-model, it transfers the intermediate feature to the edge server where the next submodel is deployed.
%After each computing node completes the inference of the sub-model, the intermediate feature is transmitted to the computing node deploying the next sub-model.
Until the task completes inference on all sub-models, we can get the final inference result without loss of accuracy.
%Finally, we can get inference results without loss of accuracy.
In general, model partitioning can reduce the requirement of computing resources and storage resources for each edge server, maximize the resource utilization of the MEC network, but it can bring delay cost due to the transmission of intermediate feature.
%Model partitioning can reduce the requirement of computing resources and storage resources for each node, maximize the resource utilization of the MEC network, but it may bring some delay cost due to the transmission of intermediate feature.
%%%%早退机制
Therefore, some studies have proposed using an early exit mechanism on Deep Neural Network(DNN).
The early exit mechanism refers to inserting several exit branches into the middle of the DNN model without modifying the model backbone.
%There are also studies that propose to use the early exit mechanism on DNN. Without modifying the backbone of the model, we set several branch exits in the middle of the DNN model. 
Each early exit branch can predict the result of the task, and will decide whether to end the task inference based on the confidence of the prediction result\cite{exit1,exit2}.
%When each sample passes through the branch, the sample will decide whether to early exit according to the judgment of the branch on the sample.
Since only shallow layers of DNN and early exit branch are needed to obtain the prediction result of the task, early exit mechanism can reduce delay and computational resources required for inference at the cost of accuracy.
%Since only shallow DNN and early exit branch are needed to obtain the inference result of the sample, without completing the remaining calculation, we can reduce the inference delay and computational resources required by the inference at the cost of partial precision loss. 
In addition, the early exit mechanism can be combined with model partitioning to realize collaborative inference in MEC network.
%%%卸载算法
%Research has focused on distributed task offloading algorithms, where each edge mobile device makes offloading decision in a decentralized manner. 
%the algorithm not only needs to take into account the heterogeneous edge system, each edge server has different computing resources and bandwidth resources; 
%Dynamic edge environments also need to be considered, 
%The load level of the edge server greatly affects the quality of service, and the load level mainly depends on the number of edge mobile devices, task arrival rate, and offload decisions, which may change over time. 
%In addition, due to the dynamic environment, it is difficult for edge mobile devices to collect global real-time information of the entire network, so we can only use limited local information to make offload decisions.
%
%参考文献 [16] 假设 DNN 已被划分为一组固定的分区.[16] 没有优化分区点，而是优化了 MEC 服务器上固定 DNN 分区的部署，以最大限度地减少端到端延迟
%Based on model partitioning and early exit mechanism, multiple edge servers can form an edge cooperative inference system. 
%Edge mobile devices offload tasks to edge servers with the first part of the model, and each edge server sends the results to edge servers with the next part of the model after completing its own part of the inference, until the middle exit of the model in advance or at the end of the model to complete the entire inference process. 
%This inference mode can make full use of the computing resources of edge servers and improve the performance of MEC system. 
%However, in most of the previous relevant work, they mainly focus on the selection of model partition points and early exit. 
%In the research on model partitioning\cite{2partition1,2partition2,2partition3}, most of them mainly reduce the data transmission delay by transmitting intermediate feature smaller than the original data. 
%They generally consider that edge servers have sufficient computing resources and memory capacity. They only consider a single model partition, which divides the model into two parts. One part is deployed on edge mobile devices and the other part is deployed on edge servers. 
%This approach is not feasible for large models with more and more parameters today.
%In the research on early exit mechanism\cite{exit2,exit3}, most of them focus on the selection of the early exit point, but ignore the impact of the early exit mechanism on the burden of the edge server. Therefore, in a distributed environment based on model partitioning, we also need to consider the impact of early exit mechanism on task flow size
%
%and most of the studies only consider a single model partition, they split the model into two parts and introduce it into the cloud center for inference calculation. One part is deployed in the edge server and the other part is deployed in the cloud center, forming a three-layer task offloading framework of edge mobile device-edge server-cloud server. Although this forwarding mode can solve the resource constraint problem of edge system to some extent, it still has the disadvantages of the forwarding mode based on cloud computing, which has large end-to-end delay and energy consumption

%边缘协同推理
%调度
%现有工作考虑到边缘服务器的资源约束，引入云中心进行计算，将模型分割成两部分，一部分部署在边缘服务器，另一部分部署云中心，形成一种边缘移动设备-边缘服务器-云服务器的三层任务卸载框架，
Nowadays, many smart home devices are applied to collaborative inference, such as Network Attached Storage (NAS), computing router, etc.
By combining the computing resources and storage capacity of multiple devices, users can realize the intelligent and personalized upgrade of some IoT device (such as camera, SmartWatch) while protecting data privacy\cite{shlezinger2022collaborative,hadidi2020toward}.
%
Based on model partitioning and early exit mechanism, we propose an edge collaborative inference framework, in which a pipeline system composed of multiple edge servers provides inference services for edge mobile devices. 
As shown in Figure \ref{fig:edgecol}, the large-scale model is divided into multiple sub-models, and each edge server deploys one of the sub-models.
After each task is offloaded to the edge server, it will be inferred on the sub-models of multiple edge servers until all inferences are completed or exited early from the branch.
Although the edge collaborative inference framework provides the aforementioned advantages, it still suffers from three other critical challenges in practical applications.
$\mathbf{1) System Heterogeneity.}$ In MEC system, edge servers  commonly possess limited and heterogeneous resources. For example, computing and bandwidth resources may differ by more than ten times between edge servers. Resource-short edge servers can lead to severe network congestion and compute load, which significantly affects the response latency of the system.
$\mathbf{2) Dynamic Environment.}$ The location of the edge mobile device and the frequency with which it offloads tasks may be constantly changing. For example, in the intelligent transportation system (ITS), the distribution of vehicles is spatially uneven and temporally dynamic\cite{car}, which will lead to the unbalanced load of edge servers in time and space, affecting the efficiency of task inference.
$\mathbf{3) Unavailable Global Information.}$ Due to the dynamic environment, it is difficult to collect global real-time information of the entire network, outdated global information can lead to bad decisions. 

%work
To address the above challenges, we consider two unique properties of edge cooperative inference architectures, model partitioning and early exit mechanism, and find two basic observations:
1) Based on model partitioning, each sub-model is deployed to multiple edge servers with different capabilities. Inspired by the previous work\cite{car}, we can optimize the task offloading strategy for each ED and each edge server, and assigning appropriate task loads to different edge servers helps to accommodate their different capabilities. For example, the task is mainly offloaded to the edge server with rich computing resources and bandwidth resources, so as to prevent the resource-poor edge server from becoming the bottleneck of response speed.
2) In a dynamic environment, the choice of the confidence threshold of the early exit mechanism is the key to balance the response delay and inference accuracy. The early exit mechanism can make some simple tasks exit early, and reduce the resource competition among the remaining tasks, so as to reduce the average response delay. Whether the task exits early depend on whether the prediction probability of tasks in exit branch is greater than the confidence threshold. In general, a larger confidence threshold will bring higher overall accuracy, but it will also reduce the number of tasks exit early, resulting in an increase in the average response delay. When the system load is too large, we need to appropriately reduce the confidence threshold, reduce the system load at the cost of a small loss of accuracy, and reduce the task response delay. On the contrary, when the system load is light, we also need to appropriately increase the confidence threshold to improve the accuracy.


Motivated by the above insights, we propose a distributed algorithm DTO to build an efficient edge cooperative inference framework by jointly optimizing task offloading strategy and confidence threshold. The difficulty of algorithm design is how to quantify and balance the interaction between task offloading strategy and confidence threshold.
On the one hand, achieve the balance between precision and delay, it is desired to select an appropriate confidence threshold and balance the system load. However, Due to the change of system load, we also need to readjust the task offloading strategy to minimize the average response delay.
On the other hand, in order to make full use of the resources of heterogeneous nodes, the task offloading strategy will assign different computing and bandwidth loads to different nodes, and we needs to dynamically select an appropriate confidence threshold to strike a balance between delay and accuracy.
Only by jointly optimizing task offloading strategy and confidence threshold can DTO help better solve the challenges of system heterogeneity and environment dynamics, and realize an efficient edge cooperative inference framework. 

%Since each sub-model may be deployed on multiple edge servers, we need to set an appropriate task offloading strategy for each ED and edge server.
%After the tasks arrive at the EDs or inference is complete on the edge servers, we need to choose which edge server to offload the tasks to.
%The task offloading strategy is multi-dimensional, and more challenging to optimize the task offloading strategy in edge network.
%Firstly, there is system heterogeneity in edge networks, the performance of edge servers is different due to the differences in hardware, software and other aspects.
%Secondly,the dynamic environment in the edge network also needs to be considered, the location of the EDs and the arrival rate of the tasks may change continuously.
%In addition, due to the dynamic environment, it is difficult to collect global real-time information of the entire network, we can only optimize the task offloading strategy by local local information in a distributed way.
%Therefore, we propose a distributed algorithm to address these challenges.
%Specifically, in order to minimize the average response delay of tasks in the edge collaborative framework while meeting various resource constraints, our distributed algorithm dynamically updates the task offloading strategy of each ED and edge server by collecting local information.
%In this paper, we optimize the task offloading strategy of each edge mobile device and edge server in the edge collaborative inference framework to minimize the average response delay of all tasks.
%We model the response delay of the task and design a distributed algorithm. Under the premise of meeting each resource constraint, the distributed algorithm dynamically optimizes the task offloading strategy of each node by collecting local information.


%总结123
%In this paper, we propose an edge cooperative inference mode, in which the whole system consists of multiple edge mobile devices and multiple edge servers, each edge server loads a part of the whole model and collaboratively completes the entire inference task. In the joint early exit mechanism, we schedule the task flow for any edge cooperative inference system. After the inference of the current edge server is completed, we need to decide which server the task flow should be sent to the next part, so that the average response delay of the task is the shortest. It is also necessary to consider the heterogeneity of the edge system and the resource constraints of each edge server.

The main contributions of this paper are as follows:
\begin{itemize}
	\item [1)]
	We propose an edge collaborative inference framework, which is deployed only at the edge. Based on model partitioning and early exit mechanism, the framework can improve resource utilization of the edge. 
	In addition, we model the response delay of the tasks based on queuing theory, and propose the formal definition of the optimization problem, which includes the power consumption limits of EDs and the computing resource limits of edge servers
	\item [2)]
	In order to minimize the average response delay of tasks in the edge collaborative inference framework, we propose a distributed task offloading algorithm. 
	Under the resource constraints, the distributed algorithm can dynamically optimize the task offloading strategy by collecting local information.
	%This algorithm allows each node to optimize its offloading strategy without knowing the offloading strategy of other nodes.
	\item [3)]
	We investigate the effects of multiple system settings on the performance of the distributed algorithms. Simulation results show that our distributed algorithm outperforms other baselines in a wide range of parameter settings.
\end{itemize}
The rest of this paper is organized as follows. 
Section \ref{sec:prelim} gives the system model and problem definition. We introduce our distributed algorithm in Section \ref{sec:alg}, evaluate its performance through simulation experiments in Section \ref{sec:results}, Section \ref{sec:related} introduces the relevant work, and summarize this paper in section \ref{sec:conclusion}.



\end{comment}

==> content/prelim_copy.tex <==
\subsection{Task Offloading}

Machine learning (ML) has been successfully applied to image recognition, natural language processing, recommendation systems and many other applications. The traditional way is to use the deep learning model of the cloud center platform to handle various requests from users, but with the continuous development of the Internet of Things (IoT), the amount of data explodes, and a large amount of data is transmitted to the cloud platform through the Internet, which poses a great challenge to the transmission bandwidth and delay of real-time applications. Edge computing is a new solution that offloads tasks from the end device to the edge server installed nearby for better responsiveness, lower latency, and higher bandwidth utilization.

With the continuous development of deep learning, various large models have achieved optimal results in many fields such as natural language processing (NLP), computer vision (CV) and generation. Large models typically have hundreds of millions to hundreds of billions of parameters, and inferences using large models require a lot of computing resources and storage space, which makes large models potentially difficult to deploy directly at the edge, while cloud-centric approaches lead to huge end-to-end latency and energy consumption on mobile devices. In order to strike a balance between latency and load, previous studies have proposed to divide the model into two parts, respectively offloading to the edge device and the edge server, but for large models, due to the memory capacity of the edge device, this method is almost impossible to achieve. Therefore, we propose the federated inference of edge servers, aiming to address the shortcomings of the first two.



	
\subsection{Cooperative Inference}



\begin{figure}
	\centering
	\includegraphics[width=0.95\linewidth]{./fig2/edge_inference.png}
	\caption{\label{fig:pipeline}multi-pipeline system.}
\end{figure}

In order to deploy the large model on the edge network, we need to divide the model into several sub-models. Here, we assume that the complete model $H$ is divided into $K$ sub-models, $H=\{h_{1},h_{2},...,h_{K}\}$ with $|H|=K$. 
For any sub-model $h_{k} \in H\backslash{h_{K}}$, its output is the input of the next sub-model $h_{k+1}$.
The complete model can be regarded as a function $H(\cdot)$, which maps the input $x$ to the final prediction $H(x)$. 
The complete forward inference process can be divided into $K$ parts, any part $h_{k}(\cdot)$ corresponds to the mapping of sub-model $h_{k}$:
\begin{equation}
	\hat{y} = H(x) = (h_{K} \circ h_{K-1} \circ \cdots \circ h_{1})(x)
\end{equation}
where $\hat{y}$ is the final prediction. The operator $\circ$ represents a combination of two functions, $\ie$$(h_{k} \circ h_{k-1})(\cdot) = h_{k}(h_{k-1}(\cdot))$.
%In the case of limited memory capacity and computing resources of edge servers, in order to deploy the large deep learning model at the edge, we need to divide the model into several sub-models, here we assume that there are $K$ sub-models $Model=\{m_{1},m_{2},...,m_{K}\}$ with $|Model|=K$. The output of the previous sub-model $m_{k} \in M\backslash{m_{K}}$ is the input of the latter sub-model $m_{k+1} \in M$. The complete model can be regarded as a function $M(\cdot)$, which maps the input $x$ to the final prediction $M(x)$. The complete forward inference process can be divided into $K$ parts, any part $m_{k}(\cdot)$ corresponds to the mapping of sub-model $m_{k}$:
%\begin{equation}
%	\hat{y} = M(x) = (m_{K} \circ m_{K-1} \circ \cdots \circ m_{1})(x)
%\end{equation}
%where $\hat{y}$ is the final prediction. The operator $\circ$ represents a combination of two functions, $\ie$$(m_{k} \circ m_{k-1})(\cdot) = m_{k}(m_{k-1}(\cdot))$.
%Each edge server only load one of the sub-models, we use $S^{k}$ to represent the set of edge servers that load the sub-model $m_{k}$, so that multiple edge servers can cooperatively complete the inference task of the large model. As shown in the figure 1, multiple edge servers form a multi-pipeline system. Each task propagates in the direction of the arrow (forward inference direction of model), and when a task arrives, each server performs the inference task on the sub-model it loads, gets the intermediate inference result, and then sends it to the server with the next sub-model, until gets the final inference result.

We consider an edge network composed of multiple nodes, the whole system includes the set of edge mobile devices $D = \{d_1,d_{2},...d_{M}\}$ with $|D|=M$, and the set of edge servers $S=\{s_{M+1},s_{M+2},...,s_{M+N}\}$ with $|S|=N$, here we assume that node $e_{i}$ refers to the edge mobile device $d_{i}$ or the edge server $s_{i}$.
Each edge mobile device will continuously generate new tasks and offload them to nearby edge servers. To get closer to reality, we consider that the task arrival process conforms to a Poisson process, and the tasks arrive in batches.
We use $\phi_{i}$ to represent the task arrival rate of edge mobile device $d_{i}$ and $\theta_{0}$ to represent the number of tasks per batch.
The task arrival rate of the whole system is $\Phi = \sum_{d_{i} \in D} \phi_{i}$.
For each edge server $s_{i}$, it will only load one sub-model, we use $S^{k}$ to represent the set of edge servers that load the sub-model $h_{k}$, thus $S=\cup S^{k},h_{k}\in H$.
We consider the edge network with system heterogeneity, the edge servers in the system are heterogeneous, they have different computing resources and bandwidth resources.
We use $\mu_{i}$ to represent the maximum compute resources of the edge server $s_{i}$, measured by the number of CPU cycles per unit time. 
And we use $r_{ij}$ to represent the transfer rate of node $e_{i}$ to edge server $s_{j}$, measured by the number of bits transferred per unit time.
The entire inference process of the task requires calculations on multiple sub-models and multiple transmission of intermediate data.
For different sub-models, the computational resources required for inference on them and the size of their input data are different
We use $\alpha_{i}$ and $\beta_{i}$ to represent the computational resources required for inference and the size of input data for a single task for a single task in $s_{i}$, respectively.
Tasks are offloaded to the next sub-model after they reach the edge mobile device or after the inference is completed on the edge server, we use $L_{i}$ to represent the set of offloaded target edge servers for node $e_{i}$.
For any edge mobile device $d_{i}$, $L_{i}$ is a set of edge servers which in $S^{1}$ and can communicate with $d_{i}$; for edge server $s_{i} \in S^{k},k \neq K$, $L_{i}$ is the set of edge servers which in $S^{k+1}$ and can communicate with $s_{i}$.
In addition, we use $V_{i}$ to denote the set of edge mobile devices or edge servers that can offload tasks to $s_{i}$.
We use the vector $p_{i} = \{p_{i,j}\}_{s_{j}\in S}$ to represent the offloading strategy of edge node $e_{i}$, where $p_{ij}$ is the probability that node $e_{i}$ offload its tasks to $s_{j}$, so $p_{i,j} \in [0,1]$, $\sum_{s_{j}\in L_{i}}p_{i,j} = 1$, and for $s_{j} \notin L_{i}, p_{i,j}=0$.
For ease of expression, we list some important notations in Table 1. 

%We consider an edge network system with a set of edge mobile devices $D = \{d_1,d_{2},...d_{M}\}$ with $|D|=M$. Each edge mobile device generates a batch of application tasks from time to time, The batchsize of each batch task is $\theta_{0}$. Assuming that the process of task arrival to $d_{m} \in D$ follows the Poisson process and the average arrival rate is $\phi_{m}$, the total task arrival rate of the system is $\Phi = \sum_{d_{m} \in D} \phi_{m}$. There are N edge servers deployed in the system, which have wireless access and computing capabilities. we use  $S=\{s_{M+1},s_{M+2},...,s_{M+N}\}$ with $|S|=N$  to represent the set of edge servers in the network, $S=\cup S^{k},m_{k}\in M$. The edge servers in $S$ are heterogeneous, they have different computing resources and bandwidth resources. we use $\mu_{i}$  to represent the maximum computing resources of edge server $s_{i} \in S$, measured by the number of CPU cycles per unit time. Each edge server loads a sub-model, and tasks through different sub-models require different computing resources, and will generate intermediate inference results of different sizes. We use $\alpha_{i}$ and $\beta_{i}$ to represent the computational resources required by a single task for inference and the size of input data for a single task in $s_{i}$.
%%
%We represent $V_{i}$ as the set of edge mobile devices or edge servers whose tasks can be offloaded to $s_{i}$. For edge server $s_{i} \in S^{1}$, $V_{i}$ is the set of edge mobile devices which can communicate with $s_{i}$; for edge server $s_{i} \in S^{k}, k\neq 1$,  $V_{i}$ is the set of edge servers which can communicate with $s_{i}$, and the edge server in $V_{i}$ loads the previous sub-model $m_{k-1}$. 
%%改
%And we represent $L$ as the set of offloading target edge servers to which the edge mobile device or edge server can offload. For edge mobile device $d_{m} \in D$, $L_{m}$ is the set of edge servers which can communicate with $d_{m}$; for edge server $s_{i} \in S^{k}, k \neq K$,  $V_{i}$ is the set of edge servers which can communicate with $s_{i}$, and the edge server in $V_{i}$ loads the latter sub-model $m_{k+1}$.
%After the task is generated by the edge mobile device, the edge mobile device will offload the task to a edge server $s_{n}$, $s_{n} \in S^{1}$, which loads the first sub-model. 
%In order to reduce bandwidth resource contention, we consider that each edge device will only offload tasks to one edge server in $S^{1}$.
%We use $a_{m}\in\{0,1\}$ to represent the offloading decision of the edge mobile device, $a_{m} = \{a_{m,j}\}_{s_{j}\in L_{m}}$ and $\sum_{s_{n}\in L_{m}}a_{m,j} = 1$. $a_{m,j}=1$ means that the $d_{m}$ will offload the task to $s_{j}$; $a_{m,j}=0$ indicates that $d_{m}$ does not perform the offloading process on $s_{j}$.
%The edge server $s_{i}$ receives the task for calculation and then obtains the intermediate inference result, which will be sent to a edge server that loads the next sub-model. We use $p_{i}\in [0,1]$ to represent the scheduling policy of edge server $s_{i}$, $p_{i} = \{p_{i,j}\}_{s_{j}\in L_{i}}$ and $\sum_{s_{j}\in L_{i}}p_{i,j} = 1$. $p_{i,j}$ represent the probability that edge server $s_{i}$ will send the intermediate inference result to $s_{j}$. 
%For ease of expression, we list some important notations in Table 1. 



\begin{table}[h]
	\setlength{\abovecaptionskip}{10pt}%
	\setlength{\belowcaptionskip}{0pt}%
	\centering
	\caption{Key Notations.}
	\label{tbl:natation}
	\resizebox{\linewidth}{!}{
		\begin{tabular}{cl}
			\hline
			\textbf{Symbol} & \textbf{Semantics}\\
			\hline
			$H$ & the set of sub-models $\{h_{1}, h_{2},..., h_{K}\}$ \\
			$D$ & the set of edge mobile devices $\{d_{1},d_{2},...,d_{M}\}$ \\
			$S$ & the set of edge servers $\{s_{M+1},s_{M+2},...,s_{M+N}\}$  \\ 
			$S^{k}$ & the set of edge servers that load sub-model $h_{k}$ \\
			%$V_{m}$ & the set of edge mobile devices whose tasks can be offloaded to $s_{i}$ \\
			$V_{i}$ & the set of nodes whose tasks can be offloaded to $s_{i}$ \\
			%$L_{m}$ & the set of target edge servers to which $d_{m}$ can task offload \\
			%$L_{i}$ & the set of target edge servers to which $d_{i}$ or $s_{i}$ can offload its tasks to\\
			$L_{i}$ & the set of target edge servers to which $e_{i}$ can offload its tasks to\\
			$\phi_{i}$ & Task arrival rate of edge mobile device $d_{i}$ \\
			$\Phi_{i}$ & Task arrival rate of edge server $s_{i}$ \\
			$\Phi$ & Total task arrival rate of system \\
			$\mu_{i}$ & the maximum computing resources of edge server $s_{i}$\\
			$\alpha_{i}$ & The computing resources required by a single task for inference in $s_{i}$ \\
			$\beta_{i}$ & the size of input data for a single task in $s_{i}$ \\
			%$a_{m}$ & the offloading decision of $d_{m}$ \\
			$p_{i}$ & the task offloading strategy of edge node $e_{i}$ \\
			$r_{i,j}^{d2s}$ & the uplink transmission rate from $d_{i}$ to $s_{j}$ \\
			$r_{i,j}^{s2s}$ & the transmission rate from $s_{i}$ to $s_{j}$ \\
			$\lambda_{i}$ & the total computing resource required on edge server $s_{i}$ \\
			$\theta_{i}$ & the batchsize of a batch input task of edge server $s_{i}$ \\
			$\theta_{0}$ & the batchsize of a batch output task of edge mobile device \\
			\hline
		\end{tabular}
	}
\end{table}



\subsection{Delay Model}

In the edge collaborative inference framework, MDs immediately offload tasks to nearby edge servers after the task arrives. 
Each task will be inferred on multiple edge servers in the order of sub-models until the final inference result is obtained.
The delay of the entire inference process is the response delay of the task, which consists of three parts: transmission delay, queuing delay and calculation delay.
%Tasks are generated from edge devices and then offloaded to edge servers. Each edge server calculates tasks on its sub-model, obtains intermediate inference result, and sends it to the next edge server, until the last edge server gets the final result. The delay of this whole process is composed of three parts: transmission delay, computation delay and queuing delay.

Similar to many studies such as []-[], since the results of DNN inference are usually small, the time overhead and energy consumption of MDs downloading the inference results are negligible. 
In addition, since we focus on edge computing systems, where MDs and edge servers are spatially close, we ignore the propagation delay.
In edge networks, MDs mainly offload tasks to edge servers through wireless channels due to their mobility. We consider channel access solutions (such as CMDA) in which multiple MDs can share the same spectrum resources.
%Edge devices communicate with edge servers through wireless links, so there is a preemption of bandwidth resources between edge devices. 
We use $\eta_{i}$ to represent the upstream transmission power of edge device $d_{i}$, and $h_{i,j}$ to represent the uplink channel gain from $d_{i}$ to the edge server $s_{j}$. 
If edge device is too far away from the edge server or the signal is too weak, then the edge device cannot connect to the edge server. 
The uplink transmission rate from $d_{i}$ to $s_{j}$ can be calculated by Shannon's theorem:
\begin{equation}
	r_{i,j}^{d2s} = B log_{2}(1+\frac{\eta_{i}h_{i,j}}{\sigma^2+\sum_{d_{i'}\in V_{j}\backslash \{ d_{i}\} }\eta_{i'}h_{i',j}})	
\end{equation}
where $B$ is the channel bandwidth, and $\sigma^2$ is the noise.
Different from MDs, edge servers mainly transmit intermediate data, and there exists a stable data transfer rate between edge servers.
%Data transmission between edge servers generally does not depend on wireless transmission, and there is a fixed bandwidth between them.
We use $r_{i,j}^{s2s}$ to represent the transmission rate from edge server $s_{i}$ to $s_{j}$, and we use $\theta_{i}$ to denote the batchsize of a batch input task of edge server $s_{i}$. 
The transmission delay from the edge mobile device $d_{i}$ or the edge server $s_{i}$ to the edge server $s_{j}$ is:
\begin{equation}
	T^{cm}_{i,j}=\left\{
	\begin{array}{lc}
		\theta_{j} \beta_{j} / r^{d2s}_{i,j} & d_{i}\in D, s_{j} \in S^{1}\\
		\theta_{j} \beta_{j} / r^{s2s}_{i,j} & s_{i},s_{j}\in S\\
	\end{array}
	\right.
\end{equation}
In addition, we can get the average energy consumption of $d_{i}$ offloading tasks to edge servers as:
\begin{equation}
	E^{cm}_{i}=\sum_{s_{j}\in L_{i}}p_{i,j}\eta_{i}T^{cm}_{i,j}
\end{equation}

In the edge collaborative inference framework, we assume that the MDs do not have enough computational resources and energy to support deep learning task computation, and DNN inference is all completed on the edge servers. The computing delay of inferencing a batch task on the edge server $s_{i}$ is:
%The computing time of each batch depends on the number of tasks in the batch, the computing resources required to compute a single task, and the computing resources of the edge server. therefore, the computing time for $s_{i}$ to compute a batch task is:
\begin{equation}
	T^{cp}_{i} = \frac{\theta_{i} \alpha_{i}}{\mu_{i}}	
\end{equation}

We consider establishing a task queue on each edge server, if the edge server does not complete the current inference task, subsequent tasks can only be placed on the task queue to wait. 
The process of task arrival follows Poisson process, and the inference rate of edge servers is considered as fixed, therefore, the task queue of the edge servers in $S^{1}$ can be modeled as the M/D/1 models.
According to the characteristics of the tandem queue system, the output process of edge servers in $S^{1}$ can be approximated as Poisson process, so the task queue of other edge servers can also be modeled as M/D/1 models.
The queuing delay of edge server $s_{i}$ is:
%The generation of tasks follows a Poisson process, and the computing rate of servers is considered as fixed. 
%Therefore, the server task queue in $S^{1}$ can be modeled as M/D/1 models. 
%According to the characteristics of the tandem queue system, the task arrival process of other edge servers can also be approximated as a Poisson process, so their task queues are also modeled as M/D/1 models. 
%the delay of queuing of edge server $s_{i}$ is:
\begin{equation}
	T^{q}_{i} = \frac{\lambda_{i}}{2\mu_{i}(\mu_{i}-\lambda_{i})}	
\end{equation}
where $\lambda_{i}$ is the total computing resource required on edge server $s_{i}$, $\lambda_{i} = \Phi_{i} \theta_{i} \alpha_{i}$. where $\Phi_{i}$ is the arrival rate of all tasks in edge server $s_{i}$. 

%%%
For each edge server $s_{j} $, its arrival rate of all tasks $\Phi_{j}$ is related to the offloading strategy of edge servers or edge mobile devices in $V_{j}$. 
%For the edge server $s_{j} \in S^{1}$, its task arrival rate depends on the offloading decision of the edge mobile device of $V_{j}$; for the edge server $s_{j} \in S^{k}, k\neq 1$, its task arrival rate depends on the offloading probability of all servers of $V_{j}$.
\begin{equation}
	\Phi_{j}=\left\{
	\begin{array}{lc}
		\sum\limits_{d_{i} \in V_{j}} p_{i,j} \phi_{i}  &\forall s_{j}\in S^{1}\\
		\sum\limits_{s_{i}\in V_{j}} p_{i,j} \Phi_{i} &\forall  s_{j}\notin S^{1}\\
	\end{array}
	\right.
\end{equation}







\subsection{Early Exit}

The early exit mechanism modifies the standard deep network structure by adding exit branches at certain locations throughout the network. The early exit of data in the middle layer of DNN costs a certain loss of accuracy, which can accelerate DNN inference on the one hand and reduce the size of data stream on the other hand. 

when a batch task is inferred by a model with multiple early exit points. Every time the batch task passes an early exit point, some tasks will exit early and will no longer be input to the next sub-model. We indicate that the proportion of exit tasks at the early exit point of sub-model $m_{k}$ is $E_{k}$, and when a sub-model does not have early exit point, the $E_{k}$ of the sub-model is regarded as 0. In general, the exit ratio of each early exit point is negatively correlated with the exit threshold of that early exit point. 
%伪代码
For any edge server $s_{i} \in S^{k}$ , compared to the number of tasks per batch, the proportion of the number of output tasks is $I_{i}$. On average,
\begin{equation}
	I_{i}=1-E_{k}, s_{i}\in S^{k}
\end{equation}
\begin{equation}
	\theta_{i}=\prod_{\kappa=0}^{k-1}(1-E_{\kappa}) \theta_{0}, s_{i}\in S^{k}
\end{equation}



\subsection{Problem Definition}

In the whole process from the generation of edge mobile devices to the final inference result, the task passes through $K$ edge servers at most, corresponding to $K$ sub-models respectively. This process can be regarded as $K$ times of task offloading process. We use $T^{k}$ to represent the average time to offload to the submodel $m_{k+1}$ after the computation of the submodel $m_{k}$ of the task is completed, and in particular, $T^{0}$ denote the average time of offloading the task from the edge mobile devices to the edge servers in $S^{1}$. 
%For the convenience of description, We use $S^{0}$ to represent the set of edge mobile devices $D$. 
We use $T_{i}^{k}$ and $T_{m}^{0}$ to represent the time of task offloading of the edge server $s_{i}$ in $S^{k}$ and edge mobile device $d_{m}$, respectively, and $T^{k}$ and $T^{0}$ can be represented as follows: 

\begin{equation}
	T^{k} = \sum_{s_{i}\in S^{K}}\frac{\Phi_{i}}{\Phi} T^{k}_{i}, k\neq0 
\end{equation}
\begin{equation}
	T^{0} = \sum_{d_{m}\in D}\frac{\phi_{m}}{\Phi} T^{0}_{m}
\end{equation}
\begin{equation}
	T^{k}_{i} = \sum_{s_{j}\in L_{i}} p_{i,j} (T^{cm}_{i,j} + T^{q}_{j} + T^{cp}_{j}), k\neq0
\end{equation}
\begin{equation}
	T^{0}_{m} = \sum_{s_{j}\in L_{m}} a_{m,j} (T^{cm}_{m,j} + T^{q}_{j} + T^{cp}_{j})
\end{equation}

We aim to minimize the average response time by finding the best offloading strategy of the edge server, which needs to take into account the heterogeneous situation of computing power and bandwidth resources of different edge servers, as well as the impact of the model early exit mechanism on the size of the data stream. The question can be formalized as follows:


\begin{equation}
	(P1):\min\limits_{A,P} \sum_{k=0}^{K-1} T^{k}
\end{equation}

$$ s.t.\left\{
\begin{aligned}
	&T_{i}^{k} =  \sum_{s_{j}\in L_{i}} p_{i,j} (T^{cm}_{i,j} + T^{q}_{j} + T^{cp}_{j}),   &\forall s_{i} \in S_{k}\\
	&\lambda_{i} < \mu_{i},  &\forall  s_{i} \in S\\
	&a_{m,j} \in \{0,1\}, &\forall d_{m} \in D, s_{j} \in L_{m}\\
	&\sum_{s_{j} \in L_{m}} a_{m,j} = 1 & \forall d_{m} \in D\\
	&0 \leq p_{i,j} \leq 1, &\forall  s_{i}, s_{j} \in S\\
	&\sum_{s_{j} \in L_{i}} p_{i,j} = 1, &\forall  s_{i} \in S
\end{aligned}
\right.
$$

The first equation models the time it takes to offload a task to an edge server,  which includes transmission delay, queuing delay, and computation delay. The second inequality indicates the constraint of computing resources on each edge server, the total computing resources required by the task should be less than the maximum computing resources of the edge server. The third and fourth formulas represent the offloading decision of the edge mobile device and the constraints on the decision. The fifth and sixth formulas represent the scheduling decision of each edge server and the constraints on that decision.



\begin{comment}
	内容...

\subsection{Federated Inference}

In the case of limited edge server capacity, in order to deploy the deep learning model at the edge, we need to divide the model into several sub-models, here we assume that there are $K$ sub-models $Model=\{m_{1},m_{2},...,m_{K}\}$ with $|Model|=K$. The output of the previous sub-model $m_{k} \in M\backslash{m_{K}}$ is the input of the later sub-model $m_{k+1} \in M$, and each edge server only load one of the sub-models, we use $S^{k}$ to represent the set of edge servers that load the sub-model $m_{k}$, so that multiple edge servers can jointly complete the inference task of the large model. As shown in the figure 1, multiple edge servers form a multi-pipeline system. Each task propagates in the direction of the arrow (forward inference direction of model), and when a task arrives, each server performs the inference task on the sub-model it loads, gets the intermediate inference result, and then sends it to the server with the next sub-model, until gets the final inference result.

We consider an edge network system with a set of edge mobile devices $D = \{e_1,e_{2},...e_{M}\}$ with $|D|=M$. Each edge mobile device generates a batch of application tasks from time to time, The batchsize of each batch task is $\theta_{0}$. Assuming that the process of task arrival to $e_{i} \in D$ follows the Poisson process and the average arrival rate is $\phi_{i}$, the total task arrival rate of the system is $\Phi = \sum_{e_{i} \in D} \phi_{i}$. There are N edge servers deployed in the system, which have wireless access and computing capabilities. we use  $S=\{e_{M+1},e_{M+2},...,e_{M+N}\}$ with $|S|=N$  to represent the set of edge servers in the network, $S=\cup S^{k},m_{k}\in M$. The edge servers in $S$ are heterogeneous, they have different computing resources and bandwidth resources. we use $\mu_{i}$  to represent the maximum computing resources of edge server $e_{i} \in S$, measured by the number of CPU cycles per unit time. Each edge server loads a sub-model, and tasks through different sub-models require different computing resources, and will generate intermediate inference results of different sizes. We use $\alpha_{i}$ and $\beta_{i}$ to represent the computational resources required by a single task for inference and the size of input data for a single task in $e_{i}$.
%
We represent $V_{i}$ as the set of edge mobile devices or edge servers whose tasks can be offloaded to $e_{i}$. For edge server $e_{i} \in S^{1}$, $V_{i}$ is the set of edge mobile devices which can communicate with $e_{i}$; for edge server $e_{i} \in S^{k}, k\neq 1$,  $V_{i}$ is the set of edge servers which can communicate with $e_{i}$, and the edge server in $V_{i}$ loads the previous sub-model $m_{k-1}$. 
%
And we represent $L_{i}$ as the set of offloading target edge servers to which the edge mobile device or edge server $e_{i}$ can offload. For edge mobile device $e_{i} \in D$, $L_{i}$ is the set of edge mobile devices which can communicate with $e_{i}$; for edge server $e_{i} \in S^{k}, k \neq K$,  $V_{i}$ is the set of edge servers which can communicate with $e_{i}$, and the edge server in $V_{i}$ loads the latter sub-model $m_{k+1}$.
%
After the task is generated by the edge mobile device, the edge mobile device will offload the task to a edge server $e_{i} \in S^{1}$, which loads the first sub-model. 
In order to reduce bandwidth resource contention, we consider that each edge device will only offload tasks to one edge server in $S^{1}$.
We use $a_{i}\in\{0,1\}$ to represent the offloading decision of the edge mobile device $e_{i}$, $a_{i} = \{a_{i,j}\}_{e_{j}\in L_{i}}$ and $\sum_{e_{j}\in L_{i}}a_{i,j} = 1$. $a_{i,j}=1$ means that the the edge mobile device $e_{i}$ will offload the task to the edge server $e_{j}$; $a_{m,j}=0$ indicates that the edge mobile device $e_{i}$ does not perform the offloading process the edge server $e_{j}$.
%
The edge server $e_{i} \in S$ receives the task for calculation and then obtains the intermediate inference result, which will be sent to a edge server that loads the latter sub-model. We use $p_{i}\in [0,1]$ to represent the scheduling policy of edge server $e_{i}$, $p_{i} = \{p_{i,j}\}_{e_{j}\in L_{i}}$ and $\sum_{e_{j}\in L_{i}}p_{i,j} = 1$. $p_{i,j}$ represent the probability that the edge server $e_{i}$ will send the intermediate inference result to the edge server $e_{j}$. 
 %For each edge server $s_{i} \in S^{k}, k \neq K$, it will only send intermediate inference results to the edge servers of $S^{k+1}$. For the convenience of description, we regard edge mobile devices as a special edge server. Compared with other edge servers, they do not participate in the inference calculation of tasks and can only offload tasks on a single edge server through a wireless link. We use $S^{0}$ to represent the set of edge mobile devices. 
For ease of expression, we list some important notations in Table 1. 




\subsection{Delay Model}

Tasks are generated from edge devices and then offloaded to edge servers. Each edge server calculates tasks on its sub-model, obtains intermediate inference result, and sends it to the next edge server, until the last edge server gets the final result. The delay of this whole process is composed of three parts: transmission delay, computation delay and queuing delay.


Edge devices communicate with edge servers through wireless links, so there is a preemption of bandwidth resources between edge devices. Let $\eta_{i}$ represent the upstream transmission power of the edge mobile device $e_{i} \in D$, and $h_{i,j}$ represent the uplink channel gain from the edge mobile device $e_{i}$ to the edge server $e_{j}$, if edge device is too far away from the edge server or the signal is too weak, then the edge device cannot communicate with the edge server. Then the uplink transmission rate from the edge mobile device $e_{i}$ to the edge server $e_{j}$ can be calculated by Shannon's theorem:
\begin{equation}
	r_{i,j}^{d2s} = B log_{2}(1+\frac{\eta_{i}h_{i,j}}{\sigma^2+\sum_{e_{i'}\in V_{j}\backslash \{ e_{i}\} }\eta_{i'}h_{i',j}})	
\end{equation}

where $B$ is the channel bandwidth, and $\sigma^2$ is the noise.
Because we focus on edge computing systems, devices and edge servers are close together, therefore, the propagation delay is negligible, and we only need to consider the transmission delay. Data transmission between edge servers generally does not depend on wireless transmission, and there is a fixed bandwidth between them, we use $r_{i,j}^{s2s}$ to represent the transmission rate from the edge server $e_{i}$ to the edge server $e_{j}$,  we use $\theta_{i}$ to denote the batchsize of a batch input task of edge server $e_{i}$. therefore, the transmission time from node $e_{i}$ (edge device or edge server) to the edge server $e_{j}$ is:
\begin{equation}
	T^{cm}_{i,j}=\left\{
	\begin{array}{lc}
		\theta_{j} \beta_{j} / r^{d2s}_{i,j} & e_{i}\in D, e_{j} \in S^{1}\\
		\theta_{j} \beta_{j} / r^{s2s}_{i,j} & e_{i},e_{j}\in S\\
	\end{array}
	\right.
\end{equation}



The computing time of each batch depends on the number of tasks in the batch, the computing resources required to compute a single task, and the computing resources of the edge server. therefore, the computing time for the edge server $e_{i}$ to compute a batch task is:
\begin{equation}
	T^{cp}_{i} = \frac{\theta_{i} \alpha_{i}}{\mu_{i}}	
\end{equation}


The generation of tasks follows a Poisson process, and the computing rate of servers is considered as fixed. Therefore, the server task queue in $S^{1}$ can be modeled as M/D/1 models. According to the characteristics of the tandem queue system, the task arrival process of other edge servers can also be approximated as a Poisson process, so their task queues are also modeled as M/D/1 models. the delay of queuing of edge server $e_{i}$ is:
\begin{equation}
	T^{q}_{i} = \frac{\lambda_{i}}{2\mu_{i}(\mu_{i}-\lambda_{i})}	
\end{equation}
where $\lambda_{i}$ is the total computing resource required on edge server $s_{i}$, $\lambda_{i} = \Phi_{i} \theta_{i} \alpha_{i}$. where $\Phi_{i}$ is the arrival rate of all task in edge server $e_{i}$. 


%%%%
For edge server $e_{j} $, the $\Phi_{j}$ is related to the offloading decision of other edge servers or edge mobile devices. For the edge server $e_{j} \in S^{1}$, its task arrival rate depends on the offloading decision of the edge mobile device in $V_{j}$; for the edge server $e_{j} \in S^{k}, k\neq 1$, its task arrival rate depends on the offloading probability of all servers in $V_{j}$.
\begin{equation}
	\Phi_{j}=\left\{
	\begin{array}{lc}
		\sum\limits_{e_{i} \in V_{j}} a_{i,j} \phi_{i}  &\forall e_{j}\in S^{1}\\
		\sum\limits_{s_{i}\in V_{j}} p_{i,j} \Phi_{i} &\forall  e_{j}\notin S^{1}\\
	\end{array}
	\right.
\end{equation}






\begin{figure}
	\centering
	\includegraphics[width=0.9\linewidth]{./fig/pipeline.png}
	\caption{\label{fig:pipeline}multi-pipeline system.}
\end{figure}


\begin{table}[h]
	\setlength{\abovecaptionskip}{10pt}%
	\setlength{\belowcaptionskip}{0pt}%
	\centering
	\caption{Key Notations.}
	\label{tbl:natation}
	\resizebox{\linewidth}{!}{
	\begin{tabular}{cl}
		\hline
		\textbf{Symbol} & \textbf{Semantics}\\
		\hline
		$Model$ & the set of sub-models $\{m_{1}, m_{2},..., m_{K}\}$ \\
		$D$ & the set of edge mobile devices $\{d_{1},d_{2},...,d_{M}\}$ \\
		$S$ & the set of edge servers $\{s_{1},s_{2},...,s_{N}\}$  \\ 
		$S^{k}$ & the set of edge servers that load sub-model $m_{k}$ \\
		$D_{i}^{d}$ & the set of edge mobile devices whose tasks can be offloaded to $s_{i}$ \\
		$D_{i}^{s}$ & the set of edge servers whose tasks can be offloaded to $s_{i}$ \\
		$S_{m}^{d}$ & the set of target edge servers to which $d_{m}$ can task offload \\
		$S_{i}^{s}$ & the set of target edge servers to which $s_{i}$ can task offload \\
		$\phi_{m}$ & Task arrival rate of edge mobile device $d_{m}$ \\
		$\Phi_{i}$ & Task arrival rate of edge server $s_{i}$ \\
		$\Phi$ & Total task arrival rate of system \\
		$\mu_{i}$ & the maximum computing resources of edge server $s_{i}$\\
		$\alpha_{i}$ & The computing resources required by a single task for inference in $s_{i}$ \\
		$\beta_{i}$ & the size of input data for a single task in $s_{i}$ \\
		$a_{m}$ & the offloading decision of $d_{m}$ \\
		$p_{i}$ & the scheduling policy of edge server $s_{i}$ \\
		$r_{m,j}^{d2s}$ & the uplink transmission rate from $d_{m}$ to $s_{j}$ \\
		$r_{i,j}^{s2s}$ & the transmission rate from $s_{i}$ to $s_{j}$ \\
		$\lambda_{i}$ & the total computing resource required on edge server $s_{i}$ \\
		$\theta_{i}$ & the batchsize of a batch input task of edge server $s_{i}$ \\
		\hline
	\end{tabular}
	}
\end{table}




\subsection{Early Exit}

The early exit mechanism modifies the standard deep network structure by adding exit branches at certain locations throughout the network. The early exit of data in the middle layer of DNN costs a certain loss of accuracy, which can accelerate DNN inference on the one hand and reduce the size of data stream on the other hand. 

when a batch task is inferred by a model with multiple early exit points. Every time the batch task passes an early exit point, some tasks will exit early and will no longer be input to the next layer of the model. We indicate that the proportion of exit tasks at the early exit point of sub-model $m_{k}$ is $E_{k}$, and when a block does not exit early, it is regarded as 0. In general, the exit ratio of each early exit point is negatively correlated with the exit threshold of that early exit point. Compared with the number of tasks in the initial batch task, the proportion of the number of input tasks in sub-model $m_{k}$ is $I_{k}$. On average,
\begin{equation}
	I_{k}=\prod_{i=0}^{k-1}(1-E_{i})
\end{equation}
\begin{equation}
	\theta_{i}=I_{k} \theta_{0}, i\in S^{k}
\end{equation}



\subsection{Problem Definition}

In the whole process from the generation of edge mobile devices to the final inference result, the task passes through $K$ edge servers at most, corresponding to $K$ sub-models respectively. This process can be regarded as $K$ times of task offloading process. We use $T^{k}$ to represent the average time to offload to the submodel $m_{k+1}$ after the computation of the submodel $m_{k}$ of the task is completed, and in particular, $T^{0}$ denote the average time of offloading the task from the edge mobile devices to the edge servers in $S^{1}$. 
%For the convenience of description, We use $S^{0}$ to represent the set of edge mobile devices $D$. 
We use $T_{i}^{k}$ and $T_{j}^{0}$ to represent the time of task offloading of the edge server $e_{i}$ in $S^{k}$ and edge mobile device $e_{j}$ in $D$, respectively, and $T^{k}$ and $T^{0}$ can be represented as follows: 

\begin{equation}
	T^{k} = \sum_{e_{i}\in S^{K}}\frac{\Phi_{i}}{\Phi} T^{k}_{i}, k\neq0 
\end{equation}
\begin{equation}
	T^{0} = \sum_{e_{i}\in D}\frac{\phi_{i}}{\Phi} T^{0}_{i}
\end{equation}
\begin{equation}
	T^{k}_{i} = \sum_{e_{j}\in L_{i}} p_{i,j} (T^{cm}_{i,j} + T^{q}_{j} + T^{cp}_{j}), k\neq0
\end{equation}
\begin{equation}
	T^{0}_{i} = \sum_{e_{j}\in L_{i}} a_{i,j} (T^{cm}_{i,j} + T^{q}_{j} + T^{cp}_{j})
\end{equation}

We aim to minimize the average response time by finding the best offloading strategy of the edge server, which needs to take into account the heterogeneous situation of computing power and bandwidth resources of different edge servers, as well as the impact of the model early exit mechanism on the size of the data stream. The question can be formalized as follows:


\begin{equation}
	(P1):\min\limits_{A,P} \sum_{k=0}^{K-1} T^{k}
\end{equation}

$$ s.t.\left\{
\begin{aligned}
	&T_{i}^{k} =  \sum_{e_{j}\in L_{i}} p_{i,j} (T^{cm}_{i,j} + T^{q}_{j} + T^{cp}_{j}),   &\forall e_{i} \in S_{k}\\
	&\lambda_{i} < \mu_{i},  &\forall  e_{i} \in S\\
	&a_{i,j} \in \{0,1\}, &\forall e_{i} \in D, e_{j} \in L_{i}\\
	&\sum_{e_{j} \in L_{i}} a_{i,j} = 1 & \forall e_{i} \in D\\
	&0 \leq p_{i,j} \leq 1, &\forall  e_{i}, e_{j} \in S\\
	&\sum_{e_{j} \in L_{i}} p_{i,j} = 1, &\forall  e_{i} \in S
\end{aligned}
\right.
$$

The first equation models the time it takes to offload a task to an edge server,  which includes transmission delay, queuing delay, and computation delay. The second inequality indicates the constraint of computing resources on each edge server, the total computing resources required by the task should be less than the maximum computing resources of the edge server. The third and fourth formulas represent the offloading decision of the edge mobile device and the constraints on the decision. The fifth and sixth formulas represent the scheduling decision of each edge server and the constraints on that decision.

\section{Algorithm Design}

The above formula is a mixed integer nonlinear programming problem, and finding the optimal solution for such problems is computationally complex. Moreover, in distributed network scenarios, due to limitations such as communication range, some edge servers may not have communication links, so we can not solve the problem by collecting global information in real time like centralized machine learning. That means solutions are hard to come by.

Therefore, we design a distributed scheduling update algorithm in which each node (edge mobile device or edge server) updates its offload decision only based on local information (including local information and information of adjacent communicable nodes). We divide the system time into fixed length time slots, and each node in each time slot exchanges information with its neighboring nodes, and updates its task offloading decisions until the whole system reaches Nash equilibrium and all decisions converge to the approximate optimal solution.

\subsection{Problem Transformation}

From formula (5), we know that in the stationary state of the system, the task arrival rate $\Phi_{i}$ of edge server $e_{i}$ depends on the offloading decision of node in $V_{i}$. The $\Phi_{i}$ of any edge server $e_{i}$ is also optimal when all edge mobile devices and all edge servers use the optimal offload decisions.
The sum of the transfer delay, queuing delay and computing delay in the process of offloading task to the next edge server is regarded as the local offloading delay.
For each edge mobile device or edge server $e_{i}$, just minimizing the local offload delay does not minimize the response delay of the entire system, because an offload decision that minimizes the local offloading delay does not make $\Phi_{j}$ of next edge server $e_{j}$ in $e_{i}$ optimal.
Therefore, the optimal offloading decision needs to consider not only the transmission delay, queuing delay and calculation delay during the local offloading process, but also needs to consider how long it will take from the completion of the calculation of the edge server to the completion of all the reasoning of the task.
%%%例子
Therefore, we also need to introduce a variable $r$ and $rd$, which represents the remaining completion time and the gradient information of the edge server, respectively. The remaining completion $r_{i}$ time represents the time from the completion of inference calculation on the edge server $e_{i}$ to the final inference result of the task. The remaining completion time of each edge server can be calculated by the following formula:
\begin{equation}
	r_{i} = \sum_{s_{j} \in S_{i}^{s}}p_{i,j}(T^{cm}_{i,j} + T^{q}_{j} + T^{cp}_{j} + r_{j})
\end{equation}
for any edge server $e_{i}$,The remaining completion time $r_{i}$ includes the local offloading delay and the remaining completion time of the edge server $e_{j}$ in $L_{i}$. In particular, for any edge servers $e_{j}$ in $S^{K}$, $r_{j}=0$.

%%%rd解释


In order to facilitate the description and analysis of distributed algorithms, we first transform the constraints of the problem (P1) into its optimization objective by using the outer point method, so as to deal with the problem whose solution may exceed the feasible domain. Therefore, we construct the constraint as a penalty function.
\begin{equation}
	N(p) = L \cdot \sum_{e_{i}\in S}max\{0,\lambda_{i}-\mu_{i} + \epsilon\}
\end{equation}
where $L$ is a given large enough normal number, called the penalty factor. The penalty function is then added to the objective function to transform the original problem into the following optimization problem for each edge server $e_{i}$.
\begin{equation}
	(P2):\min\limits_{p_{i}} R_{i}
\end{equation}

$$ s.t.\left\{
\begin{aligned}
	&R_{i} =  \sum_{e_{j}\in L_{i}} p_{i,j} (T^{cm}_{i,j} + T^{q}_{j} + T^{cp}_{j} + r_{j} + N(p)) \\
	&0 \leq p_{i,j} \leq 1\\
	&\sum_{e_{j}\in L_{i}} p_{i,j} = 1
\end{aligned}
\right.
$$

If the policy $p$ does not satisfy $\lambda_{i} < \mu_{i}$ for any edge server $e_{i}$, then the value of the optimization objective $R_{i}$ will be very large, so setting a sufficiently large value for $L$ can obtain an approximate optimal solution of (P1).

The main challenge to obtain the optimal solution of problem (P2) is the incompleteness of node information in distributed scenarios. Because a single node cannot know the decision information of other nodes, it is difficult to consider the computing power and constraint of edge nodes when making its own delay optimal decision. In order to solve this problem, the DTO algorithm is designed in this section, so that each node only needs to consider the computing and communication resource information of its own neighboring nodes when making decisions.

\subsection{Process of system}

In each time slot, the edge mobile device runs the resource request algorithm. The edge server $e_{i}$ is a resource requester for $L_{i}$ and a task receiver for $V_{i}$, so it runs both the resource request algorithm and the task receiving algorithm.

We first introduce the initialization and termination conditions of the algorithm. At the beginning of the algorithm, the edge mobile device $e_{m}$ randomly selects an edge server in $L_{i}$ as the target for task offloading, and each edge server $e_{i}$ average its offloading probabilities, $p_{i,j} = 1 / |L_{i}|$. 

We define a positive threshold $\Psi$, which determines the accuracy required when the algorithm terminates. Each edge server $s_{i}$ detects the following two conditions:
\begin{equation}
	\left\{
	\begin{aligned}
		&\lambda_{j} < \mu_{j},  \forall s_{j} \in S_{i}^{s}\\
		&R_{i}^{t} \leq (1+\Psi)R_{i}^{t-1}\\
	\end{aligned}
	\right.
\end{equation}
Condition 1 means that as long as required computing resources on any edge server $s_{j} \in S_{i}^{s}$ exceeds its limit, the iterative algorithm will continue to execute. The condition 2 indicates that the algorithm convergence can be judged when the performance difference between two successive iterations is very small. If the above two conditions are met, the iteration will terminate, otherwise it will start the next round of iteration to obtain a new round of offloading strategy.

$p^{(t)}$ and $a^{(t)}$ represent the offload decision of the edge servers and edge mobile devices in the round t iteration. In round t iteration of the resource request algorithm, the edge mobile device $d_{m}$ or edge server $s_{i}$ sends the resource request message (RRM) to the offload target in $S_{m}^{d}$ and $S_{i}^{s}$ respectively. RRM includes the required resources $\xi^{(t)}$, for edge mobile devices $d_{m}$, RRM also includes $\eta_{m}$, $h_{m,j}$, and $\xi_{m,j}^{(t)}=a_{m,j}^{(t)}\phi_{m}\theta_{j}\alpha_{j}$, for edge servers $s_{i}$, $\xi_{i,j}^{(t)} = p_{i,j}^{(t)}\Phi_{i}\theta_{j}\alpha_{j}$.

In the round t iteration of the task receiving algorithm, the edge server receives the all the RRMs to obtain the total computing resources required, transmission rate, and estimate its remaining completion time. 
Then each edge server $s_{j}$ broadcasts its resource status message (RSM) to the nodes in $D_{j}^{s}$ or $D_{j}^{d}$. The RSM includs the total compute resources required $\lambda_{i}$, transmission rate $r^{d2s}_{m,j}$ or $r^{s2s}_{i,j}$, remaining completion time $r_{j}$, and gradient information $rd_{j}$. Note that the compute resources and remaining completion time here are not the actual data of the edge server, it is a numerical estimate based on the request message sent by the device at round t. After all RUSs is received by the edge mobile device or edge server, new offloading decisions are made based on this information.
In this way, edge mobile devices and edge servers adjust their offload decisions through multiple iterations. When all nodes have reached a convergent unload decision, the algorithm terminates, nodes will send END message to the edge servers.

\begin{algorithm} 
	\caption{Task Receiving Algorithm for $s_{j}$} 
	\label{TRA} 
	\begin{algorithmic}
		%\REQUIRE $n \geq 0 \vee x \neq 0$ 
		%\ENSURE $y = x^n$ 
		\STATE $t = 0$ 
		\WHILE{$true$} 
			\STATE receive RRM and END from $D_{j}^{d}$ or $D_{j}^{s}$ to get $\xi_{\cdot,j}^{(t)}$, $r_{j}^{(t)}$, $rd_{j}^{(t)}$, $\eta_{\cdot}$ and $h_{\cdot,j}$
			\STATE $\lambda_{j}^{(t)} = \sum \xi_{\cdot,j}^{(t)}$
			\STATE $\Phi_{j} = \lambda_{j}^{(t)} / \theta_{j}\alpha_{j}$
			\IF{$s_{j} \in S^{1}$}
				\FOR{each $d_{m}$ in $D_{j}^{d}$}
					\STATE $r_{m,j}^{d2s} = B log_{2}(1+\frac{\eta_{m}h_{m,j}}{\sigma^2+\sum_{d_{m'}\in D_{j}^{d}\backslash \{ d_{m'}\} }\eta_{m'}h_{m',j}})$
				\ENDFOR
			\ENDIF
			\STATE Broadcast RSM including $\lambda_{j}^{(t)},r_{j}^{(t)},rd_{j}^{(t)}$ in $D_{j}^{d}$ or $D_{j}^{s}$
		
			\STATE $t=t+1$ 
		
		\ENDWHILE 
	\end{algorithmic} 
\end{algorithm}

\begin{algorithm} 
	\caption{Resource Request Algorithm for $s_{i}$} 
	\label{RRA} 
	\begin{algorithmic}
		%\REQUIRE $n \geq 0 \vee x \neq 0$ 
		%\ENSURE $y = x^n$ 
		\STATE Initialize $r_{i}^{(0)} = 0$
		\STATE Initialize $rd_{i}^{(0)} = 0$
		\FOR{each $s_{j} \in S_{i}^{s}$}
			\STATE Initialize $p_{i,j}^{(0)} = 1/|S_{i}^{s}|$
			\STATE send RRM including $\xi_{i}^{(0)}$, $r_{i}^{(0)}$, $rd_{i}^{(0)}$ to $s_{j}$
		\ENDFOR
		\STATE $t = 0$ 
		\WHILE{$true$} 
			\STATE receive $\lambda_{j}^{(t)},r_{j}^{(t)},rd_{j}^{(t)}$ from $S_{i}^{d}$ or $S_{j}^{s}$
			\STATE $R_{i}^{(t)} \gets $
			\IF{t>0 and Condition (16) is true}
				\FOR{each $s_{j} \in S_{i}^{s}$}
					\STATE send END to $s_{j}$
					\STATE $p_{i,j} = p_{i,j}^{(t)}$
				\ENDFOR
				\STATE return $p_{i,\cdot}$
			\ENDIF
			\STATE $p_{i,\cdot}^{(t+1)} \gets$
			\STATE $r_{i}^{(t+1)} \gets$
			\STATE $rd_{i}^{(t+1)} \gets$
			\FOR{each $s_{j} \in S_{i}^{s}$}
				\STATE $\xi_{i,j}^{(t+1)} = p_{i,j}^{(t+1)}$
				\STATE send RRM including $\xi_{i,j}^{(t+1)}$, $r_{i}^{(t+1)}$, $rd_{i}^{(t+1)}$
			\ENDFOR
		\STATE $t=t+1$ 
		\ENDWHILE
	\end{algorithmic} 
\end{algorithm}


\end{comment}



\begin{comment}

The response time of a batch of tasks on the edge server $s_{j}$ is composed of its computation delay and transmission delay.
$$T_{j} = t^{cp}_{j} + \hat{t}^{cm}_{\cdot,j} = \frac{\delta_{j}}{\mu_{j} - \lambda_{j}} + \sum\limits_{i}\frac{p_{ij}D_{j}}{\omega_{ij}}$$

For all tasks, the average system response time is $T(p)$
$$T(p) = \frac{1}{\Phi}\sum\limits_{j}T_{j}\Phi_{j} = \frac{1}{\Phi}\sum\limits_{j}(\frac{\delta_{j}\Phi_{j}}{\mu_{j} - \sum\limits_{i}p_{ij}\Phi_{i}\delta_{j}} + \sum\limits_{i}\frac{p_{ij}D_{j}\Phi_{j}}{\omega_{ij}})$$
where $p$ is the offloading strategy for all edge servers.


We aim to minimize the average response time by finding the best scheduling strategy of each edge server, which needs to take into account the heterogeneous situation of computing resource and bandwidth resources of different edge servers, as well as the impact of the early exit mechanism on the size of the data stream.





In the face of dynamic task request frequencies, our goal is to minimize system delay while maintaining as much accuracy as possible. In the case of low task request frequency, we need the system to be able to minimize system delay without compromising accuracy, In the case of high task request frequency, we need to achieve the trade-off between delay and precision without losing tasks as much as possible.
\end{comment}


\begin{comment}
	In order to meet latency and throughput requirements, \sout{ we need to determine the optimal model partitioning method and decide which edge servers to offload the partitioned models. Because different edge servers have different memory capacity and communication bandwidths, the partition of model directly affects the deployment of the entire system. If the granularity of partition is coarse, many edge servers may not load part of the model, resulting in reduced system throughput. If the granularity of partition is finer, the intermediate data propagating multiple times between edge servers will increases latency.}
	
	
\end{comment}


\begin{comment}
	$$\min_{B,X} ( \sum_{k=1}^{p-1} T^{cm}(\Phi_{k},\Phi_{k+1})+\sum_{k=1}^{p} T^{cp}(\Phi_{k}) )$$ 
	
	$$s.t.(1) M^{s}_{i}\geq mem(B_{k}), \forall S_{i}\in \Phi_{k}, k=1,2,...,p$$ 
	
	$$(2) \sum_{s_{i}\in \Phi_{k}} \frac{r^{c}_{i}}{f(B_{k})}\geq \alpha + (\beta_{max}-\alpha)\cdot I_{k}, k=1,2,...,p$$
\end{comment}

\begin{comment}
	内容...

\begin{equation}
	\label{1}
	\min_{p} T(p)
\end{equation}

\begin{equation}
	\label{2}
	\text{ s.t. }	
	\lambda_{i} < \mu_{i},   \forall s_{i}\in S
\end{equation}

\begin{equation}
	0 \leq p_{ij} \leq \pi_{i}, \forall s_{i}\in S
\end{equation}

\begin{equation}
	\sum\limits_{j} p_{ij} = \pi_{i}, \forall s_{i}\in S
\end{equation}


The first inequality expresses that the edge server needs to have enough memory to load the block of model. The second inequality means that the throughput of any block should not be less than the threshold of throughput, at the maximum task request frequency, the system can still process all tasks. Under these two constraints, we need to find the optimal model partitioning method and determine which edge servers each block is assigned to, so as to minimize the average inference delay. 


\end{comment}




%\bibliographystyle{alpha}
%\bibliography{sample}

